Exploring cosmic origins with CORE: effects of observer peculiar motion

We discuss the effects on the CMB, CIB, and thermal SZ effect due to the peculiar motion of an observer with respect to the CMB rest frame, which induces boosting effects. We investigate the scientific perspectives opened by future CMB space missions, focussing on the CORE proposal. The improvements in sensitivity offered by a mission like CORE, together with its high resolution over a wide frequency range, will provide a more accurate estimate of the CMB dipole. The extension of boosting effects to polarization and cross-correlations will enable a more robust determination of purely velocity-driven effects that are not degenerate with the intrinsic CMB dipole, allowing us to achieve a S/N ratio of 13; this improves on the Planck detection and essentially equals that of an ideal cosmic-variance-limited experiment up to a multipole l of 2000. Precise inter-frequency calibration will offer the opportunity to constrain or even detect CMB spectral distortions, particularly from the cosmological reionization, because of the frequency dependence of the dipole spectrum, without resorting to precise absolute calibration. The expected improvement with respect to COBE-FIRAS in the recovery of distortion parameters (in principle, a factor of several hundred for an ideal experiment with the CORE configuration) ranges from a factor of several up to about 50, depending on the quality of foreground removal and relative calibration. Even for 1% accuracy in both foreground removal and relative calibration at an angular scale of 1 deg, we find that dipole analyses for a mission like CORE will be able to improve the recovery of the CIB spectrum amplitude by a factor of 17 in comparison with current results based on FIRAS. In addition to the scientific potential of a mission like CORE for these analyses, synergies with other planned and ongoing projects are also discussed.

==> pecmotreferences <==
@ARTICLE{2017arXiv170400718M,
   author = {{Meerburg}, P.~D. and {Meyers}, J. and {van Engelen}, A.},
    title = "{Reconstructing the Primary CMB Dipole}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1704.00718},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
     year = 2017,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170400718M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170310456M,
   author = {{J.-B.Melin, A. Bonaldi, M. Remazeilles, S. Hagstotz, J.~M. Diego, et al., for the CORE collaboration}},
    title = "{Exploring Cosmic Origins with CORE: Cluster Science}",
    journal = {{\rm Companion Paper}, ArXiv e-prints},
    archivePrefix = "arXiv",
   eprint = {1703.10456},
 keywords = {},
     year = 2017,
    month = mar    
}

@article{Aghanim:2016yuo,
      author         = "{Planck Collaboration XLVI}",
      title          = "{Planck 2016 intermediate results. XLVI. Reduction of
                        large-scale systematic effects in HFI polarization maps
                        and estimation of the reionization optical depth}",
      year           = "2016",
      eprint         = "1605.02985",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1605.02985;%%"
}

@article{Roldan:2016ayx,
      author         = "Roldan, Omar and Notari, Alessio and Quartin, Miguel",
      title          = "{Interpreting the CMB aberration and Doppler
                        measurements: boost or intrinsic dipole?}",
      journal        = "JCAP",
      volume         = "1606",
      year           = "2016",
      number         = "06",
      pages          = "026",
      doi            = "10.1088/1475-7516/2016/06/026",
      eprint         = "1603.02664",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1603.02664;%%"
}

@article{Andre:2013nfa,
      author         = "Andr\'e, Philippe and others",
      title          = "{PRISM (Polarized Radiation Imaging and Spectroscopy
                        Mission): An Extended White Paper}",
      collaboration  = "PRISM",
      journal        = "JCAP",
      volume         = "1402",
      year           = "2014",
      pages          = "006",
      doi            = "10.1088/1475-7516/2014/02/006",
      eprint         = "1310.1554",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1310.1554;%%"
}

@article{Kogut:2011xw,
      author         = "Kogut, A. and others",
      title          = "{The Primordial Inflation Explorer (PIXIE): A Nulling
                        Polarimeter for Cosmic Microwave Background Observations}",
      journal        = "JCAP",
      volume         = "1107",
      year           = "2011",
      pages          = "025",
      doi            = "10.1088/1475-7516/2011/07/025",
      eprint         = "1105.2044",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1105.2044;%%"
}

@article{Bennett:2012zja,
      author         = "Bennett, C. L. and others",
      title          = "{Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP)
                        Observations: Final Maps and Results}",
      collaboration  = "WMAP",
      journal        = "Astrophys. J. Suppl.",
      volume         = "208",
      year           = "2013",
      pages          = "20",
      doi            = "10.1088/0067-0049/208/2/20",
      eprint         = "1212.5225",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1212.5225;%%"
}

@Article{Kogutothers2011,
  author        = {Kogut, A. and others},
  title         = {{The Primordial Inflation Explorer (PIXIE): A Nulling Polarimeter for Cosmic Microwave Background Observations}},
  journal       = {JCAP},
  year          = {2011},
  volume        = {1107},
  pages         = {025},
  archiveprefix = {arXiv},
  doi           = {10.1088/1475-7516/2011/07/025},
  eprint        = {1105.2044},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:1105.2044;%%},
}

@ARTICLE{2011arXiv1102.2181T,
   author = {{The COrE Collaboration} and {Armitage-Caplan}, C. and {Avillez}, M. and 
	{Barbosa}, D. and {Banday}, A. and {Bartolo}, N. and {Battye}, R. and 
	{Bernard}, J. and {de Bernardis}, P. and {Basak}, S. and {Bersanelli}, M. and 
	{Bielewicz}, P. and {Bonaldi}, A. and {Bucher}, M. and {Bouchet}, F. and 
	{Boulanger}, F. and {Burigana}, C. and {Camus}, P. and {Challinor}, A. and 
	{Chongchitnan}, S. and {Clements}, D. and {Colafrancesco}, S. and 
	{Delabrouille}, J. and {De Petris}, M. and {De Zotti}, G. and 
	{Dickinson}, C. and {Dunkley}, J. and {Ensslin}, T. and {Fergusson}, J. and 
	{Ferreira}, P. and {Ferriere}, K. and {Finelli}, F. and {Galli}, S. and 
	{Garcia-Bellido}, J. and {Gauthier}, C. and {Haverkorn}, M. and 
	{Hindmarsh}, M. and {Jaffe}, A. and {Kunz}, M. and {Lesgourgues}, J. and 
	{Liddle}, A. and {Liguori}, M. and {Lopez-Caniego}, M. and {Maffei}, B. and 
	{Marchegiani}, P. and {Martinez-Gonzalez}, E. and {Masi}, S. and 
	{Mauskopf}, P. and {Matarrese}, S. and {Melchiorri}, A. and 
	{Mukherjee}, P. and {Nati}, F. and {Natoli}, P. and {Negrello}, M. and 
	{Pagano}, L. and {Paoletti}, D. and {Peacocke}, T. and {Peiris}, H. and 
	{Perroto}, L. and {Piacentini}, F. and {Piat}, M. and {Piccirillo}, L. and 
	{Pisano}, G. and {Ponthieu}, N. and {Rath}, C. and {Ricciardi}, S. and 
	{Rubino Martin}, J. and {Salatino}, M. and {Shellard}, P. and 
	{Stompor}, R. and {Urrestilla}, L.~T.~J. and {Van Tent}, B. and 
	{Verde}, L. and {Wandelt}, B. and {Withington}, S.},
    title = "{COrE (Cosmic Origins Explorer) A White Paper}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1102.2181},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2011,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1102.2181T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CORE2016,
   author = {{Delabrouille}, J. and {de Bernardis}, P. and {Bouchet}, F.~R. and {the CORE Collaboration}},
    title = "{CORE -- The Cosmic Origins Explorer}",
  journal = {A proposal in response to the ESA call  for a Medium Size space mission for launch in 2029-2030},
    year = 2016
}

@article{Bouchet:2011ck,
      author         = "Bouchet, F. R. and others",
      title          = "{COrE (Cosmic Origins Explorer) A White Paper}",
      collaboration  = "COrE",
      year           = "2011",
      eprint         = "1102.2181",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1102.2181;%%"
}

@article{Sazonov:1998ae,
      author         = "Sazonov, S. Y. and Sunyaev, R. A.",
      title          = "{Cmb radiation in the direction of a moving cluster of
                        galaxies with hot gas: Relativistic corrections}",
      journal        = "Astrophys. J.",
      volume         = "508",
      year           = "1998",
      pages          = "1-5",
      doi            = "10.1086/306406",
      eprint         = "astro-ph/9804125",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9804125;%%"
}

@article{VanWaerbeke:2013cfa,
      author         = "Van Waerbeke, Ludovic and Hinshaw, Gary and Murray,
                        Norman",
      title          = "{Detection of warm and diffuse baryons in large scale
                        structure from the cross-correlation of gravitational
                        lensing and the thermal Sunyaev-Zeldovich effect}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "2",
      pages          = "023508",
      doi            = "10.1103/PhysRevD.89.023508",
      eprint         = "1310.5721",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1310.5721;%%"
}

@article{Hill:2013dxa,
      author         = "Hill, J. Colin and Spergel, David N.",
      title          = "{Detection of thermal SZ-CMB lensing cross-correlation in
                        Planck nominal mission data}",
      journal        = "JCAP",
      volume         = "1402",
      year           = "2014",
      pages          = "030",
      doi            = "10.1088/1475-7516/2014/02/030",
      eprint         = "1312.4525",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1312.4525;%%"
}

@Article{Abramo:2006gw,
  Title                    = {{Alignment Tests for low CMB multipoles}},
  Author                   = {Abramo, L. Raul and Bernui, Armando and Ferreira, Ivan S. and Villela, T. and Wuensche, C. Alexandre},
  Journal                  = {Phys.Rev.},
  Year                     = {2006},
  Pages                    = {063506},
  Volume                   = {D74},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.74.063506},
  Doi                      = {10.1103/PhysRevD.74.063506},
  Eprint                   = {astro-ph/0604346},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0604346;%%}
}

@Article{Adam:2015rua,
  Title                    = {{Planck 2015 results. I. Overview of products and scientific results}},
  Author                   = {{Planck Collaboration I}},
  Year                     = {2015},
  Archiveprefix            = {arXiv},
  Eprint                   = {1502.01582},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1502.01582;%%}
}

@Article{Adam:2015tpy,
  Title                    = {{Planck 2015 results. IX. Diffuse component separation:
 CMB maps}},
  Author                   = {{Planck Collaboration IX}},
  Year                     = {2015},
  Archiveprefix            = {arXiv},
  Eprint                   = {1502.05956},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1502.05956;%%},
  Timestamp                = {2015.10.13}
}

@article{Adam:2015vua,
      Author         = {{Planck Collaboration VIII}},
      title          = "{Planck 2015 results. VIII. High Frequency Instrument
                        data processing: Calibration and maps}",
      Journal        = {Astron.Astrophys.},
      doi            = "10.1051/0004-6361/201525820",
      year           = "2015",
      eprint         = "1502.01587",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1502.01587;%%"
}

@Article{Adam:2015wua,
  Title                    = {{Planck 2015 results. X. Diffuse component separation: Foreground maps}},
  Author                   = {{Planck Collaboration X}},
  Year                     = {2015},
  Archiveprefix            = {arXiv},
  Eprint                   = {1502.01588},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1502.01588;%%}
}

@Article{Ade:2015ads,
  Title                    = {{Planck 2015 results. V. LFI calibration}},
  Author                   = {{Planck Collaboration V}},
  Year                     = {2015},
  Archiveprefix            = {arXiv},
  Eprint                   = {1505.08022},
  Primaryclass             = {astro-ph.IM},
  Slaccitation             = {%%CITATION = ARXIV:1505.08022;%%}
}

@Article{Ade:2015dva,
  Title                    = {{Planck 2015 results. XXI. The integrated Sachs-Wolfe effect}},
  Author                   = {{Planck Collaboration XXI}},
  Year                     = {2015},
  Archiveprefix            = {arXiv},
  Eprint                   = {1502.01595},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1502.01595;%%}
}

@Article{Planck:2015xua,
  Title                    = {{Planck 2015 results. XIII. Cosmological parameters}},
  Author                   = {{Planck Collaboration XIII}},
  Year                     = {2015},
  Archiveprefix            = {arXiv},
  Eprint                   = {1502.01589},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1502.01589;%%}
}

@Article{Ade:2013eta,
  Title                    = {{Planck 2013 results. VIII. HFI photometric calibration
 and mapmaking}},
  Author                   = {{Planck Collaboration VIII}},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A8},
  Volume                   = {571},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361/201321538},
  Eprint                   = {1303.5069},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5069;%%},
  Timestamp                = {2015.10.13}
}

@Article{Ade:2013fta,
  Title                    = {{Planck 2013 results. IX. HFI spectral response}},
  Author                   = {{Planck Collaboration IX}},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A9},
  Volume                   = {571},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361/201321531},
  Eprint                   = {1303.5070},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.IM},
  Slaccitation             = {%%CITATION = ARXIV:1303.5070;%%},
  Timestamp                = {2015.10.13}
}

@Article{Ade:2013kta,
  Title                    = {{Planck 2013 results. XV. CMB power spectra and
 likelihood}},
  Author                   = {{Planck Collaboration XV}},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A15},
  Volume                   = {571},
  Archiveprefix            = {arXiv},
  Collaboration            = {Planck},
  Doi                      = {10.1051/0004-6361/201321573},
  Eprint                   = {1303.5075},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5075;%%},
  Timestamp                = {2015.10.13}
}


@Article{Ade:2013zuv,
  Title                    = {{Planck 2013 results. XVI. Cosmological parameters}},
  Author                   = {{Planck Collaboration XVI}},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A16},
  Volume                   = {571},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361/201321591},
  Eprint                   = {1303.5076},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5076;%%},
  Timestamp                = {2015.10.13}
}

@article{Ade:2013hta,
      author         = {{Planck Collaboration XII}},
      title          = "{Planck 2013 results. XII. Diffuse component separation}",
      journal        = "Astron. Astrophys.",
      volume         = "571",
      year           = "2014",
      pages          = "A12",
      doi            = "10.1051/0004-6361/201321580",
      eprint         = "1303.5072",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "CERN-PH-TH-2013-125",
      SLACcitation   = "%%CITATION = ARXIV:1303.5072;%%"
}

@Article{Ade:2013nlj,
  Title                    = {{Planck 2013 results. XXIII. Isotropy and statistics of the CMB, v3}},
  Author                   = {{Planck Collaboration XXIII}},
  Year                     = {2013},
  Archiveprefix            = {arXiv},
  Eprint                   = {1303.5083},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5083;%%}
}

@Article{Ade:2013nlj-v1,
  Title                    = {{Planck 2013 results. XXIII. Isotropy and statistics of the CMB, v1}},
  Author                   = {{Planck Collaboration XXIII}},
  Year                     = {2013},
  Archiveprefix            = {arXiv},
  Eprint                   = {1303.5083v1},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5083;%%}
}


@ARTICLE{2016A&A...594A..16P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Akrami}, Y. and {Aluri}, P.~K. and {Arnaud}, M. and {Ashdown}, M. and 
	{Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and et al.},
    title = "{Planck 2015 results. XVI. Isotropy and statistics of the CMB}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1506.07135},
 keywords = {cosmology: observations, cosmic background radiation, polarization, methods: data analysis, methods: statistical},
     year = 2016,
    month = sep,
   volume = 594,
      eid = {A16},
    pages = {A16},
      doi = {10.1051/0004-6361/201526681},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A..16P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ade:2013sjv,
	Archiveprefix = {arXiv},
	Author = {Ade, P.A.R. and others},
	Collaboration = {Planck},
	Doi = {10.1051/0004-6361/201321529},
	Eprint = {1303.5062},
	Journal = {Astron.Astrophys.},
	Pages = {A1},
	Primaryclass = {astro-ph.CO},
	Slaccitation = {%%CITATION = ARXIV:1303.5062;%%},
	Title = {{Planck 2013 results. I. Overview of products and scientific results}},
	Volume = {571},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201321529}
}

@Article{Aghanim:2013bta,
  Title                    = {{Planck 2013 results. V. LFI calibration}},
  Author                   = {{Planck Collaboration V}},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A5},
  Volume                   = {571},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361/201321527},
  Eprint                   = {1303.5066},
  Primaryclass             = {astro-ph.IM},
  Slaccitation             = {%%CITATION = ARXIV:1303.5066;%%}
}


@ARTICLE{2014A&A...571A..27P,
   author = {{Planck Collaboration} and {Aghanim}, N. and {Armitage-Caplan}, C. and 
	{Arnaud}, M. and {Ashdown}, M. and {Atrio-Barandela}, F. and 
	{Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B.  and others},
    title = "{Planck 2013 results. XXVII. Doppler boosting of the CMB: Eppur si muove}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.5087},
 keywords = {cosmology: observations, cosmic background radiation, reference systems, relativistic processes},
     year = 2014,
    month = nov,
   volume = 571,
      eid = {A27},
    pages = {A27},
      doi = {10.1051/0004-6361/201321556},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...571A..27P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{Aghanim:2013suk,
  Title                    = {{Planck 2013 results. XXVII. Doppler boosting of the CMB: Eppur si muove}},
  Author                   = {{Planck Collaboration XXVII}},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A27},
  Volume                   = {571},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1051/0004-6361/201321556},
  Doi                      = {10.1051/0004-6361/201321556},
  Eprint                   = {1303.5087},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5087;%%}
}

@ARTICLE{Aghanim:2015eva,
   author = {{Planck Collaboration} and {Aghanim}, N. and {Arnaud}, M. and 
	{Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and 
	{Barreiro}, R.~B. and {Bartlett}, J.~G. and {Bartolo}, N. and others},
    title = "{Planck 2015 results. XXII. A map of the thermal Sunyaev-Zeldovich effect}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1502.01596},
 keywords = {large-scale structure of Universe, cosmology: observations},
     year = 2016,
    month = sep,
   volume = 594,
      eid = {A22},
    pages = {A22},
      doi = {10.1051/0004-6361/201525826},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A..22P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{Akrami:2014eta,
  Title                    = {{Power asymmetry in WMAP and Planck temperature sky maps as measured by a local variance estimator}},
  Author                   = {Akrami, Y. and Fantaye, Y. and Shafieloo, A. and Eriksen, H.K. and Hansen, F.K. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {2014},
  Pages                    = {L42},
  Volume                   = {784},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/2041-8205/784/2/L42},
  Doi                      = {10.1088/2041-8205/784/2/L42},
  Eprint                   = {1402.0870},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1402.0870;%%}
}

@Article{Axelsson:2013mva,
  Title                    = {{Directional dependence of $\Lambda$CDM cosmological
 parameters}},
  Author                   = {Axelsson, M. and Fantaye, Y. and Hansen, F.K. and Banday,
 A.J. and Eriksen, H.K. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {2013},
  Pages                    = {L3},
  Volume                   = {773},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/2041-8205/773/1/L3},
  Eprint                   = {1303.5371},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5371;%%},
  Timestamp                = {2015.10.13}
}

@Article{Bennett:1996ce,
  Title                    = {{Four year COBE DMR cosmic microwave background observations: Maps and basic results}},
  Author                   = {Bennett, C.L. and Banday, A. and Gorski, K.M. and Hinshaw, G. and Jackson, P. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {1996},
  Pages                    = {L1-L4},
  Volume                   = {464},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/310075},
  Doi                      = {10.1086/310075},
  Eprint                   = {astro-ph/9601067},
  Primaryclass             = {astro-ph},
  Reportnumber             = {COBE-PREPRINT-96-01},
  Slaccitation             = {%%CITATION = ASTRO-PH/9601067;%%}
}

@Article{Bennett:2010jb,
  Title                    = {{Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Are There Cosmic Microwave Background Anomalies?}},
  Author                   = {Bennett, C.L. and Hill, R.S. and Hinshaw, G. and Larson, D. and Smith, K.M. and others},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2011},
  Pages                    = {17},
  Volume                   = {192},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/0067-0049/192/2/17},
  Doi                      = {10.1088/0067-0049/192/2/17},
  Eprint                   = {1001.4758},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1001.4758;%%}
}

@Article{Bennett:2003bz,
  Title                    = {{First year Wilkinson Microwave Anisotropy Probe (WMAP) observations: Preliminary maps and basic results}},
  Author                   = {Bennett, C.L. and others},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2003},
  Pages                    = {1-27},
  Volume                   = {148},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/377253},
  Collaboration            = {WMAP Collaboration},
  Doi                      = {10.1086/377253},
  Eprint                   = {astro-ph/0302207},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0302207;%%}
}

@Article{BenoitLevy:2013bc,
  Title                    = {{Full-sky CMB lensing reconstruction in presence of sky-cuts}},
  Author                   = {Benoit-Levy, Aurelien and Dechelette, Typhaine and Benabed, Karim and Cardoso, Jean-Francois and Hanson, Duncan and others},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2013},
  Pages                    = {A37},
  Volume                   = {555},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1051/0004-6361/201321048},
  Doi                      = {10.1051/0004-6361/201321048},
  Eprint                   = {1301.4145},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1301.4145;%%}
}

@Article{Bernui:2008cr,
  Title                    = {{Anomalous CMB north-south asymmetry}},
  Author                   = {Bernui, Armando},
  Journal                  = {Phys.Rev.},
  Year                     = {2008},
  Pages                    = {063531},
  Volume                   = {D78},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.78.063531},
  Doi                      = {10.1103/PhysRevD.78.063531},
  Eprint                   = {0809.0934},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ARXIV:0809.0934;%%}
}

@Article{Bernui:2014gla,
  Title                    = {{North-South non-Gaussian asymmetry in PLANCK CMB maps}},
  Author                   = {Bernui, A. and Oliveira, A.F. and Pereira, T.S.},
  Year                     = {2014},

  Archiveprefix            = {arXiv},
  Eprint                   = {1404.2936},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1404.2936;%%},
  Timestamp                = {2015.10.13}
}

@Article{Bernui:2006ft,
  Title                    = {{On the cmb large-scales angular correlations}},
  Author                   = {Bernui, Armando and Villela, Thyrso and Wuensche, Carlos A. and Leonardi, Rodrigo and Ferreira, Ivan},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2006},
  Pages                    = {409-414},
  Volume                   = {454},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1051/0004-6361:20054243},
  Doi                      = {10.1051/0004-6361:20054243},
  Eprint                   = {astro-ph/0601593},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0601593;%%}
}

@Article{Bielewicz:2004en,
  Title                    = {{Low order multipole maps of CMB anisotropy derived from WMAP}},
  Author                   = {Bielewicz, Pawel and Gorski, K.M. and Banday, A.J.},
  Journal                  = {Mon.Not.Roy.Astron.Soc.},
  Year                     = {2004},
  Pages                    = {1283},
  Volume                   = {355},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1111/j.1365-2966.2004.08405.x},
  Doi                      = {10.1111/j.1365-2966.2004.08405.x},
  Eprint                   = {astro-ph/0405007},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0405007;%%}
}

@Article{Bobin:2014mja,
  Title                    = {{Joint Planck and WMAP CMB Map Reconstruction}},
  Author                   = {Bobin, J. and Sureau, F. and Starck, J. -L. and Rassat, A. and Paykari, P.},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2014},
  Pages                    = {A105},
  Volume                   = {563},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1051/0004-6361/201322372},
  Doi                      = {10.1051/0004-6361/201322372},
  Eprint                   = {1401.6016},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1401.6016;%%}
}

@Article{Bond:1998zw,
  Title                    = {{Estimating the power spectrum of the cosmic microwave background}},
  Author                   = {Bond, J.R. and Jaffe, Andrew H. and Knox, L.},
  Journal                  = {Phys.Rev.},
  Year                     = {1998},
  Pages                    = {2117-2137},
  Volume                   = {D57},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.57.2117},
  Doi                      = {10.1103/PhysRevD.57.2117},
  Eprint                   = {astro-ph/9708203},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/9708203;%%}
}

@Article{Burles:2006xf,
  Title                    = {{Aberration of the Cosmic Microwave Background}},
  Author                   = {Burles, Scott and Rappaport, Saul},
  Journal                  = {Astrophys.J.},
  Year                     = {2006},
  Pages                    = {L1-L4},
  Volume                   = {641},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/503743},
  Doi                      = {10.1086/503743},
  Eprint                   = {astro-ph/0601559},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0601559;%%}
}

@Article{Calvao:2004ma,
  Title                    = {{Relativistic effects of our galaxy's motion on circles - in - the - sky}},
  Author                   = {Calvao, M.O. and Gomero, G.I. and Mota, B. and Reboucas, Marcelo J.},
  Journal                  = {Class.Quant.Grav.},
  Year                     = {2005},
  Pages                    = {1991-1999},
  Volume                   = {22},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/0264-9381/22/11/005},
  Doi                      = {10.1088/0264-9381/22/11/005},
  Eprint                   = {astro-ph/0404536},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0404536;%%}
}

@Article{Castro:2014oja,
  Title                    = {{First measurement of $\sigma_8$ using supernova magnitudes only}},
  Author                   = {Castro, Tiago and Quartin, Miguel},
  Year                     = {2014},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1093/mnrasl/slu071},
  Doi                      = {10.1093/mnrasl/slu071},
  Eprint                   = {1403.0293},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1403.0293;%%}
}

@Article{Catena:2013qd,
  Title                    = {{Non-Gaussianity and CMB aberration and Doppler}},
  Author                   = {Catena, Riccardo and Liguori, Michele and Notari, Alessio and Renzi, Alessandro},
  Journal                  = {JCAP},
  Year                     = {2013},
  Pages                    = {036},
  Volume                   = {1309},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/1475-7516/2013/09/036},
  Doi                      = {10.1088/1475-7516/2013/09/036},
  Eprint                   = {1301.3777},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1301.3777;%%}
}

@article{Catena:2012hq,
      author         = "Catena, Riccardo and Notari, Alessio",
      title          = "{Cosmological parameter estimation: impact of CMB
                        aberration}",
      journal        = "JCAP",
      volume         = "1304",
      year           = "2013",
      pages          = "028",
      doi            = "10.1088/1475-7516/2013/04/028",
      eprint         = "1210.2731",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1210.2731;%%"
}

@Article{Challinor:2002zh,
  Title                    = {{Peculiar velocity effects in high resolution microwave background experiments}},
  Author                   = {Challinor, Anthony and van Leeuwen, Floor},
  Journal                  = {Phys.Rev.},
  Year                     = {2002},
  Pages                    = {103001},
  Volume                   = {D65},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.65.103001},
  Doi                      = {10.1103/PhysRevD.65.103001},
  Eprint                   = {astro-ph/0112457},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0112457;%%}
}

@article{Chluba:2011zh,
      author         = "Chluba, J.",
      title          = "{Aberrating the CMB sky: fast and accurate computation of
                        the aberration kernel}",
      journal        = "Mon. Not. Roy. Astron. Soc.",
      volume         = "415",
      year           = "2011",
      pages          = "3227",
      doi            = "10.1111/j.1365-2966.2011.18934.x",
      eprint         = "1102.3415",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1102.3415;%%"
}

@Article{Chluba:2004cn,
  Title                    = {{Superposition of blackbodies and the dipole anisotropy:
 A Possibility to calibrate CMB experiments}},
  Author                   = {Chluba, Jens and Sunyaev, R.A.},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2003},
  Pages                    = {389-408},
  Volume                   = {424},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361:20041016},
  Eprint                   = {astro-ph/0404067},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0404067;%%}
}

@Article{Copi:2005ff,
  Title                    = {{On the large-angle anomalies of the microwave sky}},
  Author                   = {Copi, Craig J. and Huterer, D. and Schwarz, D.J. and
 Starkman, G.D.},
  Journal                  = {Mon.Not.Roy.Astron.Soc.},
  Year                     = {2006},
  Pages                    = {79-102},
  Volume                   = {367},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1111/j.1365-2966.2005.09980.x},
  Eprint                   = {astro-ph/0508047},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0508047;%%},
  Timestamp                = {2015.10.13}
}

@article{Copi:2013jna,
      author         = "Copi, Craig J. and Huterer, Dragan and Schwarz, Dominik
                        J. and Starkman, Glenn D.",
      title          = "{Large-scale alignments from WMAP and Planck}",
      journal        = "Mon. Not. Roy. Astron. Soc.",
      volume         = "449",
      year           = "2015",
      number         = "4",
      pages          = "3458-3470",
      doi            = "10.1093/mnras/stv501",
      eprint         = "1311.4562",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1311.4562;%%"
}
@Article{Copi:2003kt,
  Title                    = {{Multipole vectors - A New representation of the CMB sky
 and evidence for statistical anisotropy or non-Gaussianity
 at $2 \le l \le 8$}},
  Author                   = {Copi, Craig J. and Huterer, Dragan and Starkman, Glenn
 D.},
  Journal                  = {Phys.Rev.},
  Year                     = {2004},
  Pages                    = {043515},
  Volume                   = {D70},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1103/PhysRevD.70.043515},
  Eprint                   = {astro-ph/0310511},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0310511;%%},
  Timestamp                = {2015.10.13}
}

@Article{CopiHutererStarkman2004,
  author        = {Copi, Craig J. and Huterer, Dragan and Starkman, Glenn D.},
  title         = {{Multipole vectors - A New representation of the CMB sky and evidence for statistical anisotropy or non-Gaussianity at $2 \le l \le 8$}},
  journal       = {Phys.Rev.},
  year          = {2004},
  volume        = {D70},
  pages         = {043515},
  archiveprefix = {arXiv},
  bdsk-url-1    = {http://dx.doi.org/10.1103/PhysRevD.70.043515},
  doi           = {10.1103/PhysRevD.70.043515},
  eprint        = {astro-ph/0310511},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0310511;%%},
}

@Article{Dai:2013kfa,
  Title                    = {{The Pesky Power Asymmetry}},
  Author                   = {Dai, Liang and Jeong, Donghui and Kamionkowski, Marc and Chluba, Jens},
  Year                     = {2013},

  Archiveprefix            = {arXiv},
  Eprint                   = {1303.6949},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.6949;%%}
}

@Book{Dodelson:2003ft,
  Title                    = {{Modern cosmology}},
  Author                   = {Dodelson, Scott},
  Publisher                = {Academic Press},
  Year                     = {2003},
  Note                     = {Book's website: \url{http://home.fnal.gov/~dodelson/book.html}},

  Chapter                  = {11},
  Owner                    = {Miguel Quartin},
  Timestamp                = {2015.10.13}
}

@Article{Dunkley:2013vu,
  Title                    = {{The Atacama Cosmology Telescope: likelihood for
 small-scale CMB data}},
  Author                   = {Dunkley, J. and Calabrese, E. and Sievers, J. and
 Addison, G.E. and Battaglia, N. and others},
  Year                     = {2013},

  Archiveprefix            = {arXiv},
  Eprint                   = {1301.0776},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1301.0776;%%},
  Timestamp                = {2015.10.13}
}

@Article{Efstathiou:2003tv,
  Title                    = {{A Maximum likelihood analysis of the low CMB multipoles from WMAP}},
  Author                   = {Efstathiou, G.},
  Journal                  = {Mon.Not.Roy.Astron.Soc.},
  Year                     = {2004},
  Pages                    = {885},
  Volume                   = {348},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1111/j.1365-2966.2004.07409.x},
  Doi                      = {10.1111/j.1365-2966.2004.07409.x},
  Eprint                   = {astro-ph/0310207},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0310207;%%}
}

@Article{Efstathiou:2003wr,
  Title                    = {{The Statistical significance of the low CMB multipoles}},
  Author                   = {Efstathiou, G.},
  Journal                  = {Mon.Not.Roy.Astron.Soc.},
  Year                     = {2003},
  Pages                    = {L26},
  Volume                   = {346},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1046/j.1365-2966.2003.07304.x},
  Eprint                   = {astro-ph/0306431},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0306431;%%},
  Timestamp                = {2015.10.13}
}

@Article{Eriksen:2003db,
  Title                    = {{Asymmetries in the Cosmic Microwave Background anisotropy field}},
  Author                   = {Eriksen, H.K. and Hansen, F.K. and Banday, A.J. and Gorski, K.M. and Lilje, P.B.},
  Journal                  = {Astrophys.J.},
  Year                     = {2004},
  Pages                    = {14-20},
  Volume                   = {605},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/382267},
  Doi                      = {10.1086/382267},
  Eprint                   = {astro-ph/0307507},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0307507;%%}
}

@Article{EriksenHansenBandayEtAl2004,
  author        = {Eriksen, H.K. and Hansen, F.K. and Banday, A.J. and Gorski, K.M. and Lilje, P.B.},
  title         = {{Asymmetries in the Cosmic Microwave Background anisotropy field}},
  journal       = {Astrophys.J.},
  year          = {2004},
  volume        = {605},
  pages         = {14-20},
  archiveprefix = {arXiv},
  doi           = {10.1086/382267},
  eprint        = {astro-ph/0307507},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0307507;%%},
  timestamp     = {2015.10.13},
}

@Article{Eriksen:2007pc,
  Title                    = {{Hemispherical power asymmetry in the three-year Wilkinson Microwave Anisotropy Probe sky maps}},
  Author                   = {Eriksen, Hans K. and Banday, A.J. and Gorski, K.M. and Hansen, F.K. and Lilje, P.B.},
  Journal                  = {Astrophys.J.},
  Year                     = {2007},
  Pages                    = {L81-L84},
  Volume                   = {660},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/518091},
  Doi                      = {10.1086/518091},
  Eprint                   = {astro-ph/0701089},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0701089;%%}
}

@Article{EriksenBandayGorskiEtAl2007,
  author        = {Eriksen, Hans K. and Banday, A.J. and Gorski, K.M. and Hansen, F.K. and Lilje, P.B.},
  title         = {{Hemispherical power asymmetry in the three-year Wilkinson Microwave Anisotropy Probe sky maps}},
  journal       = {Astrophys.J.},
  year          = {2007},
  volume        = {660},
  pages         = {L81-L84},
  archiveprefix = {arXiv},
  doi           = {10.1086/518091},
  eprint        = {astro-ph/0701089},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0701089;%%},
  timestamp     = {2015.10.13},
}

@Article{Fixsen:2009ug,
  Title                    = {{The Temperature of the Cosmic Microwave Background}},
  Author                   = {Fixsen, D. J.},
  Journal                  = {Astrophys. J.},
  Year                     = {2009},
  Pages                    = {916-920},
  Volume                   = {707},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/707/2/916},
  Eprint                   = {0911.1955},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:0911.1955;%%}
}

@Article{Flender:2013jja,
  Title                    = {{The small scale power asymmetry in the cosmic microwave background}},
  Author                   = {Flender, Samuel and Hotchkiss, Shaun},
  Journal                  = {JCAP},
  Year                     = {2013},
  Pages                    = {033},
  Volume                   = {1309},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/1475-7516/2013/09/033},
  Doi                      = {10.1088/1475-7516/2013/09/033},
  Eprint                   = {1307.6069},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1307.6069;%%}
}

@Article{Francis-2010,
  Title                    = {{An estimate of the local integrated Sachs-Wolfe signal and its impact on cosmic microwave background anomalies}},
  Author                   = {{Francis}, C.~L. and {Peacock}, J.~A.},
  Journal                  = {MNRAS},
  Year                     = {2010},

  Month                    = jul,
  Pages                    = {14-21},
  Volume                   = {406},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2010MNRAS.406...14F},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1111/j.1365-2966.2010.16866.x},
  Eprint                   = {0909.2495},
  Keywords                 = {cosmic background radiation, cosmology: observations, large-scale structure of Universe},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Timestamp                = {2015.10.13}
}

@Article{Galli:2014kla,
  Title                    = {{CMB Polarization can constrain cosmology better than CMB
 temperature}},
  Author                   = {Galli, Silvia and Benabed, Karim and Bouchet, François
 and Cardoso, Jean-François and Elsner, Franz and others},
  Year                     = {2014},

  Archiveprefix            = {arXiv},
  Eprint                   = {1403.5271},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1403.5271;%%},
  Timestamp                = {2015.10.13}
}

@Article{Gorski:2004by,
  Title                    = {{HEALPix - A Framework for high resolution
 discretization, and fast analysis of data distributed on
 the sphere}},
  Author                   = {Gorski, K.M. and Hivon, Eric and Banday, A.J. and
 Wandelt, B.D. and Hansen, F.K. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {2005},
  Pages                    = {759-771},
  Volume                   = {622},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1086/427976},
  Eprint                   = {astro-ph/0409513},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0409513;%%},
  Timestamp                = {2015.10.13}
}

@Article{GorskiHivonBandayEtAl2005,
  author        = {Gorski, K.M. and Hivon, Eric and Banday, A.J. and Wandelt, B.D. and Hansen, F.K. and others},
  title         = {{HEALPix - A Framework for high resolution discretization, and fast analysis of data distributed on the sphere}},
  journal       = {Astrophys.J.},
  year          = {2005},
  volume        = {622},
  pages         = {759-771},
  archiveprefix = {arXiv},
  bdsk-url-1    = {http://dx.doi.org/10.1086/427976},
  doi           = {10.1086/427976},
  eprint        = {astro-ph/0409513},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0409513;%%},
}

@Book{Gregory:2010,
  Title                    = {{Bayesian Logical Data Analysis for the Physical Sciences}},
  Author                   = {Gregory, Phil},
  Publisher                = {Cambridge University Press},
  Year                     = {2010},

  Chapter                  = {3}
}

@Article{Hansen:2008ym,
  Title                    = {{Power Asymmetry in Cosmic Microwave Background Fluctuations from Full Sky to Sub-degree Scales: Is the Universe Isotropic?}},
  Author                   = {Hansen, F.K. and Banday, A.J. and Gorski, K.M. and Eriksen, H.K. and Lilje, P.B.},
  Journal                  = {Astrophys.J.},
  Year                     = {2009},
  Pages                    = {1448-1458},
  Volume                   = {704},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/0004-637X/704/2/1448},
  Doi                      = {10.1088/0004-637X/704/2/1448},
  Eprint                   = {0812.3795},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ARXIV:0812.3795;%%}
}


@Article{Hansen:2004vq,
  Title                    = {{Testing the cosmological principle of isotropy: Local power spectrum estimates of the WMAP data}},
  Author                   = {Hansen, Frode K. and Banday, A.J. and Gorski, K.M.},
  Journal                  = {Mon.Not.Roy.Astron.Soc.},
  Year                     = {2004},
  Pages                    = {641-665},
  Volume                   = {354},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1111/j.1365-2966.2004.08229.x},
  Doi                      = {10.1111/j.1365-2966.2004.08229.x},
  Eprint                   = {astro-ph/0404206},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0404206;%%}
}

@Article{Hansen:2004mj,
  Title                    = {{Asymmetries in the local curvature of the WMAP data}},
  Author                   = {Hansen, Frode K. and Cabella, Paolo and Marinucci,
 Domenico and Vittorio, Nicola},
  Journal                  = {Astrophys.J.},
  Year                     = {2004},
  Pages                    = {L67-L70},
  Volume                   = {607},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1086/421904},
  Eprint                   = {astro-ph/0402396},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0402396;%%},
  Timestamp                = {2015.10.13}
}

@article{Hanson:2009gu,
      author         = "Hanson, Duncan and Lewis, Antony",
      title          = "{Estimators for CMB Statistical Anisotropy}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "063004",
      doi            = "10.1103/PhysRevD.80.063004",
      eprint         = "0908.0963",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:0908.0963;%%"
}

@Article{Helling:2006xh,
  Title                    = {{CMB statistical anisotropy, multipole vectors and the influence of the dipole}},
  Author                   = {Helling, Robert C. and Schupp, Peter and Tesileanu, Tiberiu},
  Journal                  = {Phys.Rev.},
  Year                     = {2006},
  Pages                    = {063004},
  Volume                   = {D74},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.74.063004},
  Doi                      = {10.1103/PhysRevD.74.063004},
  Eprint                   = {astro-ph/0603594},
  Primaryclass             = {astro-ph},
  Reportnumber             = {IUB-TH-0601},
  Slaccitation             = {%%CITATION = ASTRO-PH/0603594;%%}
}

@Article{2010A&A...520A.101H,
  Title                    = {{Revisiting the WMAP-NVSS angular cross correlation. A skeptic's view}},
  Author                   = {{Hern{\'a}ndez-Monteagudo}, C.},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2010},

  Month                    = sep,
  Pages                    = {A101},
  Volume                   = {520},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2010A%26A...520A.101H},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1051/0004-6361/200913344},
  Doi                      = {10.1051/0004-6361/200913344},
  Eid                      = {A101},
  Eprint                   = {0909.4294},
  Keywords                 = {cosmic microwave background, large scale structure of Universe},
  Primaryclass             = {astro-ph.CO}
}

@Article{Hinshaw:1996uq,
  Title                    = {{Band power spectra in the COBE DMR 4-year anisotropy
 maps}},
  Author                   = {Hinshaw, G. and Banday, A.J. and Bennett, C.L. and
 Gorski, K.M. and Kogut, Alan and others},
  Journal                  = {Astrophys.J.},
  Year                     = {1996},
  Pages                    = {L17-L20},
  Volume                   = {464},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1086/310074},
  Eprint                   = {astro-ph/9601058},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Reportnumber             = {COBE-PREPRINT-96-04},
  Slaccitation             = {%%CITATION = ASTRO-PH/9601058;%%},
  Timestamp                = {2015.10.13}
}

@Article{Hinshaw:2008kr,
  Title                    = {{Five-Year Wilkinson Microwave Anisotropy Probe (WMAP)
 Observations: Data Processing, Sky Maps, and Basic
 Results}},
  Author                   = {Hinshaw, G. and others},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2009},
  Pages                    = {225-245},
  Volume                   = {180},

  Archiveprefix            = {arXiv},
  Collaboration            = {WMAP Collaboration},
  Doi                      = {10.1088/0067-0049/180/2/225},
  Eprint                   = {0803.0732},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Timestamp                = {2015.10.13}
}

@Article{Hinshawothers2009,
  author        = {Hinshaw, G. and others},
  title         = {{Five-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Data Processing, Sky Maps, and Basic Results}},
  journal       = {Astrophys.J.Suppl.},
  year          = {2009},
  volume        = {180},
  pages         = {225-245},
  archiveprefix = {arXiv},
  bdsk-url-1    = {http://dx.doi.org/10.1088/0067-0049/180/2/225},
  collaboration = {WMAP},
  doi           = {10.1088/0067-0049/180/2/225},
  eprint        = {0803.0732},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ARXIV:0803.0732;%%},
}

@Article{Hinshaw:2003ex,
  Title                    = {{First year Wilkinson Microwave Anisotropy Probe (WMAP) observations: The Angular power spectrum}},
  Author                   = {Hinshaw, G. and others},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2003},
  Pages                    = {135},
  Volume                   = {148},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/377225},
  Collaboration            = {WMAP},
  Doi                      = {10.1086/377225},
  Eprint                   = {astro-ph/0302217},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0302217;%%}
}

@Article{Hinshawothers2003,
  author        = {Hinshaw, G. and others},
  title         = {{First year Wilkinson Microwave Anisotropy Probe (WMAP) observations: The Angular power spectrum}},
  journal       = {Astrophys.J.Suppl.},
  year          = {2003},
  volume        = {148},
  pages         = {135},
  archiveprefix = {arXiv},
  collaboration = {WMAP},
  doi           = {10.1086/377225},
  eprint        = {astro-ph/0302217},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0302217;%%},
  timestamp     = {2015.10.13},
}

@Article{Hinshaw:2003fc,
  Title                    = {{First year Wilkinson Microwave Anisotropy Probe (WMAP) observations: Data processing methods and systematic errors limits}},
  Author                   = {Hinshaw, G. and others},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2003},
  Pages                    = {63},
  Volume                   = {148},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/377222},
  Collaboration            = {WMAP},
  Doi                      = {10.1086/377222},
  Eprint                   = {astro-ph/0302222},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0302222;%%}
}

@Article{Hivon:2001jp,
  Title                    = {{Master of the cosmic microwave background anisotropy
 power spectrum: a fast method for statistical analysis of
 large and complex cosmic microwave background data sets}},
  Author                   = {Hivon, E. and Gorski, K.M. and Netterfield, C.B. and
 Crill, B.P. and Prunet, S. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {2002},
  Pages                    = {2},
  Volume                   = {567},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1086/338126},
  Eprint                   = {astro-ph/0105302},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0105302;%%},
  Timestamp                = {2015.10.13}
}

@Article{HivonGorskiNetterfieldEtAl2002,
  author        = {Hivon, E. and Gorski, K.M. and Netterfield, C.B. and Crill, B.P. and Prunet, S. and others},
  title         = {{Master of the cosmic microwave background anisotropy power spectrum: a fast method for statistical analysis of large and complex cosmic microwave background data sets}},
  journal       = {Astrophys.J.},
  year          = {2002},
  volume        = {567},
  pages         = {2},
  archiveprefix = {arXiv},
  bdsk-url-1    = {http://dx.doi.org/10.1086/338126},
  doi           = {10.1086/338126},
  eprint        = {astro-ph/0105302},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0105302;%%},
}

@Article{Hoftuft:2009rq,
  Title                    = {{Increasing evidence for hemispherical power asymmetry in
 the five-year WMAP data}},
  Author                   = {Hoftuft, J. and Eriksen, H.K. and Banday, A.J. and
 Gorski, K.M. and Hansen, F.K. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {2009},
  Pages                    = {985-989},
  Volume                   = {699},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/699/2/985},
  Eprint                   = {0903.1229},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:0903.1229;%%},
  Timestamp                = {2015.10.13}
}

@Article{HoftuftEriksenBandayEtAl2009,
  author        = {Hoftuft, J. and Eriksen, H.K. and Banday, A.J. and Gorski, K.M. and Hansen, F.K. and others},
  title         = {{Increasing evidence for hemispherical power asymmetry in the five-year WMAP data}},
  journal       = {Astrophys.J.},
  year          = {2009},
  volume        = {699},
  pages         = {985-989},
  archiveprefix = {arXiv},
  bdsk-url-1    = {http://dx.doi.org/10.1088/0004-637X/699/2/985},
  doi           = {10.1088/0004-637X/699/2/985},
  eprint        = {0903.1229},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:0903.1229;%%},
}

@Article{2011ApJS..192...14J,
  Title                    = {{Seven-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Sky Maps, Systematic Errors, and Basic Results}},
  Author                   = {{Jarosik}, N. and {Bennett}, C.~L. and {Dunkley}, J. and {Gold}, B. and {Greason}, M.~R. and {Halpern}, M. and {Hill}, R.~S. and {Hinshaw}, G. and {Kogut}, A. and {Komatsu}, E. and {Larson}, D. and {Limon}, M. and {Meyer}, S.~S. and {Nolta}, M.~R. and {Odegard}, N. and {Page}, L. and {Smith}, K.~M. and {Spergel}, D.~N. and {Tucker}, G.~S. and {Weiland}, J.~L. and {Wollack}, E. and {Wright}, E.~L.},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2011},

  Month                    = feb,
  Pages                    = {14},
  Volume                   = {192},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2011ApJS..192...14J},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/0067-0049/192/2/14},
  Collaboration            = {WMAP},
  Doi                      = {10.1088/0067-0049/192/2/14},
  Eid                      = {14},
  Eprint                   = {1001.4744},
  Keywords                 = {cosmic background radiation, space vehicles: instruments},
  Primaryclass             = {astro-ph.CO}
}

@article{Jeong:2013sxy,
      author         = "Jeong, Donghui and Chluba, Jens and Dai, Liang and
                        Kamionkowski, Marc and Wang, Xin",
      title          = "{The effect of aberration on partial-sky measurements of
                        the cosmic microwave background temperature power
                        spectrum}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "2",
      pages          = "023003",
      doi            = "10.1103/PhysRevD.89.023003",
      eprint         = "1309.2285",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1309.2285;%%"
}

@Article{Kamionkowski:2002nd,
  Title                    = {{Aspects of the cosmic microwave background dipole}},
  Author                   = {Kamionkowski, M. and Knox, Lloyd},
  Journal                  = {Phys.Rev.},
  Year                     = {2003},
  Pages                    = {063001},
  Volume                   = {D67},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.67.063001},
  Doi                      = {10.1103/PhysRevD.67.063001},
  Eprint                   = {astro-ph/0210165},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0210165;%%}
}

@Article{2012PhRvD..85f3001K,
  Title                    = {{Test for anisotropy in the mean of the CMB temperature fluctuation in spherical harmonic space}},
  Author                   = {{Kashino}, D. and {Ichiki}, K. and {Takeuchi}, T.~T.},
  Journal                  = {Phys.Rev. D},
  Year                     = {2012},

  Month                    = mar,
  Number                   = {6},
  Pages                    = {063001},
  Volume                   = {85},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2012PhRvD..85f3001K},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.85.063001},
  Doi                      = {10.1103/PhysRevD.85.063001},
  Eid                      = {063001},
  Eprint                   = {1112.0924},
  Keywords                 = {Background radiations, Cosmology, Observational cosmology},
  Primaryclass             = {astro-ph.CO}
}

@Article{Keisler:2011aw,
  Title                    = {{A Measurement of the Damping Tail of the Cosmic Microwave Background Power Spectrum with the South Pole Telescope}},
  Author                   = {Keisler, R. and Reichardt, C.L. and Aird, K.A. and Benson, B.A. and Bleem, L.E. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {2011},
  Pages                    = {28},
  Volume                   = {743},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/0004-637X/743/1/28},
  Doi                      = {10.1088/0004-637X/743/1/28},
  Eprint                   = {1105.3182},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1105.3182;%%}
}

@Article{KeislerReichardtAirdEtAl2011,
  author        = {Keisler, R. and Reichardt, C.L. and Aird, K.A. and Benson, B.A. and Bleem, L.E. and others},
  title         = {{A Measurement of the Damping Tail of the Cosmic Microwave Background Power Spectrum with the South Pole Telescope}},
  journal       = {Astrophys.J.},
  year          = {2011},
  volume        = {743},
  pages         = {28},
  archiveprefix = {arXiv},
  doi           = {10.1088/0004-637X/743/1/28},
  eprint        = {1105.3182},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:1105.3182;%%},
  timestamp     = {2015.10.13},
}

@Article{Kosowsky:2010jm,
  Title                    = {{The Signature of Proper Motion in the Microwave Sky}},
  Author                   = {Kosowsky, Arthur and Kahniashvili, Tina},
  Journal                  = {Phys.Rev.Lett.},
  Year                     = {2011},
  Pages                    = {191301},
  Volume                   = {106},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1103/PhysRevLett.106.191301},
  Eprint                   = {1007.4539},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1007.4539;%%},
  Timestamp                = {2015.10.13}
}

@Article{Larson:2014roa,
  Title                    = {{Comparing Planck and WMAP: Maps, Spectra, and
 Parameters}},
  Author                   = {Larson, D. and Weiland, J.L. and Hinshaw, G. and Bennett,
 C.L.},
  Journal                  = {Astrophys.J.},
  Year                     = {2015},
  Number                   = {1},
  Pages                    = {9},
  Volume                   = {801},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/801/1/9},
  Eprint                   = {1409.7718},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1409.7718;%%},
  Timestamp                = {2015.10.13}
}

@Article{Lewis:1999bs,
  Title                    = {{Efficient computation of CMB anisotropies in closed FRW models}},
  Author                   = {Lewis, Antony and Challinor, Anthony and Lasenby, Anthony},
  Journal                  = {Astrophys.J.},
  Year                     = {2000},
  Note                     = {\url{http://camb.info}},
  Pages                    = {473-476},
  Volume                   = {538},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/309179},
  Doi                      = {10.1086/309179},
  Eprint                   = {astro-ph/9911177},
  Primaryclass             = {astro-ph}
}

@Article{Lineweaver:1996xa,
  Title                    = {{The dipole observed in the COBE DMR four-year data}},
  Author                   = {Lineweaver, C.H. and Tenorio, L. and Smoot, George F. and
 Keegstra, P. and Banday, A.J. and others},
  Journal                  = {Astrophys.J.},
  Year                     = {1996},
  Pages                    = {38-42},
  Volume                   = {470},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1086/177846},
  Eprint                   = {astro-ph/9601151},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/9601151;%%},
  Timestamp                = {2015.10.13}
}

@Article{Mather:1998gm,
  Title                    = {{Calibrator design for the COBE far infrared absolute spectrophotometer (FIRAS)}},
  Author                   = {Mather, John C. and Fixsen, D.J. and Shafer, R.A. and Mosier, C. and Wilkinson, D.T.},
  Journal                  = {Astrophys.J.},
  Year                     = {1999},
  Pages                    = {511-520},
  Volume                   = {512},
  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/306805},
  Doi                      = {10.1086/306805},
  Eprint                   = {astro-ph/9810373},
  Primaryclass             = {astro-ph}
}

@Article{Menzies:2004vr,
  Title                    = {{Peculiar velocity and deaberration of the sky}},
  Author                   = {Menzies, Dylan and Mathews, G.J.},
  Journal                  = {Astrophys.J.},
  Year                     = {2005},
  Pages                    = {7-9},
  Volume                   = {624},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1086/428936},
  Eprint                   = {astro-ph/0409175},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Timestamp                = {2015.10.13}
}

@Article{Mukherjee:2013zbi,
  Title                    = {{Statistical isotropy violation of CMB Polarization sky
 due to Lorentz boost}},
  Author                   = {Mukherjee, Suvodip and De, Aritra and Souradeep, Tarun},
  Journal                  = {Phys.Rev.},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {083005},
  Volume                   = {D89},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1103/PhysRevD.89.083005},
  Eprint                   = {1309.3800},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1309.3800;%%},
  Timestamp                = {2015.10.13}
}

@Article{Notari:2015kla,
  Title                    = {{On the proper kinetic quadrupole CMB removal and the
 quadrupole anomalies}},
  Author                   = {Notari, Alessio and Quartin, Miguel},
  Journal                  = {JCAP},
  Year                     = {2015},
  Number                   = {06},
  Pages                    = {047},
  Volume                   = {1506},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/1475-7516/2015/06/047},
  Eprint                   = {1504.02076},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1504.02076;%%}
}

@Article{Notari:2011sb,
  Title                    = {{Measuring our Peculiar Velocity by 'Pre-deboosting' the
 CMB}},
  Author                   = {Notari, Alessio and Quartin, Miguel},
  Journal                  = {JCAP},
  Year                     = {2012},
  Pages                    = {026},
  Volume                   = {1202},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/1475-7516/2012/02/026},
  Eprint                   = {1112.1400},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1112.1400;%%},
  Timestamp                = {2015.10.13}
}

@Article{Notari:2013iva,
  Title                    = {{CMB Aberration and Doppler Effects as a Source of Hemispherical Asymmetries}},
  Author                   = {Notari, Alessio and Quartin, Miguel and Catena, Riccardo},
  Journal                  = {JCAP},
  Year                     = {2014},
  Pages                    = {019},
  Volume                   = {1403},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/1475-7516/2014/03/019},
  Doi                      = {10.1088/1475-7516/2014/03/019},
  Eprint                   = {1304.3506},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1304.3506;%%}
}

@Article{deOliveiraCosta:2003pu,
  Title                    = {{The Significance of the largest scale CMB fluctuations in WMAP}},
  Author                   = {de Oliveira-Costa, Angelica and Tegmark, Max and Zaldarriaga, Matias and Hamilton, Andrew},
  Journal                  = {Phys.Rev.},
  Year                     = {2004},
  Pages                    = {063516},
  Volume                   = {D69},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1103/PhysRevD.69.063516},
  Doi                      = {10.1103/PhysRevD.69.063516},
  Eprint                   = {astro-ph/0307282},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0307282;%%}
}

@Article{Oliveira-CostaTegmarkZaldarriagaEtAl2004,
  author        = {de Oliveira-Costa, Angelica and Tegmark, Max and Zaldarriaga, Matias and Hamilton, Andrew},
  title         = {{The Significance of the largest scale CMB fluctuations in WMAP}},
  journal       = {Phys.Rev.},
  year          = {2004},
  volume        = {D69},
  pages         = {063516},
  archiveprefix = {arXiv},
  doi           = {10.1103/PhysRevD.69.063516},
  eprint        = {astro-ph/0307282},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0307282;%%},
  timestamp     = {2015.10.13},
}


@Article{Peebles:1968,
  Title                    = {{Comment on the Anisotropy of the Primeval Fireball}},
  Author                   = {{Peebles}, P.~J. and {Wilkinson}, D.~T.},
  Journal                  = {Physical Review},
  Year                     = {1968},

  Month                    = oct,
  Pages                    = {2168-2168},
  Volume                   = {174},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/1968PhRv..174.2168P},
  Doi                      = {10.1103/PhysRev.174.2168}
}

@ARTICLE{Pereira:2010dn,
   author = {{Pereira}, T.~S. and {Yoho}, A. and {Stuke}, M. and {Starkman}, G.~D.
	},
    title = "{Effects of a Cut, Lorentz-Boosted sky on the Angular Power Spectrum}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1009.4937},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2010,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1009.4937P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Aghanim:2013zsg,
      author         = {{Planck Collaboration V}},
      title          = "{Planck 2013 results. V. LFI calibration}",
      journal        = "Astron. Astrophys.",
      volume         = "571",
      year           = "2014",
      pages          = "A5",
      doi            = "10.1051/0004-6361/201321527",
      eprint         = "1303.5066",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      reportNumber   = "CERN-PH-TH-2013-119",
      SLACcitation   = "%%CITATION = ARXIV:1303.5066;%%"
}

@Article{PolastriGruppusoNatoli2015,
  author        = {Polastri, L. and Gruppuso, A. and Natoli, P.},
  title         = {{CMB low multipole alignments in the $\mathbf{\Lambda}$CDM and Dipolar models}},
  journal       = {JCAP},
  year          = {2015},
  volume        = {1504},
  number        = {04},
  pages         = {018},
  archiveprefix = {arXiv},
  doi           = {10.1088/1475-7516/2015/04/018},
  eprint        = {1503.01611},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:1503.01611;%%},
  timestamp     = {2015.10.13},
}

@Article{Polastri:2015rda,
  Title                    = {{CMB low multipole alignments in the $\mathbf{\Lambda}$CDM and Dipolar models}},
  Author                   = {Polastri, L. and Gruppuso, A. and Natoli, P.},
  Year                     = {2015},

  Archiveprefix            = {arXiv},
  Eprint                   = {1503.01611},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1503.01611;%%}
}

@Article{Quartin:2014yaa,
  Title                    = {{On the significance of power asymmetries in Planck CMB
 data at all scales}},
  Author                   = {Quartin, Miguel and Notari, Alessio},
  Journal                  = {JCAP},
  Year                     = {2015},
  Number                   = {01},
  Pages                    = {008},
  Volume                   = {1501},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/1475-7516/2015/01/008},
  Eprint                   = {1408.5792},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1408.5792;%%},
  Timestamp                = {2015.10.13}
}

@article{Quartin:2015kaa,
      author         = "Quartin, Miguel and Notari, Alessio",
      title          = "{Improving Planck calibration by including
                        frequency-dependent relativistic corrections}",
      journal        = "JCAP",
      volume         = "1509",
      year           = "2015",
      number         = "09",
      pages          = "050",
      doi            = "10.1088/1475-7516/2015/09/050",
      eprint         = "1504.04897",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1504.04897;%%"
}

@article{Paci:2013gs,
      author         = "Paci, F. and Gruppuso, A. and Finelli, F. and De Rosa, A.
                        and Mandolesi, N. and Natoli, P.",
      title          = "{Hemispherical power asymmetries in the WMAP 7-year
                        low-resolution temperature and polarization maps}",
      journal        = "Mon. Not. Roy. Astron. Soc.",
      volume         = "434",
      year           = "2013",
      pages          = "3071",
      doi            = "10.1093/mnras/stt1219",
      eprint         = "1301.5195",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1301.5195;%%"
}

@Article{Rassat:2013gla,
  Title                    = {{On Preferred Axes in WMAP Cosmic Microwave Background Data after Subtraction of the Integrated Sachs-Wolfe Effect}},
  Author                   = {Rassat, A. and Starck, J. -L.},
  Year                     = {2013},

  Archiveprefix            = {arXiv},
  Eprint                   = {1303.5051},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.5051;%%}
}

@Article{RassatStarck2013,
  author        = {Rassat, A. and Starck, J. -L.},
  title         = {{On Preferred Axes in WMAP Cosmic Microwave Background Data after Subtraction of the Integrated Sachs-Wolfe Effect}},
  year          = {2013},
  archiveprefix = {arXiv},
  eprint        = {1303.5051},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:1303.5051;%%},
  timestamp     = {2015.10.13},
}

@Article{Rassat:2013caa,
  Title                    = {{Removal of two large scale Cosmic Microwave Background anomalies after subtraction of the Integrated Sachs Wolfe effect}},
  Author                   = {Rassat, A. and Starck, J. -L. and Dupe, F. -X.},
  Year                     = {2013},

  Archiveprefix            = {arXiv},
  Eprint                   = {1303.4727},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1303.4727;%%}
}

@Article{RassatStarckDupe2013,
  author        = {Rassat, A. and Starck, J. -L. and Dupe, F. -X.},
  title         = {{Removal of two large scale Cosmic Microwave Background anomalies after subtraction of the Integrated Sachs Wolfe effect}},
  year          = {2013},
  archiveprefix = {arXiv},
  eprint        = {1303.4727},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:1303.4727;%%},
  timestamp     = {2015.10.13},
}

@Article{Rassat:2014yna,
  Title                    = {{Planck CMB Anomalies: Astrophysical and Cosmological Secondary Effects and the Curse of Masking}},
  Author                   = {Rassat, A. and Starck, J.-L. and Paykari, P. and Sureau, F. and Bobin, J.},
  Journal                  = {JCAP},
  Year                     = {2014},
  Pages                    = {006},
  Volume                   = {1408},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/1475-7516/2014/08/006},
  Doi                      = {10.1088/1475-7516/2014/08/006},
  Eprint                   = {1405.1844},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1405.1844;%%}
}

@Article{RassatStarckPaykariEtAl2014,
  author        = {Rassat, A. and Starck, J.-L. and Paykari, P. and Sureau, F. and Bobin, J.},
  title         = {{Planck CMB Anomalies: Astrophysical and Cosmological Secondary Effects and the Curse of Masking}},
  journal       = {JCAP},
  year          = {2014},
  volume        = {1408},
  pages         = {006},
  archiveprefix = {arXiv},
  doi           = {10.1088/1475-7516/2014/08/006},
  eprint        = {1405.1844},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph.CO},
  slaccitation  = {%%CITATION = ARXIV:1405.1844;%%},
  timestamp     = {2015.10.13},
}

@Article{Rath:2013yra,
  Title                    = {{Testing the Dipole Modulation Model in CMBR}},
  Author                   = {Rath, Pranati K. and Jain, Pankaj},
  Journal                  = {JCAP},
  Year                     = {2013},
  Pages                    = {014},
  Volume                   = {1312},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1088/1475-7516/2013/12/014},
  Doi                      = {10.1088/1475-7516/2013/12/014},
  Eprint                   = {1308.0924},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1308.0924;%%}
}

@Article{Sazonov:1999zp,
  Title                    = {{Microwave polarization in the direction of galaxy
 clusters induced by the CMB quadrupole anisotropy}},
  Author                   = {Sazonov, S.Y. and Sunyaev, R.A.},
  Journal                  = {Mon.Not.Roy.Astron.Soc.},
  Year                     = {1999},
  Pages                    = {765-772},
  Volume                   = {310},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1046/j.1365-8711.1999.02981.x},
  Eprint                   = {astro-ph/9903287},
  Primaryclass             = {astro-ph},
}

@Article{Schwarz:2004gk,
  Title                    = {{Is the low-l microwave background cosmic?}},
  Author                   = {Schwarz, Dominik J. and Starkman, Glenn D. and Huterer,
 Dragan and Copi, Craig J.},
  Journal                  = {Phys.Rev.Lett.},
  Year                     = {2004},
  Pages                    = {221301},
  Volume                   = {93},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1103/PhysRevLett.93.221301},
  Eprint                   = {astro-ph/0403353},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Reportnumber             = {CERN-PH-TH-2004-052},
  Timestamp                = {2015.10.13}
}

@ARTICLE{Sievers:2013wk,
   author = {{Sievers}, J.~L. and {Hlozek}, R.~A. and {Nolta}, M.~R. and 
	{Acquaviva}, V. and {Addison}, G.~E. and {Ade}, P.~A.~R. and 
	{Aguirre}, P. and {Amiri}, M. and {Appel}, J.~W. and others},
    title = "{The Atacama Cosmology Telescope: cosmological parameters from three seasons of data}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1301.0824},
     year = 2013,
    month = oct,
   volume = 10,
      eid = {060},
    pages = {060},
      doi = {10.1088/1475-7516/2013/10/060},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...10..060S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Louis:2016ahn,
   author = {{Louis}, T. and {Grace}, E. and {Hasselfield}, M. and {Lungu}, M. and 
	{Maurin}, L. and {Addison}, G.~E. and {Ade}, P.~A.~R. and {Aiola}, S. and 
	{Allison}, R. and others},
    title = "{The Atacama Cosmology Telescope: Two-Season ACTPol Spectra and Parameters}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.02360},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161002360L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Fixsen:1998kq,
      author         = "Fixsen, D. J. and Dwek, E. and Mather, John C. and
                        Bennett, C. L. and Shafer, R. A.",
      title          = "{The Spectrum of the extragalactic far infrared
                        background from the COBE FIRAS observations}",
      journal        = "Astrophys. J.",
      volume         = "508",
      year           = "1998",
      pages          = "123",
      doi            = "10.1086/306383",
      eprint         = "astro-ph/9803021",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "COBE-PREPRINT-#98-05",
      SLACcitation   = "%%CITATION = ASTRO-PH/9803021;%%"
}

@article{Zaldarriaga:1996xe,
      author         = "Zaldarriaga, Matias and Seljak, Uros",
      title          = "{An all sky analysis of polarization in the microwave
                        background}",
      journal        = "Phys. Rev.",
      volume         = "D55",
      year           = "1997",
      pages          = "1830-1840",
      doi            = "10.1103/PhysRevD.55.1830",
      eprint         = "astro-ph/9609170",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9609170;%%"
}

@Article{Spergel:2003cb,
  Title                    = {{First year Wilkinson Microwave Anisotropy Probe (WMAP) observations: Determination of cosmological parameters}},
  Author                   = {Spergel, D.N. and others},
  Journal                  = {Astrophys.J.Suppl.},
  Year                     = {2003},
  Pages                    = {175-194},
  Volume                   = {148},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1086/377226},
  Collaboration            = {WMAP},
  Doi                      = {10.1086/377226},
  Eprint                   = {astro-ph/0302209},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0302209;%%}
}

@Article{Spergelothers2003,
  author        = {Spergel, D.N. and others},
  title         = {{First year Wilkinson Microwave Anisotropy Probe (WMAP) observations: Determination of cosmological parameters}},
  journal       = {Astrophys.J.Suppl.},
  year          = {2003},
  volume        = {148},
  pages         = {175-194},
  archiveprefix = {arXiv},
  collaboration = {WMAP},
  doi           = {10.1086/377226},
  eprint        = {astro-ph/0302209},
  owner         = {Miguel Quartin},
  primaryclass  = {astro-ph},
  slaccitation  = {%%CITATION = ASTRO-PH/0302209;%%},
  timestamp     = {2015.10.13},
}

@Article{Sunyaev:2013coa,
  Title                    = {{Motion induced second order temperature and y-type
 anisotropies after the subtraction of linear dipole in the
 CMB maps}},
  Author                   = {Sunyaev, Rashid A. and Khatri, Rishi},
  Journal                  = {JCAP},
  Year                     = {2013},
  Pages                    = {012},
  Volume                   = {1303},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/1475-7516/2013/03/012},
  Eprint                   = {1302.6571},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1302.6571;%%}
}

@Article{Tegmark:2003ve,
  Title                    = {{A high resolution foreground cleaned CMB map from WMAP}},
  Author                   = {Tegmark, Max and de Oliveira-Costa, Angelica and
 Hamilton, Andrew},
  Journal                  = {Phys.Rev.},
  Year                     = {2003},
  Pages                    = {123523},
  Volume                   = {D68},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1103/PhysRevD.68.123523},
  Eprint                   = {astro-ph/0302496},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ASTRO-PH/0302496;%%},
  Timestamp                = {2015.10.13}
}

@Article{Tristram:2011gq,
  Title                    = {{Iterative destriping and photometric calibration for Planck-HFI, polarized, multi-detector map-making}},
  Author                   = {Tristram, M. and Filliard, C. and Perdereau, O. and Plaszczynski, S. and Stompor, R. and others},
  Journal                  = {Astron.Astrophys.},
  Year                     = {2011},
  Pages                    = {A88},
  Volume                   = {534},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1051/0004-6361/201116871},
  Doi                      = {10.1051/0004-6361/201116871},
  Eprint                   = {1103.2281},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1103.2281;%%}
}

@Article{Trotta:2008qt,
  Title                    = {{Bayes in the sky: Bayesian inference and model selection in cosmology}},
  Author                   = {Trotta, Roberto},
  Journal                  = {Contemp.Phys.},
  Year                     = {2008},
  Pages                    = {71-104},
  Volume                   = {49},

  Archiveprefix            = {arXiv},
  Bdsk-url-1               = {http://dx.doi.org/10.1080/00107510802066753},
  Doi                      = {10.1080/00107510802066753},
  Eprint                   = {0803.4089},
  Primaryclass             = {astro-ph},
  Slaccitation             = {%%CITATION = ARXIV:0803.4089;%%}
}

@Article{Yoho:2012am,
  Title                    = {{Real Space Approach to CMB deboosting}},
  Author                   = {Yoho, Amanda and Copi, Craig J. and Starkman, Glenn D. and Pereira, Thiago S.},
  Year                     = {2012},

  Archiveprefix            = {arXiv},
  Eprint                   = {1211.6756},
  Primaryclass             = {astro-ph.CO},
  Slaccitation             = {%%CITATION = ARXIV:1211.6756;%%}
}

@Article{Zonca:2010fx,
  Title                    = {{Planck-LFI radiometers' spectral response}},
  Author                   = {Zonca, A and Franceschet, C and Battaglia, P and Villa, F
 and Mennella, A and others},
  Journal                  = {JINST},
  Year                     = {2009},
  Pages                    = {T12010},
  Volume                   = {4},

  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/1748-0221/4/12/T12010},
  Eprint                   = {1001.4589},
  Owner                    = {Miguel Quartin},
  Primaryclass             = {astro-ph.IM},
  Slaccitation             = {%%CITATION = ARXIV:1001.4589;%%},
  Timestamp                = {2015.10.13}
}

@Article{cosmostat-webpage,
  Note                     = {\url{http://www.cosmostat.org/}}
}

@Comment{jabref-meta: databaseType:bibtex;}


@ARTICLE{Acero2015,
   author = {{Acero}, F. and {Ackermann}, M. and {Ajello}, M. and {Albert}, A. and
	{Atwood}, W.~B. and {Axelsson}, M. and {Baldini}, L. and {Ballet}, J. and
	 and {Fermi-LAT Collaboration}
	},
    title = "{Fermi Large Area Telescope Third Source Catalog}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1501.02003},
 primaryClass = "astro-ph.HE",
 keywords = {catalogs, gamma rays: general},
     year = 2015,
    month = jun,
   volume = 218,
      eid = {23},
    pages = {23},
      doi = {10.1088/0067-0049/218/2/23},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..218...23A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alberts2014,
   author = {{Alberts}, S. and {Pope}, A. and {Brodwin}, M. and {Atlee}, D.~W. and
	{Lin}, Y.-T. and {Dey}, A. and {Eisenhardt}, P.~R.~M. and {Gettings}, D.~P. and
	{Gonzalez}, A.~H. and {Jannuzi}, B.~T. and {Mancone}, C.~L. and
	{Moustakas}, J. and {Snyder}, G.~F. and {Stanford}, S.~A. and
	{Stern}, D. and {Weiner}, B.~J. and {Zeimann}, G.~R.},
    title = "{The evolution of dust-obscured star formation activity in galaxy clusters relative to the field over the last 9 billion years}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.6040},
 keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: high-redshift, infrared: galaxies},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {437-457},
      doi = {10.1093/mnras/stt1897},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437..437A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alberts2016,
   author = {{Alberts}, S. and {Pope}, A. and {Brodwin}, M. and {Chung}, S.~M. and
	{Cybulski}, R. and {Dey}, A. and {Eisenhardt}, P. and {Galametz}, A. and
	{Gonzalez}, A. and {Jannuzi}, B. and {Stanford}, S.~A. and {Snyder}, G. and
	{Stern}, D. and {Zeimann}, G.},
    title = "{Star Formation and AGN Activity in Galaxy Clusters from $z=1-2$: a Multi-wavelength Analysis Featuring $Herschel$/PACS}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1604.03564},
 keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160403564A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Amendola2016,
   author = {{Amendola}, L. and {Appleby}, S. and {Avgoustidis}, A. and {Bacon}, D. and
	{Baker}, T. and {Baldi}, M. and {Bartolo}, N. and {Blanchard}, A. and
	{Bonvin}, C. and {Borgani}, S. and {Branchini}, E. and {Burrage}, C. and
	{Camera}, S. and {Carbone}, C. and {Casarini}, L. and {Cropper}, M. and
	{de Rham}, C. and {Dietrich}, J.~P. and {Di Porto}, C. and {Durrer}, R. and
	{Ealet}, A. and {Ferreira}, P.~G. and {Finelli}, F. and {Garcia-Bellido}, J. and
	{Giannantonio}, T. and {Guzzo}, L. and {Heavens}, A. and {Heisenberg}, L. and
	{Heymans}, C. and {Hoekstra}, H. and {Hollenstein}, L. and {Holmes}, R. and
	{Horst}, O. and {Hwang}, Z. and {Jahnke}, K. and {Kitching}, T.~D. and
	{Koivisto}, T. and {Kunz}, M. and {La Vacca}, G. and {Linder}, E. and
	{March}, M. and {Marra}, V. and {Martins}, C. and {Majerotto}, E. and
	{Markovic}, D. and {Marsh}, D. and {Marulli}, F. and {Massey}, R. and
	{Mellier}, Y. and {Montanari}, F. and {Mota}, D.~F. and {Nunes}, N.~J. and
	{Percival}, W. and {Pettorino}, V. and {Porciani}, C. and {Quercellini}, C. and
	{Read}, J. and {Rinaldi}, M. and {Sapone}, D. and {Sawicki}, I. and
	{Scaramella}, R. and {Skordis}, C. and {Simpson}, F. and {Taylor}, A. and
	{Thomas}, S. and {Trotta}, R. and {Verde}, L. and {Vernizzi}, F. and
	{Vollmer}, A. and {Wang}, Y. and {Weller}, J. and {Zlosnik}, T.
	},
    title = "{Cosmology and Fundamental Physics with the Euclid Satellite}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1606.00180},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160600180A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Aversa2015,
   author = {{Aversa}, R. and {Lapi}, A. and {de Zotti}, G. and {Shankar}, F. and
	{Danese}, L.},
    title = "{Black Hole and Galaxy Coevolution from Continuity Equation and Abundance Matching}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1507.07318},
 keywords = {black hole physics, galaxies: evolution, galaxies: formation, methods: analytical, quasars: supermassive black holes},
     year = 2015,
    month = sep,
   volume = 810,
      eid = {74},
    pages = {74},
      doi = {10.1088/0004-637X/810/1/74},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...810...74A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baes2014,
   author = {{Baes}, M. and {Herranz}, D. and {Bianchi}, S. and {Ciesla}, L. and
	{Clemens}, M. and {De Zotti}, G. and {Allaert}, F. and {Auld}, R. and
	{Bendo}, G.~J. and {Boquien}, M. and {Boselli}, A. and {Clements}, D.~L. and
	{Cortese}, L. and {Davies}, J.~I. and {De Looze}, I. and {di Serego Alighieri}, S. and
	{Fritz}, J. and {Gentile}, G. and {Gonz{\'a}lez-Nuevo}, J. and
	{Hughes}, T. and {Smith}, M.~W.~L. and {Verstappen}, J. and
	{Viaene}, S. and {Vlahakis}, C.},
    title = "{The Herschel Virgo Cluster Survey. XV. Planck submillimetre sources in the Virgo Cluster}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1401.1017},
 keywords = {galaxies: ISM, submillimeter: galaxies},
     year = 2014,
    month = feb,
   volume = 562,
      eid = {A106},
    pages = {A106},
      doi = {10.1051/0004-6361/201322384},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...562A.106B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Balashev2015,
   author = {{Balashev}, S.~A. and {Kholupenko}, E.~E. and {Chluba}, J. and
	{Ivanchik}, A.~V. and {Varshalovich}, D.~A.},
    title = "{Spectral Distortions of the CMB Dipole}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1505.06028},
 keywords = {cosmic background radiation},
     year = 2015,
    month = sep,
   volume = 810,
      eid = {131},
    pages = {131},
      doi = {10.1088/0004-637X/810/2/131},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...810..131B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Battye2011,
   author = {{Battye}, R.~A. and {Browne}, I.~W.~A. and {Peel}, M.~W. and
	{Jackson}, N.~J. and {Dickinson}, C.},
    title = "{Statistical properties of polarized radio sources at high frequency and their impact on cosmic microwave background polarization measurements}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.5846},
 keywords = {polarization, catalogues, galaxies: general, radio continuum: galaxies, cosmic microwave background},
     year = 2011,
    month = may,
   volume = 413,
    pages = {132-148},
      doi = {10.1111/j.1365-2966.2010.18115.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413..132B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beck2016,
   author = {{Beck}, R. and {Dobos}, L. and {Budav{\'a}ri}, T. and {Szalay}, A.~S. and
	{Csabai}, I.},
    title = "{Photometric redshifts for the SDSS Data Release 12}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1603.09708},
 keywords = {methods: data analysis, techniques: photometric, catalogues, galaxies: distances and redshifts},
     year = 2016,
    month = aug,
   volume = 460,
    pages = {1371-1381},
      doi = {10.1093/mnras/stw1009},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460.1371B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bleem2015,
   author = {{Bleem}, L.~E. and {Stalder}, B. and {de Haan}, T. and {Aird}, K.~A. and
	{Allen}, S.~W. and {Applegate}, D.~E. and {Ashby}, M.~L.~N. and
	{Bautz}, M. and {Bayliss}, M. and {Benson}, B.~A. and {Bocquet}, S. and
	{Brodwin}, M. and {Carlstrom}, J.~E. and {Chang}, C.~L. and et al.
	},
    title = "{Galaxy Clusters Discovered via the Sunyaev-Zel'dovich Effect in the 2500-Square-Degree SPT-SZ Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1409.0850},
 keywords = {cosmology: observations, galaxies: clusters: individual, large-scale structure of universe},
     year = 2015,
    month = feb,
   volume = 216,
      eid = {27},
    pages = {27},
      doi = {10.1088/0067-0049/216/2/27},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..216...27B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BertinArnouts1996,
   author = {{Bertin}, E. and {Arnouts}, S.},
    title = "{SExtractor: Software for source extraction.}",
  journal = {\aaps},
 keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
     year = 1996,
    month = jun,
   volume = 117,
    pages = {393-404},
      doi = {10.1051/aas:1996164},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..117..393B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bilicki2014a,
   author = {{Bilicki}, M. and {Peacock}, J.~A. and {Jarrett}, T.~H. and
	{Cluver}, M.~E. and {Steward}, L.},
    title = "{Mapping the Cosmic Web with the largest all-sky surveys}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1408.0799},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2014,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1408.0799B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bilicki2014,
   author = {{Bilicki}, M. and {Jarrett}, T.~H. and {Peacock}, J.~A. and
	{Cluver}, M.~E. and {Steward}, L.},
    title = "{Two Micron All Sky Survey Photometric Redshift Catalog: A Comprehensive Three-dimensional Census of the Whole Sky}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1311.5246},
 primaryClass = "astro-ph.CO",
 keywords = {catalogs, galaxies: distances and redshifts, large-scale structure of universe, methods: data analysis, methods: statistical, surveys },
     year = 2014,
    month = jan,
   volume = 210,
      eid = {9},
    pages = {9},
      doi = {10.1088/0067-0049/210/1/9},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..210....9B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bilicki2015,
   author = {{Bilicki}, M.},
    title = "{Cosmology with all-sky surveys}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1512.05198},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2015,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151205198B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bohringer2013,
   author = {{B{\"o}hringer}, H. and {Chon}, G. and {Collins}, C.~A. and
	{Guzzo}, L. and {Nowak}, N. and {Bobrovskyi}, S.},
    title = "{The extended ROSAT-ESO flux limited X-ray galaxy cluster survey (REFLEX II) II. Construction and properties of the survey}",
  journal = {\aap},
 keywords = {galaxies: clusters: general, large-scale structure of Universe, X-rays: galaxies: clusters},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201220722},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A..30B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brodwin2013,
   author = {{Brodwin}, M. and {Stanford}, S.~A. and {Gonzalez}, A.~H. and
	{Zeimann}, G.~R. and {Snyder}, G.~F. and {Mancone}, C.~L. and
	{Pope}, A. and {Eisenhardt}, P.~R. and {Stern}, D. and {Alberts}, S. and
	{Ashby}, M.~L.~N. and {Brown}, M.~J.~I. and {Chary}, R.-R. and
	{Dey}, A. and {Galametz}, A. and {Gettings}, D.~P. and {Jannuzi}, B.~T. and
	{Miller}, E.~D. and {Moustakas}, J. and {Moustakas}, L.~A.},
    title = "{The Era of Star Formation in Galaxy Clusters}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1310.6039},
 keywords = {galaxies: clusters: general, galaxies: distances and redshifts, galaxies: evolution, galaxies: formation, galaxies: starburst },
     year = 2013,
    month = dec,
   volume = 779,
      eid = {138},
    pages = {138},
      doi = {10.1088/0004-637X/779/2/138},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779..138B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Cai2013,
   author = {{Cai}, Z.-Y. and {Lapi}, A. and {Xia}, J.-Q. and {De Zotti}, G. and
	{Negrello}, M. and {Gruppioni}, C. and {Rigby}, E. and {Castex}, G. and
	{Delabrouille}, J. and {Danese}, L.},
    title = "{A Hybrid Model for the Evolution of Galaxies and Active Galactic Nuclei in the Infrared}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1303.2335},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: high-redshift, submillimeter: galaxies },
     year = 2013,
    month = may,
   volume = 768,
      eid = {21},
    pages = {21},
      doi = {10.1088/0004-637X/768/1/21},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768...21C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Canameras2015,
   author = {{Ca{\~n}ameras}, R. and {Nesvadba}, N.~P.~H. and {Guery}, D. and
	{McKenzie}, T. and {K{\"o}nig}, S. and {Petitpas}, G. and {Dole}, H. and
	{Frye}, B. and {Flores-Cacho}, I. and {Montier}, L. and {Negrello}, M. and
	{Beelen}, A. and {Boone}, F. and {Dicken}, D. and {Lagache}, G. and
	{Le Floc'h}, E. and {Altieri}, B. and {B{\'e}thermin}, M. and
	{Chary}, R. and {de Zotti}, G. and {Giard}, M. and {Kneissl}, R. and
	{Krips}, M. and {Malhotra}, S. and {Martinache}, C. and {Omont}, A. and
	{Pointecouteau}, E. and {Puget}, J.-L. and {Scott}, D. and {Soucail}, G. and
	{Valtchanov}, I. and {Welikala}, N. and {Yan}, L.},
    title = "{Planck's dusty GEMS: The brightest gravitationally lensed galaxies discovered with the Planck all-sky survey}",
  journal = {\aap},
 keywords = {galaxies: high-redshift, galaxies: star formation, galaxies: starburst, submillimeter: galaxies, gravitational lensing: strong, galaxies: formation},
     year = 2015,
    month = sep,
   volume = 581,
      eid = {A105},
    pages = {A105},
      doi = {10.1051/0004-6361/201425128},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...581A.105C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Claeskens2006,
   author = {{Claeskens}, J.-F. and {Smette}, A. and {Vandenbulcke}, L. and
	{Surdej}, J.},
    title = "{Identification and redshift determination of quasi-stellar objects with medium-band photometry: application to Gaia}",
  journal = {\mnras},
 keywords = {methods: data analysis, quasars: general},
     year = 2006,
    month = apr,
   volume = 367,
    pages = {879-904},
      doi = {10.1111/j.1365-2966.2006.10024.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367..879C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clemens2013,
   author = {{Clemens}, M.~S. and {Negrello}, M. and {De Zotti}, G. and {Gonzalez-Nuevo}, J. and
	{Bonavera}, L. and {Cosco}, G. and {Guarese}, G. and {Boaretto}, L. and
	{Salucci}, P. and {Baccigalupi}, C. and {Clements}, D.~L. and
	{Danese}, L. and {Lapi}, A. and {Mandolesi}, N. and {Partridge}, R.~B. and
	{Perrotta}, F. and {Serjeant}, S. and {Scott}, D. and {Toffolatti}, L.
	},
    title = "{Dust and star formation properties of a complete sample of local galaxies drawn from the Planck Early Release Compact Source Catalogue}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.1647},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: general, galaxies: luminosity function, mass function, infrared: galaxies, submillimetre: galaxies},
     year = 2013,
    month = jul,
   volume = 433,
    pages = {695-711},
      doi = {10.1093/mnras/stt760},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433..695C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clements2014,
   author = {{Clements}, D.~L. and {Braglia}, F.~G. and {Hyde}, A.~K. and
	{P{\'e}rez-Fournon}, I. and {Bock}, J. and {Cava}, A. and {Chapman}, S. and
	{Conley}, A. and {Cooray}, A. and {Farrah}, D. and {Gonz{\'a}lez Solares}, E.~A. and
	{Marchetti}, L. and {Marsden}, G. and {Oliver}, S.~J. and {Roseboom}, I.~G. and
	{Schulz}, B. and {Smith}, A.~J. and {Vaccari}, M. and {Vieira}, J. and
	{Viero}, M. and {Wang}, L. and {Wardlow}, J. and {Zemcov}, M. and
	{de Zotti}, G.},
    title = "{Herschel Multitiered Extragalactic Survey: clusters of dusty galaxies uncovered by Herschel and Planck}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1311.5758},
 keywords = {galaxies: high redshift, galaxies: starburst, submillimetre: galaxies},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {1193-1211},
      doi = {10.1093/mnras/stt2253},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.1193C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Clements2016,
   author = {{Clements}, D.~L. and {Braglia}, F. and {Petitpas}, G. and {Greenslade}, J. and
	{Cooray}, A. and {Valiante}, E. and {De Zotti}, G. and {O'Halloran}, B. and
	{Holdship}, J. and {Morris}, B. and {Herranz}, I.~P.-F.~D. and
	{Riechers}, D. and {Baes}, M. and {Bremer}, M. and {Bourne}, N. and
	{Dannerbauer}, H. and {Dariush}, A. and {Dunne}, L. and {Eales}, S. and
	{Fritz}, J. and {Gonzalez-Nuevo}, J. and {Hopwood}, R. and {Ibar}, E. and
	{Ivison}, R.~J. and {Leeuw}, L.~L. and {Maddox}, S. and {Negrello}, M.~J.~M.~M. and
	{Omont}, A. and {Oteo}, I. and {Serjeant}, S. and {Valtchanov}, I. and
	{Vieira}, J.~D. and {Wardlow}, J. and {van der Werf}, P.},
    title = "{H-ATLAS: A Candidate High Redshift Cluster/Protocluster of Star-Forming Galaxies}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1605.06433},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160506433C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Combes2012,
   author = {{Combes}, F. and {Rex}, M. and {Rawle}, T.~D. and {Egami}, E. and
	{Boone}, F. and {Smail}, I. and {Richard}, J. and {Ivison}, R.~J. and
	{Gurwell}, M. and {Casey}, C.~M. and {Omont}, A. and {Berciano Alba}, A. and
	{Dessauges-Zavadsky}, M. and {Edge}, A.~C. and {Fazio}, G.~G. and
	{Kneib}, J.-P. and {Okabe}, N. and {Pell{\'o}}, R. and {P{\'e}rez-Gonz{\'a}lez}, P.~G. and
	{Schaerer}, D. and {Smith}, G.~P. and {Swinbank}, A.~M. and
	{van der Werf}, P.},
    title = "{A bright z = 5.2 lensed submillimeter galaxy in the field of Abell 773. HLSJ091828.6+514223}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1201.2908},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: ISM, infrared: galaxies, submillimeter: galaxies, galaxies: individual: HLSJ091828.6+514223},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {L4},
    pages = {L4},
      doi = {10.1051/0004-6361/201118750},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538L...4C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cutini2014,
   author = {{Cutini}, S. and {Ciprini}, S. and {Orienti}, M. and {Tramacere}, A. and
	{D'Ammando}, F. and {Verrecchia}, F. and {Polenta}, G. and {Carrasco}, L. and
	{D'Elia}, V. and {Giommi}, P. and {Gonz{\'a}lez-Nuevo}, J. and
	{Grandi}, P. and {Harrison}, D. and {Hays}, E. and {Larsson}, S. and
	{L{\"a}hteenm{\"a}ki}, A. and {Le{\'o}n-Tavares}, J. and {L{\'o}pez-Caniego}, M. and
	{Natoli}, P. and {Ojha}, R. and {Partridge}, B. and {Porras}, A. and
	{Reyes}, L. and {Recillas}, E. and {Torresi}, E.},
    title = "{Radio-gamma-ray connection and spectral evolution in 4C +49.22 (S4 1150+49): the Fermi, Swift and Planck view}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.8101},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: jets, quasars: general, quasars: individual: 4C +49.22, gamma-rays: galaxies, X-rays: galaxies},
     year = 2014,
    month = dec,
   volume = 445,
    pages = {4316-4334},
      doi = {10.1093/mnras/stu2011},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445.4316C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DaneseDeZotti1981,
   author = {{Danese}, L. and {de Zotti}, G.},
    title = "{Dipole anisotropy and distortions of the spectrum of the cosmic microwave background}",
  journal = {\aap},
 keywords = {Astronomical Spectroscopy, Background Radiation, Microwave Emission, Anisotropic Media, Compton Effect, Dipoles},
     year = 1981,
    month = feb,
   volume = 94,
    pages = {L33},
   adsurl = {http://adsabs.harvard.edu/abs/1981A%26A....94L..33D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dawson2016,
   author = {{Dawson}, K.~S. and {Kneib}, J.-P. and {Percival}, W.~J. and
	{Alam}, S. and {Albareti}, F.~D. and {Anderson}, S.~F. and {Armengaud}, E. and
	{Aubourg}, {\'E}. and {Bailey}, S. and {Bautista}, J.~E. and
	{Berlind}, A.~A. and {Bershady}, M.~A. and {Beutler}, F. and
	{Bizyaev}, D. and {Blanton}, M.~R. and {Blomqvist}, M. and {Bolton}, A.~S. and
	{Bovy}, J. and {Brandt}, W.~N. and {Brinkmann}, J. and {Brownstein}, J.~R. and
	{Burtin}, E. and {Busca}, N.~G. and {Cai}, Z. and {Chuang}, C.-H. and
	{Clerc}, N. and {Comparat}, J. and {Cope}, F. and {Croft}, R.~A.~C. and
	{Cruz-Gonzalez}, I. and {da Costa}, L.~N. and {Cousinou}, M.-C. and
	{Darling}, J. and {de la Macorra}, A. and {de la Torre}, S. and
	{Delubac}, T. and {du Mas des Bourboux}, H. and {Dwelly}, T. and
	{Ealet}, A. and {Eisenstein}, D.~J. and {Eracleous}, M. and
	{Escoffier}, S. and {Fan}, X. and {Finoguenov}, A. and {Font-Ribera}, A. and
	{Frinchaboy}, P. and {Gaulme}, P. and {Georgakakis}, A. and
	{Green}, P. and {Guo}, H. and {Guy}, J. and {Ho}, S. and {Holder}, D. and
	{Huehnerhoff}, J. and {Hutchinson}, T. and {Jing}, Y. and {Jullo}, E. and
	{Kamble}, V. and {Kinemuchi}, K. and {Kirkby}, D. and {Kitaura}, F.-S. and
	{Klaene}, M.~A. and {Laher}, R.~R. and {Lang}, D. and {Laurent}, P. and
	{Le Goff}, J.-M. and {Li}, C. and {Liang}, Y. and {Lima}, M. and
	{Lin}, Q. and {Lin}, W. and {Lin}, Y.-T. and {Long}, D.~C. and
	{Lundgren}, B. and {MacDonald}, N. and {Geimba Maia}, M.~A. and
	{Malanushenko}, E. and {Malanushenko}, V. and {Mariappan}, V. and
	{McBride}, C.~K. and {McGreer}, I.~D. and {M{\'e}nard}, B. and
	{Merloni}, A. and {Meza}, A. and {Montero-Dorta}, A.~D. and
	{Muna}, D. and {Myers}, A.~D. and {Nandra}, K. and {Naugle}, T. and
	{Newman}, J.~A. and {Noterdaeme}, P. and {Nugent}, P. and {Ogando}, R. and
	{Olmstead}, M.~D. and {Oravetz}, A. and {Oravetz}, D.~J. and
	{Padmanabhan}, N. and {Palanque-Delabrouille}, N. and {Pan}, K. and
	{Parejko}, J.~K. and {P{\^a}ris}, I. and {Peacock}, J.~A. and
	{Petitjean}, P. and {Pieri}, M.~M. and {Pisani}, A. and {Prada}, F. and
	{Prakash}, A. and {Raichoor}, A. and {Reid}, B. and {Rich}, J. and
	{Ridl}, J. and {Rodriguez-Torres}, S. and {Carnero Rosell}, A. and
	{Ross}, A.~J. and {Rossi}, G. and {Ruan}, J. and {Salvato}, M. and
	{Sayres}, C. and {Schneider}, D.~P. and {Schlegel}, D.~J. and
	{Seljak}, U. and {Seo}, H.-J. and {Sesar}, B. and {Shandera}, S. and
	{Shu}, Y. and {Slosar}, A. and {Sobreira}, F. and {Streblyanska}, A. and
	{Suzuki}, N. and {Taylor}, D. and {Tao}, C. and {Tinker}, J.~L. and
	{Tojeiro}, R. and {Vargas-Maga{\~n}a}, M. and {Wang}, Y. and
	{Weaver}, B.~A. and {Weinberg}, D.~H. and {White}, M. and {Wood-Vasey}, W.~M. and
	{Yeche}, C. and {Zhai}, Z. and {Zhao}, C. and {Zhao}, G.-b. and
	{Zheng}, Z. and {Ben Zhu}, G. and {Zou}, H.},
    title = "{The SDSS-IV Extended Baryon Oscillation Spectroscopic Survey: Overview and Early Data}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1508.04473},
 keywords = {cosmology: observations, surveys},
     year = 2016,
    month = feb,
   volume = 151,
      eid = {44},
    pages = {44},
      doi = {10.3847/0004-6256/151/2/44},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....151...44D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Delabrouille2013,
   author = {{Delabrouille}, J. and {Betoule}, M. and {Melin}, J.-B. and
	{Miville-Desch{\^e}nes}, M.-A. and {Gonzalez-Nuevo}, J. and
	{Le Jeune}, M. and {Castex}, G. and {de Zotti}, G. and {Basak}, S. and
	{Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and
	{Bernard}, J.-P. and {Bouchet}, F.~R. and {Clements}, D.~L. and
	{da Silva}, A. and {Dickinson}, C. and {Dodu}, F. and {Dolag}, K. and
	{Elsner}, F. and {Fauvet}, L. and {Fa{\"y}}, G. and {Giardino}, G. and
	{Leach}, S. and {Lesgourgues}, J. and {Liguori}, M. and {Mac{\'{\i}}as-P{\'e}rez}, J.~F. and
	{Massardi}, M. and {Matarrese}, S. and {Mazzotta}, P. and {Montier}, L. and
	{Mottet}, S. and {Paladini}, R. and {Partridge}, B. and {Piffaretti}, R. and
	{Prezeau}, G. and {Prunet}, S. and {Ricciardi}, S. and {Roman}, M. and
	{Schaefer}, B. and {Toffolatti}, L.},
    title = "{The pre-launch Planck Sky Model: a model of sky emission at submillimetre to centimetre wavelengths}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1207.3675},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: miscellaneous, radio continuum: general, submillimeter: general, cosmic background radiation, ISM: general, galaxies: general},
     year = 2013,
    month = may,
   volume = 553,
      eid = {A96},
    pages = {A96},
      doi = {10.1051/0004-6361/201220019},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...553A..96D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeZotti2005,
   author = {{de Zotti}, G. and {Ricci}, R. and {Mesa}, D. and {Silva}, L. and
	{Mazzotta}, P. and {Toffolatti}, L. and {Gonz{\'a}lez-Nuevo}, J.
	},
    title = "{Predictions for high-frequency radio surveys of extragalactic sources}",
  journal = {\aap},
   eprint = {astro-ph/0410709},
 keywords = {galaxies: active, galaxies: quasars: general, galaxies: BL Lacertae objects: general, radio continuum: general},
     year = 2005,
    month = mar,
   volume = 431,
    pages = {893-903},
      doi = {10.1051/0004-6361:20042108},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...431..893D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeZotti2010,
   author = {{de Zotti}, G. and {Massardi}, M. and {Negrello}, M. and {Wall}, J.
	},
    title = "{Radio and millimeter continuum surveys and their astrophysical implications}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {0908.1896},
 keywords = {Radio continuum: galaxies, Galaxies: active, Galaxies: starburst, Galaxies: statistics, Quasars: general},
     year = 2010,
    month = feb,
   volume = 18,
    pages = {1-65},
      doi = {10.1007/s00159-009-0026-0},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26ARv..18....1D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeZotti2015,
   author = {{De Zotti}, G. and {Castex}, G. and {Gonz{\'a}lez-Nuevo}, J. and
	{Lopez-Caniego}, M. and {Negrello}, M. and {Cai}, Z.-Y. and
	{Clemens}, M. and {Delabrouille}, J. and {Herranz}, D. and {Bonavera}, L. and
	{Melin}, J.-B. and {Tucci}, M. and {Serjeant}, S. and {Bilicki}, M. and
	{Andreani}, P. and {Clements}, D.~L. and {Toffolatti}, L. and
	{Roukema}, B.~F.},
    title = "{Extragalactic sources in Cosmic Microwave Background maps}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1501.02170},
     year = 2015,
    month = jun,
   volume = 6,
      eid = {018},
    pages = {018},
      doi = {10.1088/1475-7516/2015/06/018},
   adsurl = {http://adsabs.harvard.edu/abs/2015JCAP...06..018D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dole2006,
   author = {{Dole}, H. and {Lagache}, G. and {Puget}, J.-L. and {Caputi}, K.~I. and
	{Fern{\'a}ndez-Conde}, N. and {Le Floc'h}, E. and {Papovich}, C. and
	{P{\'e}rez-Gonz{\'a}lez}, P.~G. and {Rieke}, G.~H. and {Blaylock}, M.
	},
    title = "{The cosmic infrared background resolved by Spitzer. Contributions of mid-infrared galaxies to the far-infrared background}",
  journal = {\aap},
   eprint = {astro-ph/0603208},
     year = 2006,
    month = may,
   volume = 451,
    pages = {417-429},
      doi = {10.1051/0004-6361:20054446},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...451..417D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dore2014,
   author = {{Dor{\'e}}, O. and {Bock}, J. and {Ashby}, M. and {Capak}, P. and
	{Cooray}, A. and {de Putter}, R. and {Eifler}, T. and {Flagey}, N. and
	{Gong}, Y. and {Habib}, S. and {Heitmann}, K. and {Hirata}, C. and
	{Jeong}, W.-S. and {Katti}, R. and {Korngut}, P. and {Krause}, E. and
	{Lee}, D.-H. and {Masters}, D. and {Mauskopf}, P. and {Melnick}, G. and
	{Mennesson}, B. and {Nguyen}, H. and {{\"O}berg}, K. and {Pullen}, A. and
	{Raccanelli}, A. and {Smith}, R. and {Song}, Y.-S. and {Tolls}, V. and
	{Unwin}, S. and {Venumadhav}, T. and {Viero}, M. and {Werner}, M. and
	{Zemcov}, M.},
    title = "{Cosmology with the SPHEREX All-Sky Spectral Survey}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.4872},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.4872D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Eales2015,
   author = {{Eales}, S.~A.},
    title = "{Practical cosmology with lenses}",
  journal = {\mnras},
 keywords = {galaxies: high-redshift, cosmological parameters, cosmology: observations, dark matter, submillimetre: galaxies},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {3224-3234},
      doi = {10.1093/mnras/stu2214},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.3224E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Fixsen1998,
   author = {{Fixsen}, D.~J. and {Dwek}, E. and {Mather}, J.~C. and {Bennett}, C.~L. and
	{Shafer}, R.~A.},
    title = "{The Spectrum of the Extragalactic Far-Infrared Background from the COBE FIRAS Observations}",
  journal = {\apj},
   eprint = {astro-ph/9803021},
 keywords = {COSMOLOGY: OBSERVATIONS, COSMOLOGY: DIFFUSE RADIATION, INFRARED: GENERAL, INTERPLANETARY MEDIUM, Cosmology: Observations, Cosmology: Diffuse Radiation, Infrared: General, Interplanetary Medium},
     year = 1998,
    month = nov,
   volume = 508,
    pages = {123-128},
      doi = {10.1086/306383},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...508..123F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FixsenKashlinsky2011,
   author = {{Fixsen}, D.~J. and {Kashlinsky}, A.},
    title = "{Probing the Universe's Tilt with the Cosmic Infrared Background Dipole}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.0901},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmology: observations, infrared: diffuse background},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/734/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734...61F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{FixsenMather2002,
   author = {{Fixsen}, D.~J. and {Mather}, J.~C.},
    title = "{The Spectral Results of the Far-Infrared Absolute Spectrophotometer Instrument on COBE}",
  journal = {\apj},
 keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations},
     year = 2002,
    month = dec,
   volume = 581,
    pages = {817-822},
      doi = {10.1086/344402},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...581..817F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FloresCacho2016,
   author = {{Flores-Cacho}, I. and {Pierini}, D. and {Soucail}, G. and {Montier}, L. and
	{Dole}, H. and {Pointecouteau}, E. and {Pell{\'o}}, R. and {Le Floc'h}, E. and
	{Nesvadba}, N. and {Lagache}, G. and {Guery}, D. and {Ca{\~n}ameras}, R.
	},
    title = "{Multi-wavelength characterisation of z \~{} 2 clustered, dusty star-forming galaxies discovered by Planck}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1510.01585},
 keywords = {cosmology: observations, galaxies: high-redshift, galaxies: clusters: general, galaxies: star formation, submillimeter: galaxies, large-scale structure of Universe},
     year = 2016,
    month = jan,
   volume = 585,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/201425226},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...585A..54F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GalluzziMassardi2016,
   author = {{Galluzzi}, V. and {Massardi}, M.
	},
    title = "{The polarimetric multi-frequency radio sources properties}",
  journal = {Int. J. Mod. Phys. D},
 keywords = {\ },
     year = 2016,
   volume = 25,
      eid = {\ },
    pages = {1640005},
      doi = {\ }
}

@ARTICLE{Giommi2012,
   author = {{Giommi}, P. and {Polenta}, G. and {L{\"a}hteenm{\"a}ki}, A. and
	{Thompson}, D.~J. and {Capalbi}, M. and {Cutini}, S. and {Gasparrini}, D. and
	{Gonz{\'a}lez-Nuevo}, J. and {Le{\'o}n-Tavares}, J. and {L{\'o}pez-Caniego}, M. and
	{Mazziotta}, M.~N. and et al.},
    title = "{Simultaneous Planck, Swift, and Fermi observations of X-ray and {$\gamma$}-ray selected blazars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1108.1114},
 primaryClass = "astro-ph.CO",
 keywords = {relativistic processes, BL Lacertae objects: general, quasars: general, galaxies: active},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A160},
    pages = {A160},
      doi = {10.1051/0004-6361/201117825},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A.160G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Glenn2010,
   author = {{Glenn}, J. and {Conley}, A. and {B{\'e}thermin}, M. and {Altieri}, B. and
	{Amblard}, A. and {Arumugam}, V. and {Aussel}, H. and {Babbedge}, T. and
	{Blain}, A. and {Bock}, J. and {Boselli}, A. and {Buat}, V. and
	{Castro-Rodr{\'{\i}}guez}, N. and {Cava}, A. and {Chanial}, P. and
	{Clements}, D.~L. and {Conversi}, L. and {Cooray}, A. and {Dowell}, C.~D. and
	{Dwek}, E. and {Eales}, S. and {Elbaz}, D. and {Ellsworth-Bowers}, T.~P. and
	{Fox}, M. and {Franceschini}, A. and {Gear}, W. and {Griffin}, M. and
	{Halpern}, M. and {Hatziminaoglou}, E. and {Ibar}, E. and {Isaak}, K. and
	{Ivison}, R.~J. and {Lagache}, G. and {Laurent}, G. and {Levenson}, L. and
	{Lu}, N. and {Madden}, S. and {Maffei}, B. and {Mainetti}, G. and
	{Marchetti}, L. and {Marsden}, G. and {Nguyen}, H.~T. and {O'Halloran}, B. and
	{Oliver}, S.~J. and {Omont}, A. and {Page}, M.~J. and {Panuzzo}, P. and
	{Papageorgiou}, A. and {Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and
	{Pohlen}, M. and {Rigopoulou}, D. and {Rizzo}, D. and {Roseboom}, I.~G. and
	{Rowan-Robinson}, M. and {Portal}, M.~S. and {Schulz}, B. and
	{Scott}, D. and {Seymour}, N. and {Shupe}, D.~L. and {Smith}, A.~J. and
	{Stevens}, J.~A. and {Symeonidis}, M. and {Trichas}, M. and
	{Tugwell}, K.~E. and {Vaccari}, M. and {Valtchanov}, I. and
	{Vieira}, J.~D. and {Vigroux}, L. and {Wang}, L. and {Ward}, R. and
	{Wright}, G. and {Xu}, C.~K. and {Zemcov}, M.},
    title = "{HerMES: deep galaxy number counts from a P(D) fluctuation analysis of SPIRE Science Demonstration Phase observations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1009.5675},
 keywords = {cosmology: observations, submillimetre: diffuse background, submillimetre: galaxies},
     year = 2010,
    month = nov,
   volume = 409,
    pages = {109-121},
      doi = {10.1111/j.1365-2966.2010.17781.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409..109G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{GonzalezNuevo2005,
   author = {{Gonz{\'a}lez-Nuevo}, J. and {Toffolatti}, L. and {Arg{\"u}eso}, F.
	},
    title = "{Predictions of the Angular Power Spectrum of Clustered Extragalactic Point Sources at Cosmic Microwave Background Frequencies from Flat and All-Sky Two-dimensional Simulations}",
  journal = {\apj},
   eprint = {astro-ph/0405553},
 keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Large-Scale Structure of Universe, Methods: Numerical},
     year = 2005,
    month = mar,
   volume = 621,
    pages = {1-14},
      doi = {10.1086/427425},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621....1G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GonzalezNuevo2006,
   author = {{Gonz{\'a}lez-Nuevo}, J. and {Arg{\"u}eso}, F. and {L{\'o}pez-Caniego}, M. and
	{Toffolatti}, L. and {Sanz}, J.~L. and {Vielva}, P. and {Herranz}, D.
	},
    title = "{The Mexican hat wavelet family: application to point-source detection in cosmic microwave background maps}",
  journal = {\mnras},
   eprint = {astro-ph/0604376},
 keywords = {techniques: image processing: cosmic microwave background, techniques: image processing, cosmic microwave background},
     year = 2006,
    month = jul,
   volume = 369,
    pages = {1603-1610},
      doi = {10.1111/j.1365-2966.2006.10442.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.369.1603G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Granato2015,
   author = {{Granato}, G.~L. and {Ragone-Figueroa}, C. and {Dom{\'{\i}}nguez-Tenreiro}, R. and
	{Obreja}, A. and {Borgani}, S. and {De Lucia}, G. and {Murante}, G.
	},
    title = "{The early phases of galaxy clusters formation in IR: coupling hydrodynamical simulations with GRASIL-3D}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1412.6105},
 keywords = {hydrodynamics, radiative transfer, dust, extinction, galaxies: clusters: general, infrared: galaxies, submillimetre: galaxies},
     year = 2015,
    month = jun,
   volume = 450,
    pages = {1320-1332},
      doi = {10.1093/mnras/stv676},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.450.1320G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{GreavesHolland2002,
   author = {{Greaves}, J.~S. and {Holland}, W.~S.},
    title = "{Submillimetre polarization of M82 and the Galactic Center: Implications for CMB polarimetry}",
 keywords = {Background radiations, Radiation mechanisms, polarization, Galactic center bar circumnuclear matter and bulge, Interstellar dust grains, diffuse emission, infrared cirrus, Submillimeter},
booktitle = {Astrophysical Polarized Backgrounds},
     year = 2002,
   series = {American Institute of Physics Conference Series},
   volume = 609,
   editor = {{Cecchini}, S. and {Cortiglioni}, S. and {Sault}, R. and {Sbarra}, C.
	},
    month = mar,
    pages = {267-270},
      doi = {10.1063/1.1471859},
   adsurl = {http://adsabs.harvard.edu/abs/2002AIPC..609..267G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gruppioni2013,
   author = {{Gruppioni}, C. and {Pozzi}, F. and {Rodighiero}, G. and {Delvecchio}, I. and
	{Berta}, S. and {Pozzetti}, L. and {Zamorani}, G. and {Andreani}, P. and
	{Cimatti}, A. and {Ilbert}, O. and {Le Floc'h}, E. and {Lutz}, D. and et al.
	},
    title = "{The Herschel PEP/HerMES luminosity function - I. Probing the evolution of PACS selected Galaxies to $z \simeq 4$}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1302.5209},
 keywords = {galaxies: active, galaxies: evolution, galaxies: luminosity function, mass function, galaxies: starburst, cosmology: observations, infrared: galaxies},
     year = 2013,
    month = jun,
   volume = 432,
    pages = {23-52},
      doi = {10.1093/mnras/stt308},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432...23G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Harrington2016,
   author = {{Harrington}, K.~C. and {Yun}, M.~S. and {Cybulski}, R. and
	{Wilson}, G.~W. and {Aretxaga}, I. and {Chavez}, M. and {De la Luz}, V. and
	{Erickson}, N. and {Ferrusca}, D. and {Gallup}, A.~D. and {Hughes}, D.~H. and
	{Monta{\~n}a}, A. and {Narayanan}, G. and {S{\'a}nchez-Arg{\"u}elles}, D. and
	{Schloerb}, F.~P. and {Souccar}, K. and {Terlevich}, E. and
	{Terlevich}, R. and {Zeballos}, M. and {Zavala}, J.~A.},
    title = "{Early Science with the Large Millimeter Telescope: Observations of Extremely Luminous High-z Sources Identified by Planck}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1603.05622},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160305622H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hasselfield2013,
   author = {{Hasselfield}, M. and {Hilton}, M. and {Marriage}, T.~A. and
	{Addison}, G.~E. and {Barrientos}, L.~F. and {Battaglia}, N. and
	{Battistelli}, E.~S. and {Bond}, J.~R. and {Crichton}, D. and
	{Das}, S. and {Devlin}, M.~J. and {Dicker}, S.~R. and {Dunkley}, J. and
	{D{\"u}nner}, R. and {Fowler}, J.~W. and {Gralla}, M.~B. and
	{Hajian}, A. and {Halpern}, M. and {Hincks}, A.~D. and {Hlozek}, R. and
	{Hughes}, J.~P. and {Infante}, L. and {Irwin}, K.~D. and {Kosowsky}, A. and
	{Marsden}, D. and {Menanteau}, F. and {Moodley}, K. and {Niemack}, M.~D. and
	{Nolta}, M.~R. and {Page}, L.~A. and {Partridge}, B. and {Reese}, E.~D. and
	{Schmitt}, B.~L. and {Sehgal}, N. and {Sherwin}, B.~D. and {Sievers}, J. and
	{Sif{\'o}n}, C. and {Spergel}, D.~N. and {Staggs}, S.~T. and
	{Swetz}, D.~S. and {Switzer}, E.~R. and {Thornton}, R. and {Trac}, H. and
	{Wollack}, E.~J.},
    title = "{The Atacama Cosmology Telescope: Sunyaev-Zel'dovich selected galaxy clusters at 148 GHz from three seasons of data}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1301.0816},
 primaryClass = "astro-ph.CO",
     year = 2013,
    month = jul,
   volume = 7,
      eid = {008},
    pages = {008},
      doi = {10.1088/1475-7516/2013/07/008},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...07..008H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Herranz2004,
   author = {{Herranz}, D. and {Kuruo{\u g}lu}, E.~E. and {Toffolatti}, L.
	},
    title = "{An {$\alpha$}-stable approach to the study of the P(D) distribution  of unresolved point sources in CMB sky maps}",
  journal = {\aap},
   eprint = {astro-ph/0307114},
 keywords = {methods: statistical, galaxies: statistics, cosmology: cosmic microwave background},
     year = 2004,
    month = sep,
   volume = 424,
    pages = {1081-1096},
      doi = {10.1051/0004-6361:20035858},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...424.1081H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Herranz2013,
   author = {{Herranz}, D. and {Gonz{\'a}lez-Nuevo}, J. and {Clements}, D.~L. and
	{De Zotti}, G. and {Lopez-Caniego}, M. and {Lapi}, A. and {Rodighiero}, G. and
	{Danese}, L. and {Fu}, H. and {Cooray}, A. and {Baes}, M. and
	{Bendo}, G.~J. and {Bonavera}, L. and {Carrera}, F.~J. and {Dole}, H. and
	{Eales}, S. and {Ivison}, R.~J. and {Jarvis}, M. and {Lagache}, G. and
	{Massardi}, M. and {Micha{\l}owski}, M.~J. and {Negrello}, M. and
	{Rigby}, E. and {Scott}, D. and {Valiante}, E. and {Valtchanov}, I. and
	{Van der Werf}, P. and {Auld}, R. and {Buttiglione}, S. and
	{Dariush}, A. and {Dunne}, L. and {Hopwood}, R. and {Hoyos}, C. and
	{Ibar}, E. and {Maddox}, S.},
    title = "{Herschel-ATLAS: Planck sources in the phase 1 fields}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1204.3917},
 primaryClass = "astro-ph.CO",
 keywords = {general, galaxies: evolution, submillimeter: galaxies, catalogs, gravitational lensing: strong},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A31},
    pages = {A31},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A..31H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Huchra2012,
   author = {{Huchra}, J.~P. and {Macri}, L.~M. and {Masters}, K.~L. and
	{Jarrett}, T.~H. and {Berlind}, P. and {Calkins}, M. and {Crook}, A.~C. and
	{Cutri}, R. and {Erdo{\v g}du}, P. and {Falco}, E. and {George}, T. and
	{Hutcheson}, C.~M. and {Lahav}, O. and {Mader}, J. and {Mink}, J.~D. and
	{Martimbeau}, N. and {Schneider}, S. and {Skrutskie}, M. and
	{Tokarz}, S. and {Westover}, M.},
    title = "{The 2MASS Redshift Survey{\mdash}Description and Data Release}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1108.0669},
 keywords = {catalogs, galaxies: distances and redshifts, surveys},
     year = 2012,
    month = apr,
   volume = 199,
      eid = {26},
    pages = {26},
      doi = {10.1088/0067-0049/199/2/26},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..199...26H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ivison2010,
   author = {{Ivison}, R.~J. and {Swinbank}, A.~M. and {Swinyard}, B. and
	{Smail}, I. and {Pearson}, C.~P. and {Rigopoulou}, D. and {Polehampton}, E. and
	{Baluteau}, J.-P. and {Barlow}, M.~J. and {Blain}, A.~W. and
	{Bock}, J. and {Clements}, D.~L. and {Coppin}, K. and {Cooray}, A. and
	{Danielson}, A. and {Dwek}, E. and {Edge}, A.~C. and {Franceschini}, A. and
	{Fulton}, T. and {Glenn}, J. and {Griffin}, M. and {Isaak}, K. and
	{Leeks}, S. and {Lim}, T. and {Naylor}, D. and {Oliver}, S.~J. and
	{Page}, M.~J. and {P{\'e}rez Fournon}, I. and {Rowan-Robinson}, M. and
	{Savini}, G. and {Scott}, D. and {Spencer}, L. and {Valtchanov}, I. and
	{Vigroux}, L. and {Wright}, G.~S.},
    title = "{Herschel and SCUBA-2 imaging and spectroscopy of a bright, lensed submillimetre galaxy at z = 2.3}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.1071},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, infrared: galaxies, infrared: ISM, radio continuum: galaxies, submillimeter: galaxies},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L35},
    pages = {L35},
      doi = {10.1051/0004-6361/201014548},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L..35I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ivison2013,
   author = {{Ivison}, R.~J. and {Swinbank}, A.~M. and {Smail}, I. and {Harris}, A.~I. and
	{Bussmann}, R.~S. and {Cooray}, A. and {Cox}, P. and {Fu}, H. and
	{Kov{\'a}cs}, A. and {Krips}, M. and {Narayanan}, D. and {Negrello}, M. and
	{Neri}, R. and {Pe{\~n}arrubia}, J. and {Richard}, J. and {Riechers}, D.~A. and
	{Rowlands}, K. and {Staguhn}, J.~G. and {Targett}, T.~A. and
	{Amber}, S. and {Baker}, A.~J. and {Bourne}, N. and {Bertoldi}, F. and
	{Bremer}, M. and {Calanog}, J.~A. and {Clements}, D.~L. and
	{Dannerbauer}, H. and {Dariush}, A. and {De Zotti}, G. and {Dunne}, L. and
	{Eales}, S.~A. and {Farrah}, D. and {Fleuren}, S. and {Franceschini}, A. and
	{Geach}, J.~E. and {George}, R.~D. and {Helly}, J.~C. and {Hopwood}, R. and
	{Ibar}, E. and {Jarvis}, M.~J. and {Kneib}, J.-P. and {Maddox}, S. and
	{Omont}, A. and {Scott}, D. and {Serjeant}, S. and {Smith}, M.~W.~L. and
	{Thompson}, M.~A. and {Valiante}, E. and {Valtchanov}, I. and
	{Vieira}, J. and {van der Werf}, P.},
    title = "{Herschel-ATLAS: A Binary HyLIRG Pinpointing a Cluster of Starbursting Protoellipticals}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1302.4436},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: high-redshift, galaxies: starburst, infrared: galaxies, radio continuum: galaxies, radio lines: galaxies, submillimeter: galaxies},
     year = 2013,
    month = aug,
   volume = 772,
      eid = {137},
    pages = {137},
      doi = {10.1088/0004-637X/772/2/137},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772..137I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KennicuttEvans2012,
   author = {{Kennicutt}, R.~C. and {Evans}, N.~J.},
    title = "{Star Formation in the Milky Way and Nearby Galaxies}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1204.3552},
     year = 2012,
    month = sep,
   volume = 50,
    pages = {531-608},
      doi = {10.1146/annurev-astro-081811-125610},
   adsurl = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..531K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kuehn2014,
   author = {{Kuehn}, K. and {Lawrence}, J. and {Brown}, D.~M. and {Case}, S. and
	{Colless}, M. and {Content}, R. and {Gers}, L. and {Gilbert}, J. and
	{Goodwin}, M. and {Hopkins}, A.~M. and {Ireland}, M. and {Lorente}, N.~P.~F. and
	{Muller}, R. and {Nichani}, V. and {Rakman}, A. and {Richards}, S.~N. and
	{Saunders}, W. and {Staszak}, N.~F. and {Tims}, J. and {Waller}, L.~G.
	},
    title = "{TAIPAN: optical spectroscopy with StarBugs}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
     year = 2014,
   series = {\procspie},
   volume = 9147,
    month = jul,
      eid = {914710},
    pages = {914710},
      doi = {10.1117/12.2055677},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9147E..10K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{LavauxHudson2011,
   author = {{Lavaux}, G. and {Hudson}, M.~J.},
    title = "{The 2M++ galaxy redshift catalogue}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1105.6107},
 primaryClass = "astro-ph.CO",
 keywords = {methods: data analysis, methods: numerical, methods: observational, catalogues, galaxies: luminosity function, mass function, large-scale structure of Universe},
     year = 2011,
    month = oct,
   volume = 416,
    pages = {2840-2856},
      doi = {10.1111/j.1365-2966.2011.19233.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416.2840L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LeonTavares2012,
   author = {{Le{\'o}n-Tavares}, J. and {Valtaoja}, E. and {Giommi}, P. and
	{Polenta}, G. and {Tornikoski}, M. and {L{\"a}hteenm{\"a}ki}, A. and
	{Gasparrini}, D. and {Cutini}, S.},
    title = "{Exploring the Relation between (Sub-)Millimeter Radiation and {$\gamma$}-Ray Emission in Blazars with Planck and Fermi}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.3589},
 keywords = {BL Lacertae objects: general, galaxies: jets, galaxies: nuclei, gamma rays: galaxies, quasars: general, submillimeter: galaxies },
     year = 2012,
    month = jul,
   volume = 754,
      eid = {23},
    pages = {23},
      doi = {10.1088/0004-637X/754/1/23},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754...23L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LopezCaniegoVielva2012,
   author = {{L{\'o}pez-Caniego}, M. and {Vielva}, P.},
    title = "{Biparametric adaptive filter: detection of compact sources in complex microwave backgrounds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.0368},
 keywords = {filters},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {2139-2154},
      doi = {10.1111/j.1365-2966.2012.20444.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.2139L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Comparat2016,
   author = {{Comparat}, J. and {Chuang}, C.-H. and {Rodr{\'{\i}}guez-Torres}, S. and
	{Pellejero-Ibanez}, M. and {Prada}, F. and {Yepes}, G. and {Courtois}, H.~M. and
	{Zhao}, G.-B. and {Wang}, Y. and {Sanchez}, J. and {Maraston}, C. and
	{Metcalf}, R.~B. and {Peiro-Perez}, J. and {Kitaura}, F.~S. and
	{P{\'e}rez}, E. and {Gonz{\'a}lez Delgado}, R.~M.},
    title = "{The Low Redshift survey at Calar Alto (LoRCA)}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1510.00147},
 keywords = {galaxies: abundances, cosmology: observations, large-scale structure of Universe},
     year = 2016,
    month = may,
   volume = 458,
    pages = {2940-2952},
      doi = {10.1093/mnras/stw326},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.458.2940C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Maddox2010,
   author = {{Maddox}, S.~J. and {Dunne}, L. and {Rigby}, E. and {Eales}, S. and
	{Cooray}, A. and {Scott}, D. and {Peacock}, J.~A. and {Negrello}, M. and
	{Smith}, D.~J.~B. and {Benford}, D. and {Amblard}, A. and {Auld}, R. and
	{Baes}, M. and {Bonfield}, D. and {Burgarella}, D. and {Buttiglione}, S. and
	{Cava}, A. and {Clements}, D. and {Dariush}, A. and {de Zotti}, G. and
	{Dye}, S. and {Frayer}, D. and {Fritz}, J. and {Gonzalez-Nuevo}, J. and
	{Herranz}, D. and {Ibar}, E. and {Ivison}, R. and {Jarvis}, M.~J. and
	{Lagache}, G. and {Leeuw}, L. and {Lopez-Caniego}, M. and {Pascale}, E. and
	{Pohlen}, M. and {Rodighiero}, G. and {Samui}, S. and {Serjeant}, S. and
	{Temi}, P. and {Thompson}, M. and {Verma}, A.},
    title = "{Herschel-ATLAS: The angular correlation function of submillimetre galaxies at high and low redshift}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.2406},
 primaryClass = "astro-ph.CO",
 keywords = {submillimeter: galaxies, galaxies: statistics},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L11},
    pages = {L11},
      doi = {10.1051/0004-6361/201014663},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L..11M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mancuso2015,
   author = {{Mancuso}, C. and {Lapi}, A. and {Cai}, Z.-Y. and {Negrello}, M. and
	{De Zotti}, G. and {Bressan}, A. and {Bonato}, M. and {Perrotta}, F. and
	{Danese}, L.},
    title = "{Predictions for Ultra-deep Radio Counts of Star-forming Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1507.08411},
 keywords = {galaxies: evolution, galaxies: starburst, infrared: galaxies, radiation mechanisms: general, radio continuum: galaxies},
     year = 2015,
    month = sep,
   volume = 810,
      eid = {72},
    pages = {72},
      doi = {10.1088/0004-637X/810/1/72},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...810...72M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Marchetti2016,
   author = {{Marchetti}, L. and {Vaccari}, M. and {Franceschini}, A. and
	{Arumugam}, V. and {Aussel}, H. and {B{\'e}thermin}, M. and
	{Bock}, J. and {Boselli}, A. and {Buat}, V. and {Burgarella}, D. and
	{Clements}, D.~L. and {Conley}, A. and {Conversi}, L. and {Cooray}, A. and
	{Dowell}, C.~D. and {Farrah}, D. and {Feltre}, A. and {Glenn}, J. and
	{Griffin}, M. and {Hatziminaoglou}, E. and {Heinis}, S. and
	{Ibar}, E. and {Ivison}, R.~J. and {Nguyen}, H.~T. and {O'Halloran}, B. and
	{Oliver}, S.~J. and {Page}, M.~J. and {Papageorgiou}, A. and
	{Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and {Pohlen}, M. and
	{Rigopoulou}, D. and {Roseboom}, I.~G. and {Rowan-Robinson}, M. and
	{Schulz}, B. and {Scott}, D. and {Seymour}, N. and {Shupe}, D.~L. and
	{Smith}, A.~J. and {Symeonidis}, M. and {Valtchanov}, I. and
	{Viero}, M. and {Wang}, L. and {Wardlow}, J. and {Xu}, C.~K. and
	{Zemcov}, M.},
    title = "{The HerMES submillimetre local and low-redshift luminosity functions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.06167},
 keywords = {galaxies: evolution, galaxies: luminosity function, mass function, galaxies: statistics, submillimetre: galaxies},
     year = 2016,
    month = feb,
   volume = 456,
    pages = {1999-2023},
      doi = {10.1093/mnras/stv2717},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.1999M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marsden2009,
   author = {{Marsden}, G. and {Ade}, P.~A.~R. and {Bock}, J.~J. and {Chapin}, E.~L. and
	{Devlin}, M.~J. and {Dicker}, S.~R. and {Griffin}, M. and {Gundersen}, J.~O. and
	{Halpern}, M. and {Hargrave}, P.~C. and {Hughes}, D.~H. and
	{Klein}, J. and {Mauskopf}, P. and {Magnelli}, B. and {Moncelsi}, L. and
	{Netterfield}, C.~B. and {Ngo}, H. and {Olmi}, L. and {Pascale}, E. and
	{Patanchon}, G. and {Rex}, M. and {Scott}, D. and {Semisch}, C. and
	{Thomas}, N. and {Truch}, M.~D.~P. and {Tucker}, C. and {Tucker}, G.~S. and
	{Viero}, M.~P. and {Wiebe}, D.~V.},
    title = "{BLAST: Resolving the Cosmic Submillimeter Background}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.1205},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, diffuse radiation, galaxies: evolution, galaxies: starburst, submillimeter},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {1729-1739},
      doi = {10.1088/0004-637X/707/2/1729},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707.1729M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Marsden2014,
   author = {{Marsden}, D. and {Gralla}, M. and {Marriage}, T.~A. and {Switzer}, E.~R. and
	{Partridge}, B. and {Massardi}, M. and {Morales}, G. and {Addison}, G. and
	{Bond}, J.~R. and {Crichton}, D. and {Das}, S. and {Devlin}, M. and
	{D{\"u}nner}, R. and {Hajian}, A. and {Hilton}, M. and {Hincks}, A. and
	{Hughes}, J.~P. and {Irwin}, K. and {Kosowsky}, A. and {Menanteau}, F. and
	{Moodley}, K. and {Niemack}, M. and {Page}, L. and {Reese}, E.~D. and
	{Schmitt}, B. and {Sehgal}, N. and {Sievers}, J. and {Staggs}, S. and
	{Swetz}, D. and {Thornton}, R. and {Wollack}, E.},
    title = "{The Atacama Cosmology Telescope: dusty star-forming galaxies and active galactic nuclei in the Southern survey}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1306.2288},
 primaryClass = "astro-ph.CO",
 keywords = {methods: numerical, surveys, galaxies: active, galaxies: high-redshift},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {1556-1574},
      doi = {10.1093/mnras/stu001},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.1556M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Massardi2010,
   author = {{Massardi}, M. and {Bonaldi}, A. and {Negrello}, M. and {Ricciardi}, S. and
	{Raccanelli}, A. and {de Zotti}, G.},
    title = "{A model for the cosmological evolution of low-frequency radio sources}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1001.1069},
 keywords = {galaxies: active, galaxies: evolution, radio continuum: general},
     year = 2010,
    month = may,
   volume = 404,
    pages = {532-544},
      doi = {10.1111/j.1365-2966.2010.16305.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404..532M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Massardi2013,
   author = {{Massardi}, M. and {Burke-Spolaor}, S.~G. and {Murphy}, T. and
	{Ricci}, R. and {L{\'o}pez-Caniego}, M. and {Negrello}, M. and
	{Chhetri}, R. and {De Zotti}, G. and {Ekers}, R.~D. and {Partridge}, R.~B. and
	{Sadler}, E.~M.},
    title = "{A polarization survey of bright extragalactic AT20G sources}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1309.2527},
 keywords = {polarization, techniques: polarimetric, surveys, galaxies: active, radio continuum: galaxies},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {2915-2928},
      doi = {10.1093/mnras/stt1717},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436.2915M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Massardi2016,
   author = {{Massardi}, M. and {Bonaldi}, A. and {Bonavera}, L. and {De Zotti}, G. and
	{Lopez-Caniego}, M. and {Galluzzi}, V.},
    title = "{The Planck-ATCA Co-eval Observations project: analysis of radio source properties between 5 and 217 GHz}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.02605},
 keywords = {catalogues, galaxies: active, radio continuum: galaxies},
     year = 2016,
    month = jan,
   volume = 455,
    pages = {3249-3262},
      doi = {10.1093/mnras/stv2561},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.455.3249M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matthews2009,
   author = {{Matthews}, B.~C. and {McPhee}, C.~A. and {Fissel}, L.~M. and
	{Curran}, R.~L.},
    title = "{The Legacy of SCUPOL: 850 {$\mu$}m Imaging Polarimetry from 1997 to 2005}",
  journal = {\apjs},
 keywords = {ISM: clouds, ISM: magnetic fields, polarization, stars: formation, submillimeter},
     year = 2009,
    month = may,
   volume = 182,
    pages = {143-204},
      doi = {10.1088/0067-0049/182/1/143},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..182..143M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mehrtens2012,
   author = {{Mehrtens}, N. and {Romer}, A.~K. and {Hilton}, M. and {Lloyd-Davies}, E.~J. and
	{Miller}, C.~J. and {Stanford}, S.~A. and {Hosmer}, M. and {Hoyle}, B. and
	{Collins}, C.~A. and {Liddle}, A.~R. and {Viana}, P.~T.~P. and
	{Nichol}, R.~C. and {Stott}, J.~P. and {Dubois}, E.~N. and {Kay}, S.~T. and
	{Sahl{\'e}n}, M. and {Young}, O. and {Short}, C.~J. and {Christodoulou}, L. and
	{Watson}, W.~A. and {Davidson}, M. and {Harrison}, C.~D. and
	{Baruah}, L. and {Smith}, M. and {Burke}, C. and {Mayers}, J.~A. and
	{Deadman}, P.-J. and {Rooney}, P.~J. and {Edmondson}, E.~M. and
	{West}, M. and {Campbell}, H.~C. and {Edge}, A.~C. and {Mann}, R.~G. and
	{Sabirli}, K. and {Wake}, D. and {Benoist}, C. and {da Costa}, L. and
	{Maia}, M.~A.~G. and {Ogando}, R.},
    title = "{The XMM Cluster Survey: optical analysis methodology and the first data release}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1106.3056},
 keywords = {techniques: photometric, techniques: spectroscopic, surveys, galaxies: clusters: individual: XMMXCS J091821.9+211446.0, galaxies: distances and redshifts, X-rays: galaxies: clusters},
     year = 2012,
    month = jun,
   volume = 423,
    pages = {1024-1052},
      doi = {10.1111/j.1365-2966.2012.20931.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423.1024M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Meng2015,
   author = {{Meng}, X.-L. and {Treu}, T. and {Agnello}, A. and {Auger}, M.~W. and
	{Liao}, K. and {Marshall}, P.~J.},
    title = "{Precision cosmology with time delay lenses: high resolution imaging requirements}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1506.07640},
     year = 2015,
    month = sep,
   volume = 9,
      eid = {059},
    pages = {059},
      doi = {10.1088/1475-7516/2015/09/059},
   adsurl = {http://adsabs.harvard.edu/abs/2015JCAP...09..059M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Merloni2012,
   author = {{Merloni}, A. and {Predehl}, P. and {Becker}, W. and {B{\"o}hringer}, H. and
	{Boller}, T. and {Brunner}, H. and {Brusa}, M. and {Dennerl}, K. and
	{Freyberg}, M. and {Friedrich}, P. and {Georgakakis}, A. and
	{Haberl}, F. and {Hasinger}, G. and {Meidinger}, N. and {Mohr}, J. and
	{Nandra}, K. and {Rau}, A. and {Reiprich}, T.~H. and {Robrade}, J. and
	{Salvato}, M. and {Santangelo}, A. and {Sasaki}, M. and {Schwope}, A. and
	{Wilms}, J. and {German eROSITA Consortium}, t.},
    title = "{eROSITA Science Book: Mapping the Structure of the Energetic Universe}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1209.3114},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2012,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2012arXiv1209.3114M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Mittal2012,
   author = {{Mittal}, R. and {Oonk}, J.~B.~R. and {Ferland}, G.~J. and {Edge}, A.~C. and
	{O'Dea}, C.~P. and {Baum}, S.~A. and {Whelan}, J.~T. and {Johnstone}, R.~M. and
	{Combes}, F. and {Salom{\'e}}, P. and {Fabian}, A.~C. and {Tremblay}, G.~R. and
	{Donahue}, M. and {Russell}, H.},
    title = "{Herschel observations of extended atomic gas in the core of the Perseus cluster}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.1730},
 primaryClass = "astro-ph.CO",
 keywords = {dust, extinction, photodissociation region (PDR), galaxies: clusters:
 individual: NGC 1275, galaxies: clusters: intracluster medium, galaxies: ISM, galaxies: kinematics and dynamics},
     year = 2012,
    month = nov,
   volume = 426,
    pages = {2957-2977},
      doi = {10.1111/j.1365-2966.2012.21891.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.2957M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mocanu2013,
   author = {{Mocanu}, L.~M. and {Crawford}, T.~M. and {Vieira}, J.~D. and
	{Aird}, K.~A. and {Aravena}, M. and {Austermann}, J.~E. and
	{Benson}, B.~A. and {B{\'e}thermin}, M. and {Bleem}, L.~E. and et al. },
 title = "{Extragalactic Millimeter-wave Point-source Catalog, Number Counts  and Statistics from 771 deg$^{2}$ of the SPT-SZ Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1306.3470},
 keywords = {galaxies: high-redshift, submillimeter: galaxies, surveys},
     year = 2013,
    month = dec,
   volume = 779,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/779/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779...61M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Nayyeri2016,
   author = {{Nayyeri}, H. and {Keele}, M. and {Cooray}, A. and {Riechers}, D.~A. and
	{Ivison}, R.~J. and {Harris}, A.~I. and {Frayer}, D.~T. and
	{Baker}, A.~J. and {Chapman}, S.~C. and {Eales}, S. and {Farrah}, D. and
	{Fu}, H. and {Marchetti}, L. and {Marques-Chaves}, R. and {Martinez-Navajas}, P.~I. and
	{Oliver}, S.~J. and {Omont}, A. and {Perez-Fournon}, I. and
	{Scott}, D. and {Vaccari}, M. and {Vieira}, J. and {Viero}, M. and
	{Wang}, L. and {Wardlow}, J.},
    title = "{Candidate Gravitationally Lensed Dusty Star-forming Galaxies in the Herschel Wide Area Surveys}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1601.03401},
 keywords = {galaxies: high-redshift, galaxies: starburst, gravitational lensing: strong, sub-millimeter: galaxies },
     year = 2016,
    month = may,
   volume = 823,
      eid = {17},
    pages = {17},
      doi = {10.3847/0004-637X/823/1/17},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...823...17N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Negrello2005,
   author = {{Negrello}, M. and {Gonz{\'a}lez-Nuevo}, J. and {Magliocchetti}, M. and
	{Moscardini}, L. and {De Zotti}, G. and {Toffolatti}, L. and
	{Danese}, L.},
    title = "{Effect of clustering on extragalactic source counts with low-resolution instruments}",
  journal = {\mnras},
   eprint = {astro-ph/0406388},
 keywords = {galaxies: clusters: general, galaxies: evolution, submillimetre},
     year = 2005,
    month = apr,
   volume = 358,
    pages = {869-874},
      doi = {10.1111/j.1365-2966.2005.08783.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.358..869N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Negrello2007,
   author = {{Negrello}, M. and {Perrotta}, F. and {Gonz{\'a}lez-Nuevo}, J. and
	{Silva}, L. and {de Zotti}, G. and {Granato}, G.~L. and {Baccigalupi}, C. and
	{Danese}, L.},
    title = "{Astrophysical and cosmological information from large-scale submillimetre surveys of extragalactic sources}",
  journal = {\mnras},
   eprint = {astro-ph/0703210},
 keywords = {gravitational lensing, galaxies: evolution, cosmology: observations, submillimetre},
     year = 2007,
    month = jun,
   volume = 377,
    pages = {1557-1568},
      doi = {10.1111/j.1365-2966.2007.11708.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.377.1557N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Negrello2013,
   author = {{Negrello}, M. and {Clemens}, M. and {Gonzalez-Nuevo}, J. and
	{De Zotti}, G. and {Bonavera}, L. and {Cosco}, G. and {Guarese}, G. and
	{Boaretto}, L. and {Serjeant}, S. and {Toffolatti}, L. and {Lapi}, A. and
	{Bethermin}, M. and {Castex}, G. and {Clements}, D.~L. and {Delabrouille}, J. and
	{Dole}, H. and {Franceschini}, A. and {Mandolesi}, N. and {Marchetti}, L. and
	{Partridge}, B. and {Sajina}, A.},
    title = "{The local luminosity function of star-forming galaxies derived from the Planck Early Release Compact Source Catalogue}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1211.3832},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: luminosity function, mass function, galaxies: photometry, galaxies: starburst, submillimetre: galaxies},
     year = 2013,
    month = feb,
   volume = 429,
    pages = {1309-1323},
      doi = {10.1093/mnras/sts417},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.429.1309N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Negrello2010,
   author = {{Negrello}, M. and {Hopwood}, R. and {De Zotti}, G. and {Cooray}, A. and
	{Verma}, A. and {Bock}, J. and {Frayer}, D.~T. and {Gurwell}, M.~A. and
	{Omont}, A. and {Neri}, R. and {Dannerbauer}, H. and {Leeuw}, L.~L. and
	{Barton}, E. and {Cooke}, J. and {Kim}, S. and {da Cunha}, E. and
	{Rodighiero}, G. and {Cox}, P. and {Bonfield}, D.~G. and {Jarvis}, M.~J. and
	{Serjeant}, S. and {Ivison}, R.~J. and {Dye}, S. and {Aretxaga}, I. and
	{Hughes}, D.~H. and {Ibar}, E. and {Bertoldi}, F. and {Valtchanov}, I. and
	{Eales}, S. and {Dunne}, L. and {Driver}, S.~P. and {Auld}, R. and
	{Buttiglione}, S. and {Cava}, A. and {Grady}, C.~A. and {Clements}, D.~L. and
	{Dariush}, A. and {Fritz}, J. and {Hill}, D. and {Hornbeck}, J.~B. and
	{Kelvin}, L. and {Lagache}, G. and {Lopez-Caniego}, M. and {Gonzalez-Nuevo}, J. and
	{Maddox}, S. and {Pascale}, E. and {Pohlen}, M. and {Rigby}, E.~E. and
	{Robotham}, A. and {Simpson}, C. and {Smith}, D.~J.~B. and {Temi}, P. and
	{Thompson}, M.~A. and {Woodgate}, B.~E. and {York}, D.~G. and
	{Aguirre}, J.~E. and {Beelen}, A. and {Blain}, A. and {Baker}, A.~J. and
	{Birkinshaw}, M. and {Blundell}, R. and {Bradford}, C.~M. and
	{Burgarella}, D. and {Danese}, L. and {Dunlop}, J.~S. and {Fleuren}, S. and
	{Glenn}, J. and {Harris}, A.~I. and {Kamenetzky}, J. and {Lupu}, R.~E. and
	{Maddalena}, R.~J. and {Madore}, B.~F. and {Maloney}, P.~R. and
	{Matsuhara}, H. and {Micha{\l}owski}, M.~J. and {Murphy}, E.~J. and
	{Naylor}, B.~J. and {Nguyen}, H. and {Popescu}, C. and {Rawlings}, S. and
	{Rigopoulou}, D. and {Scott}, D. and {Scott}, K.~S. and {Seibert}, M. and
	{Smail}, I. and {Tuffs}, R.~J. and {Vieira}, J.~D. and {van der Werf}, P.~P. and
	{Zmuidzinas}, J.},
    title = "{The Detection of a Population of Submillimeter-Bright, Strongly Lensed Galaxies}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1011.1255},
 primaryClass = "astro-ph.CO",
     year = 2010,
    month = nov,
   volume = 330,
    pages = {800-},
      doi = {10.1126/science.1193420},
   adsurl = {http://adsabs.harvard.edu/abs/2010Sci...330..800N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Patanchon2009,
   author = {{Patanchon}, G. and {Ade}, P.~A.~R. and {Bock}, J.~J. and {Chapin}, E.~L. and
	{Devlin}, M.~J. and {Dicker}, S.~R. and {Griffin}, M. and {Gundersen}, J.~O. and
	{Halpern}, M. and {Hargrave}, P.~C. and {Hughes}, D.~H. and
	{Klein}, J. and {Marsden}, G. and {Mauskopf}, P. and {Moncelsi}, L. and
	{Netterfield}, C.~B. and {Olmi}, L. and {Pascale}, E. and {Rex}, M. and
	{Scott}, D. and {Semisch}, C. and {Thomas}, N. and {Truch}, M.~D.~P. and
	{Tucker}, C. and {Tucker}, G.~S. and {Viero}, M.~P. and {Wiebe}, D.~V.
	},
    title = "{Submillimeter Number Counts from Statistical Analysis of BLAST Maps}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0906.0981},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: statistics, methods: data analysis, submillimeter},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {1750-1765},
      doi = {10.1088/0004-637X/707/2/1750},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707.1750P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{PlanckCollaborationI2011,
   author = {{Planck Collaboration I} and {Ade}, P.~A.~R. and {Aghanim}, N. and
	{Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and
	{Baker}, M. and {Balbi}, A. and {Banday}, A.~J. and et al.},
    title = "{Planck early results. I. The Planck mission}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.2022},
 primaryClass = "astro-ph.IM",
 keywords = {cosmology: observations, cosmic background radiation, surveys, space vehicles: instruments, instrumentation: detectors, catalogs},
     year = 2011,
    month = dec,
   volume = 536,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201116464},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A...1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckCollaboration2011stat_prop,
   author = {{Planck Collaboration XIII} and {Ade}, P.~A.~R. and {Aghanim}, N. and
	{Arg{\"u}eso}, F. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and
	{Baccigalupi}, C. and {Balbi}, A. and {Banday}, A.~J. and et al.},
    title = "{Planck early results. XIII. Statistical properties of extragalactic radio sources in the Planck Early Release Compact Source Catalogue}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.2044},
 keywords = {surveys, radio continuum: general, galaxies: active},
     year = 2011,
    month = dec,
   volume = 536,
      eid = {A13},
    pages = {A13},
      doi = {10.1051/0004-6361/201116471},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A..13P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckCollaboration2011radioSED,
   author = {{Planck Collaboration XV} and {Aatrokoski}, J. and {Ade}, P.~A.~R. and
	{Aghanim}, N. and {Aller}, H.~D. and {Aller}, M.~F. and {Angelakis}, E. and
	{Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and et al.},
    title = "{Planck early results. XV. Spectral energy distributions and radio continuum spectra of northern extragalactic radio sources}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1101.2047},
 keywords = {galaxies: active, BL Lacertae objects: general, quasars: general, radiation mechanisms: non-thermal},
     year = 2011,
    month = dec,
   volume = 536,
      eid = {A15},
    pages = {A15},
      doi = {10.1051/0004-6361/201116466},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A..15P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Planck_counts2013,
   author = {{Planck Collaboration VII} },
    title = "{Planck intermediate results. VII. Statistical properties of infrared and radio extragalactic sources from the Planck Early Release Compact Source Catalogue at frequencies between 100 and 857 GHz}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1207.4706},
 keywords = {cosmology: observations, surveys, galaxies: statistics, galaxies: evolution, galaxies: star formation, galaxies: active},
     year = 2013,
    month = feb,
   volume = 550,
      eid = {A133},
    pages = {A133},
      doi = {10.1051/0004-6361/201220053},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...550A.133P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{PlanckCollaborationXXVIII2013,
   author = {{Planck Collaboration XXVIII} and {Ade}, P.~A.~R. and {Aghanim}, N. and
	{Arg{\"u}eso}, F. and {Armitage-Caplan}, C. and {Arnaud}, M. and
	{Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and
	{Baccigalupi}, C. and et al.},
    title = "{Planck 2013 results. XXVIII. The Planck Catalogue of Compact Sources}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5088},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5088P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckCollaborationXXX2013,
   author = {{Planck Collaboration XXX} and {Ade}, P.~A.~R. and {Aghanim}, N. and
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 results. XXX. Cosmic infrared background measurements and implications for star formation}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1309.0382},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1309.0382P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Planck_parameters2015,
   author = {{Planck Collaboration. XIII} },
    title = "{Planck 2015 results. XIII. Cosmological parameters}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1502.01589},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2015,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150201589P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PCCS2_2015,
   author = {{Planck Collaboration. XXVI} },
    title = "{Planck 2015 results. XXVI. The Second Planck Catalogue of Compact Sources}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1507.02058},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2015,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150702058P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckHerschel2015,
   author = {{Planck Collaboration. XXVII}
	},
    title = "{Planck intermediate results. XXVII. High-redshift infrared galaxy overdensity candidates and lensed sources discovered by Planck and confirmed by Herschel-SPIRE}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1503.08773},
 keywords = {galaxies: high-redshift, galaxies: clusters: general, galaxies: evolution, galaxies: star formation, cosmology: observations, large-scale structure of Universe},
     year = 2015,
    month = oct,
   volume = 582,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201424790},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...582A..30P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Planck_high_z2015,
   author = {{Planck Collaboration. XXXIX} },
    title = "{Planck intermediate results. XXXIX. The Planck list of high-redshift source candidates}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1508.04171},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2015,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150804171P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckCollaboration2015SZ_CIB,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and
	{Arnaud}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and
	{Barreiro}, R.~B. and {Bartlett}, J.~G. and {Bartolo}, N. and
	{Battaner}, E. and {Benabed}, K. and {Benoit-L{\'e}vy}, A. and
	{Bernard}, J.-P. and {Bersanelli}, M. and et al.},
    title = "{Planck 2015 results. XXIII. The thermal Sunyaev-Zeldovich effect--cosmic infrared background correlation}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1509.06555},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2015,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150906555P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PlanckCollaboration2015SZcatalog,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and
	{Atrio-Barandela}, F. and {Aumont}, J. and {Aussel}, H. and
	{Baccigalupi}, C. and et al.},
    title = "{Planck 2013 results. XXXII. The updated Planck catalogue of Sunyaev-Zeldovich sources}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1502.00543},
 keywords = {errata, addenda, large-scale structure of Universe, galaxies: clusters: general, catalogs},
     year = 2015,
    month = sep,
   volume = 581,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201525787},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...581A..14P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{PlanckCollaboration2016cluster_dust,
   author = {{Planck Collaboration} and {Adam}, R. and {Ade}, P.~A.~R. and
	{Aghanim}, N. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and
	{Barreiro}, R.~B. and {Bartolo}, N. and {Battaner}, E. and {Benabed}, K. and
	{Benoit-L{\'e}vy}, A. and {Bersanelli}, M. and et al.},
    title = "{Planck intermediate results. XLIII. The spectral energy distribution of dust in clusters of galaxies}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1603.04919},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160304919P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Popesso2015,
   author = {{Popesso}, P. and {Biviano}, A. and {Finoguenov}, A. and {Wilman}, D. and
	{Salvato}, M. and {Magnelli}, B. and {Gruppioni}, C. and {Pozzi}, F. and
	{Rodighiero}, G. and {Ziparo}, F. and {Berta}, S. and {Elbaz}, D. and
	{Dickinson}, M. and {Lutz}, D. and {Altieri}, B. and {Aussel}, H. and
	{Cimatti}, A. and {Fadda}, D. and {Ilbert}, O. and {Le Floch}, E. and
	{Nordon}, R. and {Poglitsch}, A. and {Xu}, C.~K.},
    title = "{The evolution of galaxy star formation activity in massive haloes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1407.8214},
 keywords = {galaxies: evolution, galaxies: clusters: general, galaxies: luminosity function, mass function, galaxies: groups: general},
     year = 2015,
    month = feb,
   volume = 574,
      eid = {A105},
    pages = {A105},
      doi = {10.1051/0004-6361/201424711},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...574A.105P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Rachen2016,
   author = {{Rachen}, J.~P. and {Fuhrmann}, L. and {Krichbaum}, T. and {Angelakis}, E. and
	{Nestoras}, I. and {Zensus}, A. and {Sievers}, A. and {Ungerechts}, H. and
	{Keih{\"a}nen}, E. and {Reinecke}, M.},
    title = "{Coeval Observations of a Complete Sample of Blazars with Effelsberg, IRAM 30m, and Planck}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1603.02144},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160302144R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Riechers2013,
   author = {{Riechers}, D.~A. and {Bradford}, C.~M. and {Clements}, D.~L. and
	{Dowell}, C.~D. and {P{\'e}rez-Fournon}, I. and {Ivison}, R.~J. and
	{Bridge}, C. and {Conley}, A. and {Fu}, H. and {Vieira}, J.~D. and
	{Wardlow}, J. and {Calanog}, J. and {Cooray}, A. and {Hurley}, P. and
	{Neri}, R. and {Kamenetzky}, J. and {Aguirre}, J.~E. and {Altieri}, B. and
	{Arumugam}, V. and {Benford}, D.~J. and {B{\'e}thermin}, M. and
	{Bock}, J. and {Burgarella}, D. and {Cabrera-Lavers}, A. and
	{Chapman}, S.~C. and {Cox}, P. and {Dunlop}, J.~S. and {Earle}, L. and
	{Farrah}, D. and {Ferrero}, P. and {Franceschini}, A. and {Gavazzi}, R. and
	{Glenn}, J. and {Solares}, E.~A.~G. and {Gurwell}, M.~A. and
	{Halpern}, M. and {Hatziminaoglou}, E. and {Hyde}, A. and {Ibar}, E. and
	{Kov{\'a}cs}, A. and {Krips}, M. and {Lupu}, R.~E. and {Maloney}, P.~R. and
	{Martinez-Navajas}, P. and {Matsuhara}, H. and {Murphy}, E.~J. and
	{Naylor}, B.~J. and {Nguyen}, H.~T. and {Oliver}, S.~J. and
	{Omont}, A. and {Page}, M.~J. and {Petitpas}, G. and {Rangwala}, N. and
	{Roseboom}, I.~G. and {Scott}, D. and {Smith}, A.~J. and {Staguhn}, J.~G. and
	{Streblyanska}, A. and {Thomson}, A.~P. and {Valtchanov}, I. and
	{Viero}, M. and {Wang}, L. and {Zemcov}, M. and {Zmuidzinas}, J.
	},
    title = "{A dust-obscured massive maximum-starburst galaxy at a redshift of 6.34}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1304.4256},
 primaryClass = "astro-ph.CO",
     year = 2013,
    month = apr,
   volume = 496,
    pages = {329-333},
      doi = {10.1038/nature12050},
   adsurl = {http://adsabs.harvard.edu/abs/2013Natur.496..329R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RowanRobinsonClements2015,
   author = {{Rowan-Robinson}, M. and {Clements}, D.~L.},
    title = "{Cold galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1507.08778},
 keywords = {stars: formation, galaxies: evolution, galaxies: starburst, cosmology: observations, infrared: galaxies},
     year = 2015,
    month = oct,
   volume = 453,
    pages = {2050-2057},
      doi = {10.1093/mnras/stv1762},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.453.2050R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saunders2000,
   author = {{Saunders}, W. and {Sutherland}, W.~J. and {Maddox}, S.~J. and
	{Keeble}, O. and {Oliver}, S.~J. and {Rowan-Robinson}, M. and
	{McMahon}, R.~G. and {Efstathiou}, G.~P. and {Tadros}, H. and
	{White}, S.~D.~M. and {Frenk}, C.~S. and {Carrami{\~n}ana}, A. and
	{Hawkins}, M.~R.~S.},
    title = "{The PSCz catalogue}",
  journal = {\mnras},
   eprint = {astro-ph/0001117},
 keywords = {CATALOGUES, SURVEYS, GALAXIES: CLUSTERS: GENERAL, GALAXIES: DISTANCES AND REDSHIFTS, LARGE-SCALE STRUCTURE OF UNIVERSE},
     year = 2000,
    month = sep,
   volume = 317,
    pages = {55-63},
      doi = {10.1046/j.1365-8711.2000.03528.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.317...55S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Scheuer1957,
   author = {{Scheuer}, P.~A.~G.},
    title = "{A statistical method for analysing observations of faint radio stars}",
  journal = {Proceedings of the Cambridge Philosophical Society},
     year = 1957,
   volume = 53,
    pages = {764-773},
      doi = {10.1017/S0305004100032825},
   adsurl = {http://adsabs.harvard.edu/abs/1957PCPS...53..764S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Serjeant2014,
   author = {{Serjeant}, S.},
    title = "{Up to 100,000 Reliable Strong Gravitational Lenses in Future Dark Energy Experiments}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1409.0539},
 keywords = {cosmology: observations, galaxies: evolution, galaxies: formation, galaxies: starburst, infrared: galaxies, submillimeter: galaxies },
     year = 2014,
    month = sep,
   volume = 793,
      eid = {L10},
    pages = {L10},
      doi = {10.1088/2041-8205/793/1/L10},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...793L..10S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Serjeant2016,
   author = {{Serjeant}, S.},
    title = "{Strong Gravitational Lenses and Multi-Wavelength Galaxy Surveys with AKARI, Herschel, SPICA and Euclid}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1604.00282},
 keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160400282S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Swinbank2010,
   author = {{Swinbank}, A.~M. and {Smail}, I. and {Longmore}, S. and {Harris}, A.~I. and
	{Baker}, A.~J. and {De Breuck}, C. and {Richard}, J. and {Edge}, A.~C. and
	{Ivison}, R.~J. and {Blundell}, R. and {Coppin}, K.~E.~K. and
	{Cox}, P. and {Gurwell}, M. and {Hainline}, L.~J. and {Krips}, M. and
	{Lundgren}, A. and {Neri}, R. and {Siana}, B. and {Siringo}, G. and
	{Stark}, D.~P. and {Wilner}, D. and {Younger}, J.~D.},
    title = "{Intense star formation within resolved compact regions in a galaxy at z = 2.3}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1003.3674},
 primaryClass = "astro-ph.CO",
     year = 2010,
    month = apr,
   volume = 464,
    pages = {733-736},
      doi = {10.1038/nature08880},
   adsurl = {http://adsabs.harvard.edu/abs/2010Natur.464..733S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{TakeuchiIshii2004,
   author = {{Takeuchi}, T.~T. and {Ishii}, T.~T.},
    title = "{A General Formulation of the Source Confusion Statistics and Application to Infrared Galaxy Surveys}",
  journal = {\apj},
   eprint = {astro-ph/0312229},
 keywords = {Galaxies: Statistics, Infrared: Galaxies, Cosmology: Large-Scale Structure of Universe, Methods: Statistical, Submillimeter, Surveys},
     year = 2004,
    month = mar,
   volume = 604,
    pages = {40-62},
      doi = {10.1086/381882},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...604...40T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Treu2010,
   author = {{Treu}, T.},
    title = "{Strong Lensing by Galaxies}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1003.5567},
 primaryClass = "astro-ph.CO",
     year = 2010,
    month = sep,
   volume = 48,
    pages = {87-125},
      doi = {10.1146/annurev-astro-081309-130924},
   adsurl = {http://adsabs.harvard.edu/abs/2010ARA%26A..48...87T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tucci2011,
   author = {{Tucci}, M. and {Toffolatti}, L. and {de Zotti}, G. and {Mart{\'{\i}}nez-Gonz{\'a}lez}, E.
	},
    title = "{High-frequency predictions for number counts and spectral properties of extragalactic radio sources. New evidence of a break at mm wavelengths in spectra of bright blazar sources}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1103.5707},
 keywords = {galaxies: active, galaxies: statistics, radio continuum: galaxies, catalogs},
     year = 2011,
    month = sep,
   volume = 533,
      eid = {A57},
    pages = {A57},
      doi = {10.1051/0004-6361/201116972},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A..57T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{TucciToffolatti2012,
   author = {{Tucci}, M. and {Toffolatti}, L.},
    title = "{The Impact of Polarized Extragalactic Radio Sources on the Detection of CMB Anisotropies in Polarization}",
  journal = {Advances in Astronomy},
archivePrefix = "arXiv",
   eprint = {1204.0427},
 primaryClass = "astro-ph.CO",
     year = 2012,
    month = dec,
   volume = 2012,
      eid = {624987},
    pages = {624987},
      doi = {10.1155/2012/624987},
   adsurl = {http://adsabs.harvard.edu/abs/2012AdAst2012E..52T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanderWerf2011,
   author = {{van der Werf}, P.~P. and {Berciano Alba}, A. and {Spaans}, M. and
	{Loenen}, A.~F. and {Meijerink}, R. and {Riechers}, D.~A. and
	{Cox}, P. and {Wei{\ss}}, A. and {Walter}, F.},
    title = "{Water Vapor Emission Reveals a Highly Obscured, Star-forming Nuclear Region in the QSO Host Galaxy APM 08279+5255 at z = 3.9}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1106.4825},
 keywords = {galaxies: ISM, galaxies: nuclei, quasars: individual: APM 08279+5255},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {L38},
    pages = {L38},
      doi = {10.1088/2041-8205/741/2/L38},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741L..38V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Viero2013a,
   author = {{Viero}, M.~P. and {Wang}, L. and {Zemcov}, M. and {Addison}, G. and
	{Amblard}, A. and {Arumugam}, V. and {Aussel}, H. and {B{\'e}thermin}, M. and
	{Bock}, J. and {Boselli}, A. and {Buat}, V. and {Burgarella}, D. and
	{Casey}, C.~M. and {Clements}, D.~L. and {Conley}, A. and {Conversi}, L. and
	{Cooray}, A. and {De Zotti}, G. and {Dowell}, C.~D. and {Farrah}, D. and
	{Franceschini}, A. and {Glenn}, J. and {Griffin}, M. and {Hatziminaoglou}, E. and
	{Heinis}, S. and {Ibar}, E. and {Ivison}, R.~J. and {Lagache}, G. and
	{Levenson}, L. and {Marchetti}, L. and {Marsden}, G. and {Nguyen}, H.~T. and
	{O'Halloran}, B. and {Oliver}, S.~J. and {Omont}, A. and {Page}, M.~J. and
	{Papageorgiou}, A. and {Pearson}, C.~P. and {P{\'e}rez-Fournon}, I. and
	{Pohlen}, M. and {Rigopoulou}, D. and {Roseboom}, I.~G. and
	{Rowan-Robinson}, M. and {Schulz}, B. and {Scott}, D. and {Seymour}, N. and
	{Shupe}, D.~L. and {Smith}, A.~J. and {Symeonidis}, M. and {Vaccari}, M. and
	{Valtchanov}, I. and {Vieira}, J.~D. and {Wardlow}, J. and {Xu}, C.~K.
	},
    title = "{HerMES: Cosmic Infrared Background Anisotropies and the Clustering of Dusty Star-forming Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1208.5049},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: formation, galaxies: halos, large-scale structure of universe},
     year = 2013,
    month = jul,
   volume = 772,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/772/1/77},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772...77V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Viero2013b,
   author = {{Viero}, M.~P. and {Moncelsi}, L. and {Quadri}, R.~F. and {Arumugam}, V. and
	{Assef}, R.~J. and {B{\'e}thermin}, M. and {Bock}, J. and {Bridge}, C. and
	{Casey}, C.~M. and {Conley}, A. and {Cooray}, A. and {Farrah}, D. and
	{Glenn}, J. and {Heinis}, S. and {Ibar}, E. and {Ikarashi}, S. and
	{Ivison}, R.~J. and {Kohno}, K. and {Marsden}, G. and {Oliver}, S.~J. and
	{Roseboom}, I.~G. and {Schulz}, B. and {Scott}, D. and {Serra}, P. and
	{Vaccari}, M. and {Vieira}, J.~D. and {Wang}, L. and {Wardlow}, J. and
	{Wilson}, G.~W. and {Yun}, M.~S. and {Zemcov}, M.},
    title = "{HerMES: The Contribution to the Cosmic Infrared Background from Galaxies Selected by Mass and Redshift}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1304.0446},
 keywords = {cosmology: observations, galaxies: evolution, infrared: galaxies, large-scale structure of universe, submillimeter: galaxies},
     year = 2013,
    month = dec,
   volume = 779,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-637X/779/1/32},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779...32V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wang2016,
   author = {{Wang}, T. and {Elbaz}, D. and {Daddi}, E. and {Finoguenov}, A. and
	{Liu}, D. and {Schreiber}, C. and {Martin}, S. and {Strazzullo}, V. and
	{Valentino}, F. and {van der Burg}, R. and {Zanella}, A. and
	{Ciesla}, L. and {Gobat}, R. and {Le Brun}, A. and {Pannella}, M. and
	{Sargent}, M. and {Shu Qinghua Tan}, X. and {Cappelluti}, N. and
	{Li}, Y.},
    title = "{Discovery of a galaxy cluster with a violently starbursting core at z=2.506}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1604.07404},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160407404W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Xia2012,
   author = {{Xia}, J.-Q. and {Negrello}, M. and {Lapi}, A. and {De Zotti}, G. and
	{Danese}, L. and {Viel}, M.},
    title = "{Clustering of submillimetre galaxies in a self-regulated baryon collapse model}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.4212},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: haloes, galaxies: high-redshift, galaxies: statistics, submillimetre: galaxies},
     year = 2012,
    month = may,
   volume = 422,
    pages = {1324-1331},
      doi = {10.1111/j.1365-2966.2012.20705.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.1324X},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Amendola:2010ty,
   author = {{Amendola}, L. and {Catena}, R. and {Masina}, I. and {Notari}, A. and
	{Quartin}, M. and {Quercellini}, C.},
    title = "{Measuring our peculiar velocity on the CMB with high-multipole off-diagonal correlations}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1008.1183},
 primaryClass = "astro-ph.CO",
     year = 2011,
    month = jul,
   volume = 7,
      eid = {027},
    pages = {027},
      doi = {10.1088/1475-7516/2011/07/027},
   adsurl = {http://adsabs.harvard.edu/abs/2011JCAP...07..027A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011PhRvL.106s1301K,
   author = {{Kosowsky}, A. and {Kahniashvili}, T.},
    title = "{Signature of Local Motion in the Microwave Sky}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {1007.4539},
 primaryClass = "astro-ph.CO",
 keywords = {Background radiations, Observational cosmology, Mathematical and relativistic aspects of cosmology},
     year = 2011,
    month = may,
   volume = 106,
   number = 19,
      eid = {191301},
    pages = {191301},
      doi = {10.1103/PhysRevLett.106.191301},
   adsurl = {http://adsabs.harvard.edu/abs/2011PhRvL.106s1301K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvD..65j3001C,
   author = {{Challinor}, A. and {van Leeuwen}, F.},
    title = "{Peculiar velocity effects in high-resolution microwave background experiments}",
  journal = {\prd},
   eprint = {astro-ph/0112457},
 keywords = {Background radiations, Radiation mechanisms, polarization},
     year = 2002,
    month = may,
   volume = 65,
   number = 10,
      eid = {103001},
    pages = {103001},
      doi = {10.1103/PhysRevD.65.103001},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..65j3001C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Yoon:2015lta,
      author         = "Yoon, Mijin and Huterer, Dragan",
      title          = "{Kinematic dipole detection with galaxy surveys:
                        forecasts and requirements}",
      journal        = "Astrophys. J.",
      volume         = "813",
      year           = "2015",
      number         = "1",
      pages          = "L18",
      doi            = "10.1088/2041-8205/813/1/L18",
      eprint         = "1509.05374",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1509.05374;%%"
}

@ARTICLE{Notari:2015daa,
   author = {{Notari}, A. and {Quartin}, M.},
    title = "{CMB all-scale blackbody distortions induced by linearizing temperature}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1510.08793},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2015,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151008793N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Alnes:2005rw,
      author         = "Alnes, Havard and Amarzguioui, Morad and Gron, Oyvind",
      title          = "{An inhomogeneous alternative to dark energy?}",
      journal        = "Phys. Rev.",
      volume         = "D73",
      year           = "2006",
      pages          = "083519",
      doi            = "10.1103/PhysRevD.73.083519",
      eprint         = "astro-ph/0512006",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0512006;%%"
}

@article{Blomqvist:2009ps,
      author         = "Blomqvist, Michael and Mortsell, Edvard",
      title          = "{Supernovae as seen by off-center observers in a local
                        void}",
      journal        = "JCAP",
      volume         = "1005",
      year           = "2010",
      pages          = "006",
      doi            = "10.1088/1475-7516/2010/05/006",
      eprint         = "0909.4723",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:0909.4723;%%"
}

@article{Quartin:2009xr,
      author         = "Quartin, Miguel and Amendola, Luca",
      title          = "{Distinguishing Between Void Models and Dark Energy with
                        Cosmic Parallax and Redshift Drift}",
      journal        = "Phys. Rev.",
      volume         = "D81",
      year           = "2010",
      pages          = "043522",
      doi            = "10.1103/PhysRevD.81.043522",
      eprint         = "0909.4954",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "HD-THEP-09-21",
      SLACcitation   = "%%CITATION = ARXIV:0909.4954;%%"
}

@article{King:1972td,
      author         = "King, A. R. and Ellis, G. F. R.",
      title          = "{Tilted homogeneous cosmological models}",
      journal        = "Commun. Math. Phys.",
      volume         = "31",
      year           = "1973",
      pages          = "209-242",
      doi            = "10.1007/BF01646266",
      SLACcitation   = "%%CITATION = CMPHA,31,209;%%"
}

@article{Grishchuk:1978,
      author         = "Grishchuk, L. P.  and Zeldovich, I. B.",
      title          = "{Long-wavelength perturbations of a Friedmann universe, and anisotropy of the microwave background radiation}",
      journal        = "Sov.Astron.",
      volume         = "22",
      year           = "1978",
      pages          = "125-129",
}

@article{Bartolo:2006fj,
      author         = "Bartolo, Nicola and Matarrese, Sabino and Riotto,
                        Antonio",
      title          = "{CMB Anisotropies at Second-Order. 2. Analytical
                        Approach}",
      journal        = "JCAP",
      volume         = "0701",
      year           = "2007",
      pages          = "019",
      doi            = "10.1088/1475-7516/2007/01/019",
      eprint         = "astro-ph/0610110",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "CERN-PH-TH-2006-191",
      SLACcitation   = "%%CITATION = ASTRO-PH/0610110;%%"
}

@article{Langlois:1996ms,
      author         = "Langlois, David",
      title          = "{Cosmic microwave background dipole induced by double
                        inflation}",
      journal        = "Phys. Rev.",
      volume         = "D54",
      year           = "1996",
      pages          = "2447-2450",
      doi            = "10.1103/PhysRevD.54.2447",
      eprint         = "gr-qc/9606066",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = GR-QC/9606066;%%"
}

@article{Langlois:1995ca,
      author         = "Langlois, David and Piran, Tsvi",
      title          = "{Dipole anisotropy from an entropy gradient}",
      journal        = "Phys. Rev.",
      volume         = "D53",
      year           = "1996",
      pages          = "2908-2919",
      doi            = "10.1103/PhysRevD.53.2908",
      eprint         = "astro-ph/9507094",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9507094;%%"
}

@article{Turner:1991dn,
      author         = "Turner, Michael S.",
      title          = "{A Tilted Universe (and Other Remnants of the
                        Preinflationary Universe)}",
      journal        = "Phys. Rev.",
      volume         = "D44",
      year           = "1991",
      pages          = "3737-3748",
      doi            = "10.1103/PhysRevD.44.3737",
      reportNumber   = "FERMILAB-PUB-91-043-A, C-88-12-08",
      SLACcitation   = "%%CITATION = PHRVA,D44,3737;%%"
}

@article{Ade:2015tva,
      author         = "Ade, P. A. R. and others",
      title          = "{Joint Analysis of BICEP2/$Keck Array$ and $Planck$
                        Data}",
      collaboration  = "BICEP2, Planck",
      journal        = "Phys. Rev. Lett.",
      volume         = "114",
      year           = "2015",
      pages          = "101301",
      doi            = "10.1103/PhysRevLett.114.101301",
      eprint         = "1502.00612",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1502.00612;%%"
}

@article{Roldan:2015,
      author         = "Roldan, Omar and Notari, Alessio and Quartin, Miguel",
      title          = "{Observational signatures of a Superhorizon gradient mode in the CMB}",
      journal        = "To appear",
}

@book{Weinberg:2008zzc,
      author         = "Weinberg, Steven",
      title          = "{Cosmology}",
      url            = "http://www.oup.com/uk/catalogue/?ci=9780198526827",
      journal        = "Oxford, UK: Oxford Univ. Pr. (2008) 593 p",
      year           = "2008",
      reportNumber   = "ISBN-9780198526827",
      SLACcitation   = "%%CITATION = ISBN-9780198526827;%%"
}

@article{Weinberg:2003sw,
      author         = "Weinberg, Steven",
      title          = "{Adiabatic modes in cosmology}",
      journal        = "Phys. Rev.",
      volume         = "D67",
      year           = "2003",
      pages          = "123504",
      doi            = "10.1103/PhysRevD.67.123504",
      eprint         = "astro-ph/0302326",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "UTTG-12-02",
      SLACcitation   = "%%CITATION = ASTRO-PH/0302326;%%"
}

@article{Hu:1994jd,
      author         = "Hu, Wayne and Sugiyama, Naoshi",
      title          = "{Toward understanding CMB anisotropies and their
                        implications}",
      journal        = "Phys. Rev.",
      volume         = "D51",
      year           = "1995",
      pages          = "2599-2630",
      doi            = "10.1103/PhysRevD.51.2599",
      eprint         = "astro-ph/9411008",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "CFPA-TH-94-55, CFPA-94-TH-55, UTAP-193",
      SLACcitation   = "%%CITATION = ASTRO-PH/9411008;%%"
}

@article{Lewis:2006fu,
      author         = "Lewis, Antony and Challinor, Anthony",
      title          = "{Weak gravitational lensing of the cmb}",
      journal        = "Phys. Rept.",
      volume         = "429",
      year           = "2006",
      pages          = "1-65",
      doi            = "10.1016/j.physrep.2006.03.002",
      eprint         = "astro-ph/0601594",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0601594;%%"
}

@article{Seljak:1995ve,
      author         = "Seljak, Uros",
      title          = "{Gravitational lensing effect on cosmic microwave
                        background anisotropies: A Power spectrum approach}",
      journal        = "Astrophys. J.",
      volume         = "463",
      year           = "1996",
      pages          = "1",
      doi            = "10.1086/177218",
      eprint         = "astro-ph/9505109",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MIT-CSR-94-29",
      SLACcitation   = "%%CITATION = ASTRO-PH/9505109;%%"
}

@article{Malik:2008im,
      author         = "Malik, Karim A. and Wands, David",
      title          = "{Cosmological perturbations}",
      journal        = "Phys. Rept.",
      volume         = "475",
      year           = "2009",
      pages          = "1-51",
      doi            = "10.1016/j.physrep.2009.03.001",
      eprint         = "0809.4944",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ARXIV:0809.4944;%%"
}

@phdthesis{Christopherson:2011ra,
      author         = "Christopherson, Adam J.",
      title          = "{Applications of Cosmological Perturbation Theory}",
      school         = "Queen Mary, U. of London, Math. Sci.",
      year           = "2011",
      url            = "https://inspirehep.net/record/902523/files/arXiv:1106.0446.pdf",
      eprint         = "1106.0446",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1106.0446;%%"
}

@article{Bartolo:2003bz,
      author         = "Bartolo, N. and Matarrese, Sabino and Riotto, A.",
      title          = "{Evolution of second - order cosmological perturbations
                        and non-Gaussianity}",
      journal        = "JCAP",
      volume         = "0401",
      year           = "2004",
      pages          = "003",
      doi            = "10.1088/1475-7516/2004/01/003",
      eprint         = "astro-ph/0309692",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "DFPD-A-03-36",
      SLACcitation   = "%%CITATION = ASTRO-PH/0309692;%%"
}

@article{Bartolo:2005kv,
      author         = "Bartolo, Nicola and Matarrese, Sabino and Riotto,
                        Antonio",
      title          = "{The full second-order radiation transfer function for
                        large-scale cmb anisotropies}",
      journal        = "JCAP",
      volume         = "0605",
      year           = "2006",
      pages          = "010",
      doi            = "10.1088/1475-7516/2006/05/010",
      eprint         = "astro-ph/0512481",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0512481;%%"
}

@article{Bartolo:2004if,
      author         = "Bartolo, N. and Komatsu, E. and Matarrese, Sabino and
                        Riotto, A.",
      title          = "{Non-Gaussianity from inflation: Theory and
                        observations}",
      journal        = "Phys. Rept.",
      volume         = "402",
      year           = "2004",
      pages          = "103-266",
      doi            = "10.1016/j.physrep.2004.08.022",
      eprint         = "astro-ph/0406398",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "DFPD-04-A-12",
      SLACcitation   = "%%CITATION = ASTRO-PH/0406398;%%"
}

@article{Turner:1991di,
      author         = "Turner, Michael S.",
      title          = "{The Tilted universe}",
      year           = "1991",
      reportNumber   = "FERMILAB-PUB-91-073-A",
      SLACcitation   = "%%CITATION = FERMILAB-PUB-91-073-A;%%"
}

@article{Erickcek:2008jp,
      author         = "Erickcek, Adrienne L. and Carroll, Sean M. and
                        Kamionkowski, Marc",
      title          = "{Superhorizon Perturbations and the Cosmic Microwave
                        Background}",
      journal        = "Phys. Rev.",
      volume         = "D78",
      year           = "2008",
      pages          = "083012",
      doi            = "10.1103/PhysRevD.78.083012",
      eprint         = "0808.1570",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ARXIV:0808.1570;%%"
}

@book{Lyth:2009zz,
      author         = "Lyth, David H. and Liddle, Andrew R.",
      title          = "{The primordial density perturbation: Cosmology,
                        inflation and the origin of structure}",
      url            = "http://www.cambridge.org/uk/catalogue/catalogue.asp?isbn=9780521828499",
      journal        = "Cambridge, UK: Cambridge Univ. Pr. (2009) 497 p",
      year           = "2009",
      SLACcitation   = "%%CITATION = INSPIRE-853992;%%"
}

@article{Mollerach:1997up,
      author         = "Mollerach, Silvia and Matarrese, Sabino",
      title          = "{Cosmic microwave background anisotropies from second
                        order gravitational perturbations}",
      journal        = "Phys. Rev.",
      volume         = "D56",
      year           = "1997",
      pages          = "4494-4502",
      doi            = "10.1103/PhysRevD.56.4494",
      eprint         = "astro-ph/9702234",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9702234;%%"
}

@article{Bartolo:2004ty,
      author         = "Bartolo, Nicola and Matarrese, Sabino and Riotto,
                        Antonio",
      title          = "{Gauge-invariant temperature anisotropies and primordial
                        non-Gaussianity}",
      journal        = "Phys. Rev. Lett.",
      volume         = "93",
      year           = "2004",
      pages          = "231301",
      doi            = "10.1103/PhysRevLett.93.231301",
      eprint         = "astro-ph/0407505",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0407505;%%"
}

@article{Pyne:1995bs,
      author         = "Pyne, Ted and Carroll, Sean M.",
      title          = "{Higher order gravitational perturbations of the cosmic
                        microwave background}",
      journal        = "Phys. Rev.",
      volume         = "D53",
      year           = "1996",
      pages          = "2920-2929",
      doi            = "10.1103/PhysRevD.53.2920",
      eprint         = "astro-ph/9510041",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MIT-CTP-2455",
      SLACcitation   = "%%CITATION = ASTRO-PH/9510041;%%"
}

@article{Matarrese:1997ay,
      author         = "Matarrese, Sabino and Mollerach, Silvia and Bruni, Marco",
      title          = "{Second order perturbations of the Einstein-de Sitter
                        universe}",
      journal        = "Phys. Rev.",
      volume         = "D58",
      year           = "1998",
      pages          = "043504",
      doi            = "10.1103/PhysRevD.58.043504",
      eprint         = "astro-ph/9707278",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "SISSA-83-97-A",
      SLACcitation   = "%%CITATION = ASTRO-PH/9707278;%%"
}

@article{Creminelli:2011sq,
      author         = "Creminelli, Paolo and Pitrou, Cyril and Vernizzi,
                        Filippo",
      title          = "{The CMB bispectrum in the squeezed limit}",
      journal        = "JCAP",
      volume         = "1111",
      year           = "2011",
      pages          = "025",
      doi            = "10.1088/1475-7516/2011/11/025",
      eprint         = "1109.1822",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1109.1822;%%"
}

@article{Mirbabayi:2014hda,
      author         = "Mirbabayi, Mehrdad and Zaldarriaga, Matias",
      title          = "{CMB Anisotropies from a Gradient Mode}",
      journal        = "JCAP",
      volume         = "1503",
      year           = "2015",
      number         = "03",
      pages          = "056",
      doi            = "10.1088/1475-7516/2015/03/056",
      eprint         = "1409.4777",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1409.4777;%%"
}

@article{Ade:2015zua,
      author         = "Ade, P. A. R. and others",
      title          = "{Planck 2015 results. XV. Gravitational lensing}",
      collaboration  = "Planck",
      doi            = "10.1051/0004-6361/201525941",
      year           = "2015",
      eprint         = "1502.01591",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1502.01591;%%"
}

@article{Hu:2001yq,
      author         = "Hu, Wayne and Cooray, Asantha",
      title          = "{Gravitational time delay effects on cosmic microwave
                        background anisotropies}",
      journal        = "Phys. Rev.",
      volume         = "D63",
      year           = "2001",
      pages          = "023504",
      doi            = "10.1103/PhysRevD.63.023504",
      eprint         = "astro-ph/0008001",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0008001;%%"
}

@book{Mukhanov:2005sc,
      author         = "Mukhanov, V.",
      title          = "{Physical Foundations of Cosmology}",
      publisher      = "Cambridge University Press",
      address        = "Oxford",
      year           = "2005",
      url            = "http://www-spires.fnal.gov/spires/find/books/www?cl=QB981.M89::2005",
      ISBN           = "0521563984, 9780521563987",
      SLACcitation   = "%%CITATION = INSPIRE-706151;%%"
}

@article{cosmostat-webpage,
	Note = {\url{http://www.cosmostat.org/}}}

@article{Paci:2013gs,
	Archiveprefix = {arXiv},
	Author = {Paci, F. and Gruppuso, A. and Finelli, F. and De Rosa, A. and Mandolesi, N. and others},
	Eprint = {1301.5195},
	Primaryclass = {astro-ph.CO},
	Slaccitation = {%%CITATION = ARXIV:1301.5195;%%},
	Title = {{Hemispherical power asymmetries in the WMAP 7-year low-resolution temperature and polarization maps}},
	Year = {2013}}

@article{Axelsson:2013mva,
	Archiveprefix = {arXiv},
	Author = {Axelsson, M. and Fantaye, Y. and Hansen, F.K. and Banday, A.J. and Eriksen, H.K. and others},
	Eprint = {1303.5371},
	Primaryclass = {astro-ph.CO},
	Slaccitation = {%%CITATION = ARXIV:1303.5371;%%},
	Title = {{Directional dependence of LCDM cosmological parameters}},
	Year = {2013}}

@ARTICLE{2004A&A...416..447B,
   author = {{Basu}, K. and {Hern{\'a}ndez-Monteagudo}, C. and {Sunyaev}, R.~A.
	},
    title = "{CMB observations and the production of chemical elements   at the end of the dark ages}",
  journal = {\aap},
   eprint = {astro-ph/0311620},
 keywords = {cosmology: cosmic microwave background, cosmology: theory, galaxies: intergalactic medium, atomic processes, nuclear reactions, nucleosynthesis, abundances},
     year = 2004,
    month = mar,
   volume = 416,
    pages = {447-466},
      doi = {10.1051/0004-6361:20034298},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...416..447B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.458L..99M,
   author = {{Mashian}, N. and {Loeb}, A. and {Sternberg}, A.},
    title = "{Spectral distortion of the CMB by the cumulative CO emission from galaxies throughout cosmic history}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1601.02618},
 keywords = {intergalactic medium, cosmic background radiation, cosmology: theory, early Universe},
     year = 2016,
    month = may,
   volume = 458,
    pages = {L99-L103},
      doi = {10.1093/mnrasl/slw027},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.458L..99M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014MNRAS.438.2547B,
   author = {{Bonato}, M. and {Negrello}, M. and {Cai}, Z.-Y. and {De Zotti}, G. and 
	{Bressan}, A. and {Lapi}, A. and {Gruppioni}, C. and {Spinoglio}, L. and 
	{Danese}, L.},
    title = "{Exploring the early dust-obscured phase of galaxy formation with blind mid-/far-infrared spectroscopic surveys}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.1891},
 keywords = {galaxies: active, galaxies: evolution, galaxies: luminosity function, mass function, galaxies: starburst, infrared: galaxies},
     year = 2014,
    month = mar,
   volume = 438,
    pages = {2547-2564},
      doi = {10.1093/mnras/stt2375},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.2547B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012MNRAS.419.1294C,
   author = {{Chluba}, J. and {Sunyaev}, R.~A.},
    title = "{The evolution of CMB spectral distortions in the early Universe}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1109.6552},
 keywords = {cosmology: observations, cosmology: theory},
     year = 2012,
    month = jan,
   volume = 419,
    pages = {1294-1314},
      doi = {10.1111/j.1365-2966.2011.19786.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.419.1294C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2015mgm..conf..373S,
   author = {{Sunyaev}, R.~A. and {Khatri}, R.},
    title = "{Unavoidable CMB Spectral Features and Blackbody Photosphere of Our Universe}",
booktitle = {Thirteenth Marcel Grossmann Meeting: On Recent Developments in Theoretical and Experimental General Relativity, Astrophysics and Relativistic Field Theories},
     year = 2015,
   editor = {{Rosquist}, K.},
    month = jan,
    pages = {373-397},
      doi = {10.1142/9789814623995_0020},
   adsurl = {http://adsabs.harvard.edu/abs/2015mgm..conf..373S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PTEP.2014fB107T,
   author = {{Tashiro}, H.},
    title = "{CMB spectral distortions and energy release in the early universe}",
  journal = {Progress of Theoretical and Experimental Physics},
 keywords = {E63, E65},
     year = 2014,
    month = jun,
   volume = 2014,
   number = 6,
      eid = {06B107},
    pages = {06B107},
      doi = {10.1093/ptep/ptu066},
   adsurl = {http://adsabs.harvard.edu/abs/2014PTEP.2014fB107T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1974IAUS...63..167S,
   author = {{Sunyaev}, R.~A.},
    title = "{The thermal history of the universe and the spectrum of relic radiation}",
 keywords = {Astronomical Models, Background Radiation, Big Bang Cosmology, Black Body Radiation, Radio Spectra, Antimatter, Brightness Temperature, Galactic Clusters, Optical Thickness, Red Shift, Spectrum Analysis, Turbulence Effects, X Ray Astronomy},
booktitle = {Confrontation of Cosmological Theories with Observational Data},
     year = 1974,
   series = {IAU Symposium},
   volume = 63,
   editor = {{Longair}, M.~S.},
    pages = {167-173},
   adsurl = {http://adsabs.harvard.edu/abs/1974IAUS...63..167S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975SvA....18..413I,
   author = {{Illarionov}, A.~F. and {Siuniaev}, R.~A.},
    title = "{Comptonization, characteristic radiation spectra, and thermal balance of low-density plasma}",
  journal = {\sovast},
 keywords = {Compton Effect, Cosmic Plasma, Cosmology, Emission Spectra, Heat Balance, Rarefied Plasmas, Black Body Radiation, Electromagnetic Scattering, Ion Temperature, Photon-Electron Interaction, Plasma Spectra, X Ray Sources},
     year = 1975,
    month = feb,
   volume = 18,
    pages = {413-419},
   adsurl = {http://adsabs.harvard.edu/abs/1975SvA....18..413I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1974AZh....51..698I,
   author = {{Illarionov}, A.~F. and {Siuniaev}, R.~A.},
    title = "{Comptonization, characteristic spectra, and heat balance of low-density plasma}",
  journal = {\azh},
 keywords = {Compton Effect, Cosmic Plasma, Cosmology, Emission Spectra, Heat Balance, Rarefied Plasmas, Black Body Radiation, Electromagnetic Scattering, Ion Temperature, Photon-Electron Interaction, Plasma Spectra, X Ray Sources},
     year = 1974,
    month = aug,
   volume = 51,
    pages = {698-711},
   adsurl = {http://adsabs.harvard.edu/abs/1974AZh....51..698I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...195....1C,
   author = {{Chan}, K.~L. and {Jones}, B.~J.~T.},
    title = "{Distortions of the 3 K background radiation spectrum - Observational constraints on the early thermal history of the universe}",
  journal = {\apj},
 keywords = {Background Radiation, Brightness Temperature, Cosmology, Radio Spectra, Bremsstrahlung, Compton Effect, Electron Energy, Microwave Spectra, Recombination Reactions, Universe},
     year = 1975,
    month = jan,
   volume = 195,
    pages = {1-11},
      doi = {10.1086/153299},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...195....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...198..245C,
   author = {{Chan}, K.~L. and {Jones}, B.~J.~T.},
    title = "{Distortions of the microwave background radiation spectrum in the submillimeter wavelength region}",
  journal = {\apj},
 keywords = {Background Radiation, Brightness Temperature, Compton Effect, Microwave Spectra, Submillimeter Waves, Astronomical Models, Microwave Scattering, Numerical Analysis, Perturbation Theory, Radio Astronomy},
     year = 1975,
    month = jun,
   volume = 198,
    pages = {245-248},
      doi = {10.1086/153600},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...198..245C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...200..454C,
   author = {{Chan}, K.~L. and {Jones}, B.~J.~T.},
    title = "{The evolution of the cosmic radiation spectrum under the influence of turbulent heating. I - Theory. II - Numerical calculation and application}",
  journal = {\apj},
 keywords = {Background Radiation, Cosmic Rays, Energy Spectra, Plasma Heating, Turbulent Heat Transfer, Electron Plasma, Energy Transfer, Incompressible Fluids, Radiative Transfer, Stimulated Emission},
     year = 1975,
    month = sep,
   volume = 200,
    pages = {454-470},
      doi = {10.1086/153811},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...200..454C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...200..461C,
   author = {{Chan}, K.~L. and {Jones}, B.~J.~T.},
    title = "{The Evolution of the Cosmic Radiation Spectrum Under the Influence of Turbulent Heating. II. Numerical Calculation and Application}",
  journal = {\apj},
     year = 1975,
    month = sep,
   volume = 200,
    pages = {461-470},
      doi = {10.1086/153812},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...200..461C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977NCimR...7..277D,
   author = {{Danese}, L. and {de Zotti}, G.},
    title = "{The relic radiation spectrum and the thermal history of the Universe}",
  journal = {Nuovo Cimento Rivista Serie},
 keywords = {Background Radiation, Black Body Radiation, Cosmic Plasma, Cosmology, Microwave Spectra, Universe, Astronomical Models, Bibliographies, Big Bang Cosmology, Bremsstrahlung, Compton Effect, Electromagnetic Scattering, Electron Energy, Interstellar Matter, Kinetic Energy, Photons, Radiation Distribution},
     year = 1977,
    month = sep,
   volume = 7,
    pages = {277-362},
      doi = {10.1007/BF02747276},
   adsurl = {http://adsabs.harvard.edu/abs/1977NCimR...7..277D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978A&A....68..157D,
   author = {{Danese}, L. and {de Zotti}, G.},
    title = "{A statistical analysis of the data on the microwave background radiation spectrum}",
  journal = {\aap},
 keywords = {Background Radiation, Cosmology, Microwave Spectra, Statistical Analysis, Big Bang Cosmology, Confidence Limits, Microwave Radiometers},
     year = 1978,
    month = aug,
   volume = 68,
    pages = {157-164},
   adsurl = {http://adsabs.harvard.edu/abs/1978A%26A....68..157D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982AcC....11...55D,
   author = {{de Zotti}, G.},
    title = "{Distortions in the Rayleigh-Jeans Region of the Cosmic Background Radiation Spectrum}",
  journal = {Acta Cosmologica},
     year = 1982,
   volume = 11,
    pages = {55},
   adsurl = {http://adsabs.harvard.edu/abs/1982AcC....11...55D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980A&A....84..364D,
   author = {{Danese}, L. and {de Zotti}, G.},
    title = "{On distortions in the Rayleigh-Jeans region of the cosmic background radiation spectrum}",
  journal = {\aap},
 keywords = {Background Radiation, Big Bang Cosmology, Jeans Theory, Radiation Spectra, Relic Radiation, Distortion, Line Shape, Red Shift, Spectrum Analysis},
     year = 1980,
    month = apr,
   volume = 84,
    pages = {364},
   adsurl = {http://adsabs.harvard.edu/abs/1980A%26A....84..364D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980ARA&A..18..537S,
   author = {{Sunyaev}, R.~A. and {Zeldovich}, I.~B.},
    title = "{Microwave background radiation as a probe of the contemporary structure and history of the universe}",
  journal = {\araa},
 keywords = {Background Radiation, Cosmology, Microwaves, Relic Radiation, Universe, Big Bang Cosmology, Compton Effect, Cosmic Gases, Energy Transfer, Galactic Clusters, Intergalactic Media, Microwave Spectra},
     year = 1980,
   volume = 18,
    pages = {537-560},
      doi = {10.1146/annurev.aa.18.090180.002541},
   adsurl = {http://adsabs.harvard.edu/abs/1980ARA%26A..18..537S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982A&A...107...39D,
   author = {{Danese}, L. and {de Zotti}, G.},
    title = "{Double Compton process and the spectrum of the microwave background}",
  journal = {\aap},
 keywords = {Background Radiation, Big Bang Cosmology, Compton Effect, Cosmic Rays, Microwave Spectra, Relic Radiation, Bremsstrahlung, Data Smoothing, Galactic Evolution, Kinetic Equations, Photon Density, Radiation Distribution, Red Shift},
     year = 1982,
    month = mar,
   volume = 107,
    pages = {39-42},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...107...39D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983A&A...123..171L,
   author = {{Lyubarsky}, Y.~E. and {Sunyaev}, R.~A.},
    title = "{The spectral features in the microwave background spectrum due to energy release in the early universe}",
  journal = {\aap},
 keywords = {Background Radiation, Big Bang Cosmology, Hydrogen Recombinations, Lyman Spectra, Microwave Spectra, Relic Radiation, Abundance, Atomic Spectra, Black Body Radiation, Electron Transitions, Helium, Quantum Statistics, Red Shift},
     year = 1983,
    month = jul,
   volume = 123,
    pages = {171-183},
   adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...123..171L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986PhLB..169..280K,
   author = {{Kawasaki}, M. and {Sato}, K.},
    title = "{The effect of radiative decay of massive particles on the spectrum of the microwave background radiation}",
  journal = {Physics Letters B},
     year = 1986,
    month = mar,
   volume = 169,
    pages = {280-284},
      doi = {10.1016/0370-2693(86)90666-0},
   adsurl = {http://adsabs.harvard.edu/abs/1986PhLB..169..280K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1987PASJ...39..837K,
   author = {{Kawasaki}, M. and {Sato}, K.},
    title = "{Distortion of microwave background radiation by decaying particles}",
  journal = {\pasj},
 keywords = {Cosmology, Radioactive Decay, Relic Radiation, Weak Interactions (Field Theory), Heavy Ions, Neutrinos, Spectrum Analysis, Stellar Radiation},
     year = 1987,
   volume = 39,
    pages = {837-842},
   adsurl = {http://adsabs.harvard.edu/abs/1987PASJ...39..837K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1990ASSL..164..153D,
   author = {{Danese}, L. and {Burigana}, C. and {Toffolatti}, L. and {de Zotti}, G. and 
	{Franceschini}, A.},
    title = "{Theoretical implications of the CMB spectral distortions}",
 keywords = {Astronomical Spectroscopy, Extraterrestrial Radio Waves, Microwave Spectra, Radio Astronomy, Relic Radiation, Anisotropy, Compton Effect, Cosmology, Galactic Clusters, Red Shift, Submillimeter Waves},
booktitle = {The Cosmic Microwave Backround: 25 Years Later},
     year = 1990,
   series = {Astrophysics and Space Science Library},
   volume = 164,
   editor = {{Mandolesi}, N. and {Vittorio}, N.},
    pages = {153-172},
      doi = {10.1007/978-94-009-0655-6_10},
   adsurl = {http://adsabs.harvard.edu/abs/1990ASSL..164..153D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990PhRvD..41..354B,
   author = {{Bernstein}, J. and {Dodelson}, S.},
    title = "{Aspects of the Zel'dovich-Sunyaev mechanism}",
  journal = {\prd},
     year = 1990,
    month = jan,
   volume = 41,
    pages = {354-373},
      doi = {10.1103/PhysRevD.41.354},
   adsurl = {http://adsabs.harvard.edu/abs/1990PhRvD..41..354B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014arXiv1405.6938C,
   author = {{Chluba}, J.},
    title = "{Science with CMB spectral distortions}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1405.6938},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Theory},
     year = 2014,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1405.6938C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.443.1881C,
   author = {{Chluba}, J.},
    title = "{Tests of the CMB temperature-redshift relation, CMB spectral distortions and why adiabatic photon production is hard}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1405.1277},
 keywords = {cosmic background radiation, cosmological parameters, cosmology: observations, cosmology: theory, dark energy, early Universe},
     year = 2014,
    month = sep,
   volume = 443,
    pages = {1881-1888},
      doi = {10.1093/mnras/stu1260},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.443.1881C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..90h3529A,
   author = {{Amin}, M.~A. and {Grin}, D.},
    title = "{Probing early-universe phase transitions with CMB spectral distortions}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1405.1039},
 keywords = {Origin and formation of the Universe, Particle-theory and field-theory models of the early Universe, Background radiations, Cosmology},
     year = 2014,
    month = oct,
   volume = 90,
   number = 8,
      eid = {083529},
    pages = {083529},
      doi = {10.1103/PhysRevD.90.083529},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90h3529A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002astro.ph..2082A,
   author = {{Afshordi}, N.},
    title = "{Cyclotron Emission and Thermalization of the CMB Spectrum}",
  journal = {ArXiv Astrophysics e-prints},
   eprint = {astro-ph/0202082},
 keywords = {Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
     year = 2002,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2002astro.ph..2082A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@unpublished{ediss4063,
            year = {2005},
       publisher = {Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen},
           title = {Spectral Distortions of the Cosmic Microwave Background},
          author = {Jens Chluba},
           month = {July},
        keywords = {Cosmic Microwave Background, spectral distortions, double Compton scattering, SZ effect},
             url = {http://nbn-resolving.de/urn:nbn:de:bvb:19-40639}
}

@ARTICLE{2005NewA...11....1Z,
   author = {{Zizzo}, A. and {Burigana}, C.},
    title = "{On the effect of cyclotron emission on the spectral distortions of the cosmic microwave background}",
  journal = {\na},
   eprint = {astro-ph/0505259},
     year = 2005,
    month = oct,
   volume = 11,
    pages = {1-16},
      doi = {10.1016/j.newast.2005.05.003},
   adsurl = {http://adsabs.harvard.edu/abs/2005NewA...11....1Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...825..130I,
   author = {{Imara}, N. and {Loeb}, A.},
    title = "{The Distortion of the Cosmic Microwave Background Spectrum Due to Intergalactic Dust}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1604.00005},
 keywords = {cosmic background radiation, dark ages, reionization, first stars, dust, extinction, galaxies: high-redshift, intergalactic medium},
     year = 2016,
    month = jul,
   volume = 825,
      eid = {130},
    pages = {130},
      doi = {10.3847/0004-637X/825/2/130},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...825..130I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JCAP...03..047D,
   author = {{De Zotti}, G. and {Negrello}, M. and {Castex}, G. and {Lapi}, A. and 
	{Bonato}, M.},
    title = "{Another look at distortions of the Cosmic Microwave Background spectrum}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1512.04816},
     year = 2016,
    month = mar,
   volume = 3,
      eid = {047},
    pages = {047},
      doi = {10.1088/1475-7516/2016/03/047},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...03..047D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...688...24G,
   author = {{Gervasi}, M. and {Zannoni}, M. and {Tartari}, A. and {Boella}, G. and 
	{Sironi}, G.},
    title = "{TRIS. II. Search for CMB Spectral Distortions at 0.60, 0.82, and 2.5 GHz}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.4750},
 keywords = {cosmic microwave background, cosmological parameters, cosmology: observations, diffuse radiation, radio continuum: galaxies},
     year = 2008,
    month = nov,
   volume = 688,
      eid = {24-31},
    pages = {24-31},
      doi = {10.1086/592134},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...688...24G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1970AuJPh..23...45W,
   author = {{Wall}, J.~V. and {Chu}, T.~Y. and {Yen}, J.~L.},
    title = "{Measurements of absolute sky brightness temperatures at 320 and 707 MHz.}",
  journal = {Australian Journal of Physics},
     year = 1970,
   volume = 23,
    pages = {45-57},
      doi = {10.1071/PH700045},
   adsurl = {http://adsabs.harvard.edu/abs/1970AuJPh..23...45W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975PhRvL..34.1036W,
   author = {{Woody}, D.~P. and {Mather}, J.~C. and {Nishioka}, N.~S. and 
	{Richards}, P.~L.},
    title = "{Measurement of the spectrum of the submillimeter cosmic background}",
  journal = {Physical Review Letters},
     year = 1975,
    month = apr,
   volume = 34,
    pages = {1036-1039},
      doi = {10.1103/PhysRevLett.34.1036},
   adsurl = {http://adsabs.harvard.edu/abs/1975PhRvL..34.1036W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989HiA.....8..689M,
   author = {{Matsumoto}, T.},
    title = "{Submillimeter spectrum of the cosmic background radiation}",
  journal = {Highlights of Astronomy},
     year = 1989,
   volume = 8,
    pages = {689},
   adsurl = {http://adsabs.harvard.edu/abs/1989HiA.....8..689M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989SvAL...15..333Z,
   author = {{Zinchenko}, I.~I.},
    title = "{The Submillimeter Cosmic Background Spectrum and the Dust Content of the Universe}",
  journal = {Soviet Astronomy Letters},
     year = 1989,
    month = sep,
   volume = 15,
    pages = {333},
   adsurl = {http://adsabs.harvard.edu/abs/1989SvAL...15..333Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988ApJ...329..567M,
   author = {{Matsumoto}, T. and {Hayakawa}, S. and {Matsuo}, H. and {Murakami}, H. and 
	{Sato}, S. and {Lange}, A.~E. and {Richards}, P.~L.},
    title = "{The submillimeter spectrum of the cosmic background radiation}",
  journal = {\apj},
 keywords = {Background Radiation, Radio Astronomy, Relic Radiation, Submillimeter Waves, Earth Atmosphere, Liquid Helium, Radiometers, Rocket-Borne Instruments},
     year = 1988,
    month = jun,
   volume = 329,
    pages = {567-571},
      doi = {10.1086/166403},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...329..567M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990ApJ...362..107B,
   author = {{Bernstein}, G.~M. and {Fischer}, M.~L. and {Richards}, P.~L. and 
	{Peterson}, J.~B. and {Timusk}, T.},
    title = "{A measurement of the spectrum of the cosmic background radiation from 1 to 3 millimeter wavelength}",
  journal = {\apj},
 keywords = {Brightness Temperature, Millimeter Waves, Radiation Spectra, Relic Radiation, Spectral Bands, Black Body Radiation, Cosmic Background Explorer Satellite, Plancks Constant, Spectral Methods},
     year = 1990,
    month = oct,
   volume = 362,
    pages = {107-113},
      doi = {10.1086/169247},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...362..107B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1985PhRvL..55..332P,
   author = {{Peterson}, J.~B. and {Richards}, P.~L. and {Timusk}, T.},
    title = "{Spectrum of the cosmic background radiation at millimeter wavelengths}",
  journal = {Physical Review Letters},
 keywords = {Brightness Temperature, Cosmology, Radiation Spectra, Relic Radiation, Background Radiation, Balloon-Borne Instruments, Millimeter Waves},
     year = 1985,
    month = jul,
   volume = 55,
    pages = {332-335},
      doi = {10.1103/PhysRevLett.55.332},
   adsurl = {http://adsabs.harvard.edu/abs/1985PhRvL..55..332P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...473..576F,
   author = {{Fixsen}, D.~J. and {Cheng}, E.~S. and {Gales}, J.~M. and {Mather}, J.~C. and 
	{Shafer}, R.~A. and {Wright}, E.~L.},
    title = "{The Cosmic Microwave Background Spectrum from the Full COBE FIRAS Data Set}",
  journal = {\apj},
   eprint = {astro-ph/9605054},
 keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: OBSERVATIONS},
     year = 1996,
    month = dec,
   volume = 473,
    pages = {576},
      doi = {10.1086/178173},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...473..576F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...734....6S,
   author = {{Seiffert}, M. and {Fixsen}, D.~J. and {Kogut}, A. and {Levin}, S.~M. and 
	{Limon}, M. and {Lubin}, P.~M. and {Mirel}, P. and {Singal}, J. and 
	{Villela}, T. and {Wollack}, E. and {Wuensche}, C.~A.},
    title = "{Interpretation of the ARCADE 2 Absolute Sky Brightness Measurement}",
  journal = {\apj},
 keywords = {cosmic background radiation, cosmology: observations},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {6},
    pages = {6},
      doi = {10.1088/0004-637X/734/1/6},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734....6S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...802..135R,
   author = {{Ruan}, J.~J. and {McQuinn}, M. and {Anderson}, S.~F.},
    title = "{Detection of Quasar Feedback from the Thermal Sunyaev-Zel{\rsquo}dovich Effect in Planck}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1502.01723},
 keywords = {quasars: general, cosmic background radiation},
     year = 2015,
    month = apr,
   volume = 802,
      eid = {135},
    pages = {135},
      doi = {10.1088/0004-637X/802/2/135},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...802..135R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJS...88..253S,
   author = {{Sutherland}, R.~S. and {Dopita}, M.~A.},
    title = "{Cooling functions for low-density astrophysical plasmas}",
  journal = {\apjs},
 keywords = {Cooling Flows (Astrophysics), Cosmic Plasma, Nonequilibrium Ionization, One Dimensional Flow, Plasma Slabs, Radiative Transfer, Charge Exchange, Electron Impact, Grid Generation (Mathematics), Hydrogen Recombinations, Ionization, Mathematical Models, Metallicity, Photoionization, Radiative Recombination, Rarefied Plasmas, Resonance Lines},
     year = 1993,
    month = sep,
   volume = 88,
    pages = {253-327},
      doi = {10.1086/191823},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJS...88..253S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhRvL.115z1301H,
   author = {{Hill}, J.~C. and {Battaglia}, N. and {Chluba}, J. and {Ferraro}, S. and 
	{Schaan}, E. and {Spergel}, D.~N.},
    title = "{Taking the Universe's Temperature with Spectral Distortions of the Cosmic Microwave Background}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {1507.01583},
 keywords = {Background radiations, Observational cosmology},
     year = 2015,
    month = dec,
   volume = 115,
   number = 26,
      eid = {261301},
    pages = {261301},
      doi = {10.1103/PhysRevLett.115.261301},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhRvL.115z1301H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.463.1797D,
   author = {{Dolag}, K. and {Komatsu}, E. and {Sunyaev}, R.},
    title = "{SZ effects in the Magneticum Pathfinder simulation: comparison with the Planck, SPT, and ACT results}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1509.05134},
 keywords = {hydrodynamics, methods: numerical, galaxies: clusters: general, cosmic background radiation, cosmology: theory},
     year = 2016,
    month = dec,
   volume = 463,
    pages = {1797-1811},
      doi = {10.1093/mnras/stw2035},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.463.1797D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015JCAP...08..013K,
   author = {{Khatri}, R. and {Sunyaev}, R.},
    title = "{Limits on the fluctuating part of y-type distortion monopole from Planck and SPT results}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1505.00781},
     year = 2015,
    month = aug,
   volume = 8,
      eid = {013},
    pages = {013},
      doi = {10.1088/1475-7516/2015/08/013},
   adsurl = {http://adsabs.harvard.edu/abs/2015JCAP...08..013K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.336.1256K,
   author = {{Komatsu}, E. and {Seljak}, U.},
    title = "{The Sunyaev-Zel'dovich angular power spectrum as a probe of cosmological parameters}",
  journal = {\mnras},
   eprint = {astro-ph/0205468},
 keywords = {galaxies: clusters: general, galaxies: haloes, cosmic microwave background, cosmological parameters, cosmology: theory, dark matter},
     year = 2002,
    month = nov,
   volume = 336,
    pages = {1256-1270},
      doi = {10.1046/j.1365-8711.2002.05889.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336.1256K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1970PSS1825F,
   author = {{Forman}, M.~A.},
    title = "{The Compton-Getting effect for cosmic-ray particles and photons and the Lorentz-invariance of distribution functions}",
  journal = {\planss},
     year = 1970,
    month = jan,
   volume = 18,
    pages = {25-31},
      doi = {10.1016/0032-0633(70)90064-4},
   adsurl = {http://adsabs.harvard.edu/abs/1970P%26SS...18...25F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990SvA....34..130D,
   author = {{Dorosheva}, E.~I. and {Naselskii}, P.~D. and {Novikov}, I.~D.
	},
    title = "{Distortion of the Spectrum of the Microwave Background Radiation by the Decay of Massive Primordial Particles in the Universe}",
  journal = {\sovast},
     year = 1990,
    month = apr,
   volume = 34,
    pages = {130},
   adsurl = {http://adsabs.harvard.edu/abs/1990SvA....34..130D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990AZh....67..257D,
   author = {{Dorosheva}, E.~I. and {Naselskij}, P.~D. and {Novikov}, I.~D.
	},
    title = "{Distortion of the microwave background spectrum due to decays of massive relic particles in the universe}",
  journal = {\azh},
 keywords = {Microwave Spectra, Relic Radiation, Signal Distortion, Weak Energy Interactions, Astronomical Models, Brightness Temperature, Space Plasmas, Universe},
     year = 1990,
    month = apr,
   volume = 67,
    pages = {257-262},
   adsurl = {http://adsabs.harvard.edu/abs/1990AZh....67..257D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...246...49B,
   author = {{Burigana}, C. and {Danese}, L. and {de Zotti}, G.},
    title = "{Formation and evolution of early distortions of the microwave background spectrum - A numerical study}",
  journal = {\aap},
 keywords = {Microwave Emission, Microwave Spectra, Red Shift, Relic Radiation, Thermalization (Energy Absorption), Analytic Functions, Baryons, Compton Effect, Cosmology, Numerical Analysis},
     year = 1991,
    month = jun,
   volume = 246,
    pages = {49-58},
   adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...246...49B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...379....1B,
   author = {{Burigana}, C. and {Danese}, L. and {de Zotti}, G.},
    title = "{Constraints on the thermal history of the universe from the cosmic microwave background spectrum}",
  journal = {\apj},
 keywords = {Background Radiation, Microwave Spectra, Relic Radiation, Universe, Analytic Functions, Compton Effect, Cosmology, Energy Dissipation, Numerical Analysis},
     year = 1991,
    month = sep,
   volume = 379,
    pages = {1-5},
      doi = {10.1086/170479},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...379....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991MNRAS.248...52B,
   author = {{Barrow}, J.~D. and {Coles}, P.},
    title = "{Primordial density fluctuations and the microwave background spectrum}",
  journal = {\mnras},
 keywords = {Black Body Radiation, Density Distribution, Galactic Evolution, Relic Radiation, Baryons, Cosmic Background Explorer Satellite, Microwave Spectra},
     year = 1991,
    month = jan,
   volume = 248,
    pages = {52-57},
      doi = {10.1093/mnras/248.1.52},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.248...52B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...371...14D,
   author = {{Daly}, R.~A.},
    title = "{Spectral distortions of the microwave background radiation resulting from the damping of pressure waves}",
  journal = {\apj},
 keywords = {Astronomical Spectroscopy, Damping, Elastic Waves, Microwaves, Relic Radiation, Universe, Computational Astrophysics, Mass Distribution, Perturbation Theory, Photons, Power Spectra, Radiation Distribution},
     year = 1991,
    month = apr,
   volume = 371,
    pages = {14-28},
      doi = {10.1086/169866},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...371...14D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993ASPC...51..554B,
   author = {{Burigana}, C.},
    title = "{Distortions of the CMB Spectrum by Continuous Heating}",
booktitle = {Observational Cosmology},
     year = 1993,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 51,
   editor = {{Chincarini}, G.~L. and {Iovino}, A. and {Maccacaro}, T. and 
	{Maccagni}, D.},
    month = jan,
    pages = {554},
   adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...51..554B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992NuPhB.373..399E,
   author = {{Ellis}, J. and {Gelmini}, G.~B. and {Lopez}, J.~L. and {Nanopoulos}, D.~V. and 
	{Sarkar}, S.},
    title = "{Astrophysical constraints on massive unstable neutral relic particles}",
  journal = {Nuclear Physics B},
     year = 1992,
    month = apr,
   volume = 373,
    pages = {399-437},
      doi = {10.1016/0550-3213(92)90438-H},
   adsurl = {http://adsabs.harvard.edu/abs/1992NuPhB.373..399E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993PhRvL..70.2661H,
   author = {{Hu}, W. and {Silk}, J.},
    title = "{Thermalization constraints and spectral distortions for massive unstable relic particles}",
  journal = {Physical Review Letters},
 keywords = {Astronomical Spectroscopy, Particle Mass, Relic Radiation, Thermalization (Energy Absorption), Bremsstrahlung, Jeans Theory, Universe},
     year = 1993,
    month = may,
   volume = 70,
    pages = {2661-2664},
      doi = {10.1103/PhysRevLett.70.2661},
   adsurl = {http://adsabs.harvard.edu/abs/1993PhRvL..70.2661H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993PhRvD..48..485H,
   author = {{Hu}, W. and {Silk}, J.},
    title = "{Thermalization and spectral distortions of the cosmic background radiation}",
  journal = {\prd},
 keywords = {Background radiations, Particle-theory and field-theory models of the early Universe, Observational cosmology},
     year = 1993,
    month = jul,
   volume = 48,
    pages = {485-502},
      doi = {10.1103/PhysRevD.48.485},
   adsurl = {http://adsabs.harvard.edu/abs/1993PhRvD..48..485H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...430L...5H,
   author = {{Hu}, W. and {Scott}, D. and {Silk}, J.},
    title = "{Power spectrum constraints from spectral distortions in the cosmic microwave background}",
  journal = {\apjl},
   eprint = {astro-ph/9402045},
 keywords = {Background Radiation, Cosmology, Damping, Microwave Emission, Perturbation, Cosmic Noise, Power Gain, Power Spectra, Relic Radiation},
     year = 1994,
    month = jul,
   volume = 430,
    pages = {L5-L8},
      doi = {10.1086/187424},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...430L...5H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...436..456H,
   author = {{Hu}, W. and {Sugiyama}, N.},
    title = "{Thermal history constraints on the isocurvature baryon model}",
  journal = {\apj},
   eprint = {astro-ph/9403031},
 keywords = {Astronomical Models, Background Radiation, Baryons, Cosmology, Extraterrestrial Radio Waves, Galactic Evolution, Thermal Analysis, Universe, Anisotropy, Cosmic Background Explorer Satellite, Dark Matter, Galactic Clusters, Mathematical Models, Radio Astronomy, Spaceborne Astronomy},
     year = 1994,
    month = dec,
   volume = 436,
    pages = {456-466},
      doi = {10.1086/174921},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...436..456H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995A&A...303..323B,
   author = {{Burigana}, C. and {de Zotti}, G. and {Danese}, L.},
    title = "{Analytical description of spectral distortions of the cosmic microwave background.}",
  journal = {\aap},
 keywords = {COSMIC MICROWAVE BACKGROUND},
     year = 1995,
    month = nov,
   volume = 303,
    pages = {323},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...303..323B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001PhRvD..63b3001M,
   author = {{McDonald}, P. and {Scherrer}, R.~J. and {Walker}, T.~P.},
    title = "{Cosmic microwave background constraint on residual annihilations of relic particles}",
  journal = {\prd},
   eprint = {astro-ph/0008134},
 keywords = {Background radiations, Particle-theory and field-theory models of the early Universe, Observational cosmology, Origin formation and abundances of the elements},
     year = 2001,
    month = jan,
   volume = 63,
   number = 2,
      eid = {023001},
    pages = {023001},
      doi = {10.1103/PhysRevD.63.023001},
   adsurl = {http://adsabs.harvard.edu/abs/2001PhRvD..63b3001M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.336..592S,
   author = {{Salvaterra}, R. and {Burigana}, C.},
    title = "{A joint study of early and late spectral distortions of the cosmic microwave background and of the millimetric foreground}",
  journal = {\mnras},
   eprint = {astro-ph/0203294},
 keywords = {cosmic microwave background, cosmology: theory, diffuse radiation},
     year = 2002,
    month = oct,
   volume = 336,
    pages = {592-610},
      doi = {10.1046/j.1365-8711.2002.05784.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336..592S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2004AIPC..703..397B,
   author = {{Burigana}, C. and {Salvaterra}, R. and {Zizzo}, A.},
    title = "{Cosmological implications of future CMB spectrum experiments}",
 keywords = {Background radiations, Radio microwave},
booktitle = {Plasmas in the Laboratory and in the Universe: New Insights and New Challenges},
     year = 2004,
   series = {American Institute of Physics Conference Series},
   volume = 703,
   editor = {{Bertin}, G. and {Farina}, D. and {Pozzoli}, R.},
    month = apr,
    pages = {397-400},
      doi = {10.1063/1.1718486},
   adsurl = {http://adsabs.harvard.edu/abs/2004AIPC..703..397B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006AN....327..424B,
   author = {{Burigana}, C. and {Zizzo}, A.},
    title = "{Cyclotron emission effect on CMB spectral distortions}",
  journal = {Astronomische Nachrichten},
   eprint = {astro-ph/0601259},
 keywords = {cosmic microwave background, magnetic fields, radiation mechanism: non-thermal},
     year = 2006,
    month = jun,
   volume = 327,
    pages = {424},
      doi = {10.1002/asna.200610547},
   adsurl = {http://adsabs.harvard.edu/abs/2006AN....327..424B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.371.1939R,
   author = {{Rubi{\~n}o-Mart{\'{\i}}n}, J.~A. and {Chluba}, J. and {Sunyaev}, R.~A.
	},
    title = "{Lines in the cosmic microwave background spectrum from the epoch of cosmological hydrogen recombination}",
  journal = {\mnras},
   eprint = {astro-ph/0607373},
 keywords = {atomic processes: cosmic microwave background: cosmology: theory: early Universe, atomic processes, cosmic microwave background, cosmology: theory, early Universe},
     year = 2006,
    month = oct,
   volume = 371,
    pages = {1939-1952},
      doi = {10.1111/j.1365-2966.2006.10839.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371.1939R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...485..377R,
   author = {{Rubi{\~n}o-Mart{\'{\i}}n}, J.~A. and {Chluba}, J. and {Sunyaev}, R.~A.
	},
    title = "{Lines in the cosmic microwave background spectrum from the epoch of cosmological helium recombination}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0711.0594},
 keywords = {atomic processes, cosmology: cosmic microwave background, cosmology:, theory, cosmology: early Universe},
     year = 2008,
    month = jul,
   volume = 485,
    pages = {377-393},
      doi = {10.1051/0004-6361:20078993},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...485..377R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...478L..27C,
   author = {{Chluba}, J. and {Sunyaev}, R.~A.},
    title = "{Is there a need and another way to measure the cosmic microwave background temperature more accurately?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0707.0188},
 keywords = {cosmology: cosmic microwave background, cosmology: theory, cosmology: cosmological parameters},
     year = 2008,
    month = feb,
   volume = 478,
    pages = {L27-L30},
      doi = {10.1051/0004-6361:20078200},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...478L..27C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...501...29C,
   author = {{Chluba}, J. and {Sunyaev}, R.~A.},
    title = "{Pre-recombinational energy release and narrow features in the CMB spectrum}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0803.3584},
 keywords = {atomic processes, radiation mechanisms: general, cosmic microwave background, early Universe, cosmology:, theory},
     year = 2009,
    month = jul,
   volume = 501,
    pages = {29-47},
      doi = {10.1051/0004-6361/200809840},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501...29C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2011IAUS..274..361B,
   author = {{Burigana}, C. and {Procopio}, P. and {De Rosa}, A.},
    title = "{On the solution of the Kompaneets equation in cosmological context: a numerical code to predict the CMB spectrum under general conditions}",
 keywords = {Cosmology, cosmic microwave background, radiative processes, numerical methods},
booktitle = {Advances in Plasma Astrophysics},
     year = 2011,
   series = {IAU Symposium},
   volume = 274,
   editor = {{Bonanno}, A. and {de Gouveia Dal Pino}, E. and {Kosovichev}, A.~G.
	},
    month = jun,
    pages = {361-364},
      doi = {10.1017/S1743921311007277},
   adsurl = {http://adsabs.harvard.edu/abs/2011IAUS..274..361B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012PhRvD..86f5016L,
   author = {{Lochan}, K. and {Das}, S. and {Bassi}, A.},
    title = "{Constraining continuous spontaneous localization strength parameter {$\lambda$} from standard cosmology and spectral distortions of cosmic microwave background radiation}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1206.4425},
 primaryClass = "astro-ph.CO",
 keywords = {Nonlinear or nonlocal theories and models, Background radiations},
     year = 2012,
    month = sep,
   volume = 86,
   number = 6,
      eid = {065016},
    pages = {065016},
      doi = {10.1103/PhysRevD.86.065016},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhRvD..86f5016L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012PhRvD..86b3514D,
   author = {{Dent}, J.~B. and {Easson}, D.~A. and {Tashiro}, H.},
    title = "{Cosmological constraints from CMB distortion}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1202.6066},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, Particle-theory and field-theory models of the early Universe},
     year = 2012,
    month = jul,
   volume = 86,
   number = 2,
      eid = {023514},
    pages = {023514},
      doi = {10.1103/PhysRevD.86.023514},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhRvD..86b3514D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chlubasunyaev2012,
   author = {{Chluba}, J. and {Khatri}, R. and {Sunyaev}, R.~A.},
    title = "{CMB at 2 {$\times$} 2 order: the dissipation of primordial acoustic waves and the observable part of the associated energy release}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1202.0057},
 keywords = {cosmic background radiation, cosmology: observations, cosmology: theory },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {1129-1169},
      doi = {10.1111/j.1365-2966.2012.21474.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.1129C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...540A.124K,
   author = {{Khatri}, R. and {Sunyaev}, R.~A. and {Chluba}, J.},
    title = "{Does Bose-Einstein condensation of CMB photons cancel {$\mu$} distortions created by dissipation of sound waves in the early Universe?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.0475},
 primaryClass = "astro-ph.CO",
 keywords = {radiation mechanisms: thermal, scattering, cosmic background radiation, cosmological parameters, cosmology: theory, early Universe},
     year = 2012,
    month = apr,
   volume = 540,
      eid = {A124},
    pages = {A124},
      doi = {10.1051/0004-6361/201118194},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...540A.124K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...543A.136K,
   author = {{Khatri}, R. and {Sunyaev}, R.~A. and {Chluba}, J.},
    title = "{Mixing of blackbodies: entropy production and dissipation of sound waves in the early Universe}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1205.2871},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmology: theory, early Universe},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {A136},
    pages = {A136},
      doi = {10.1051/0004-6361/201219590},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...543A.136K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012JCAP...09..016K,
   author = {{Khatri}, R. and {Sunyaev}, R.~A.},
    title = "{Beyond y and {$\mu$}: the shape of the CMB spectral distortions in the intermediate epoch, 1.5 {\times} 10$^{4}$lesssimzlesssim2 {\times} 10$^{5}$}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1207.6654},
 primaryClass = "astro-ph.CO",
     year = 2012,
    month = sep,
   volume = 9,
      eid = {016},
    pages = {016},
      doi = {10.1088/1475-7516/2012/09/016},
   adsurl = {http://adsabs.harvard.edu/abs/2012JCAP...09..016K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013JCAP...06..026K,
   author = {{Khatri}, R. and {Sunyaev}, R.~A.},
    title = "{Forecasts for CMB {$\mu$} and i-type spectral distortion constraints on the primordial power spectrum on scales 8lesssimklesssim10$^{4}$ Mpc$^{-1}$ with the future Pixie-like experiments}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1303.7212},
 primaryClass = "astro-ph.CO",
     year = 2013,
    month = jun,
   volume = 6,
      eid = {026},
    pages = {026},
      doi = {10.1088/1475-7516/2013/06/026},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...06..026K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.436.2232C,
   author = {{Chluba}, J.},
    title = "{Distinguishing different scenarios of early energy release with spectral distortions of the cosmic microwave background}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1304.6121},
 keywords = {cosmology: observations, cosmology: theory},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {2232-2243},
      doi = {10.1093/mnras/stt1733},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436.2232C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.440.2544C,
   author = {{Chluba}, J.},
    title = "{Refined approximations for the distortion visibility function and {$\mu$}-type spectral distortions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.6030},
 keywords = {cosmology: observations, cosmology: theory},
     year = 2014,
    month = may,
   volume = 440,
    pages = {2544-2563},
      doi = {10.1093/mnras/stu414},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.440.2544C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000NewA....5...77B,
   author = {{Battistelli}, E.~S. and {Fulcoli}, V. and {Macculi}, C.},
    title = "{The CMBR spectrum: new upper limits for the distortion parameters y and {$\mu$}}",
  journal = {\na},
     year = 2000,
    month = apr,
   volume = 5,
    pages = {77-90},
      doi = {10.1016/S1384-1076(00)00014-2},
   adsurl = {http://adsabs.harvard.edu/abs/2000NewA....5...77B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016arXiv161000015Y,
   author = {{Yasini}, S. and {Pierpaoli}, E.},
    title = "{Beyond the Boost: Measuring the intrinsic dipole of the CMB using the spectral distortions of the monopole and quadrupole}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.00015},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161000015Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013JCAP03012S,
   author = {{Sunyaev}, R.~A. and {Khatri}, R.},
    title = "{Motion induced second order temperature and y-type anisotropies after the subtraction of linear dipole in the CMB maps}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1302.6571},
 primaryClass = "astro-ph.CO",
     year = 2013,
    month = mar,
   volume = 3,
      eid = {012},
    pages = {012},
      doi = {10.1088/1475-7516/2013/03/012},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...03..012S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1935PhRv47817C,
   author = {{Compton}, A.~H. and {Getting}, I.~A.},
    title = "{An Apparent Effect of Galactic Rotation on the Intensity of Cosmic Rays}",
  journal = {Physical Review},
     year = 1935,
    month = jun,
   volume = 47,
    pages = {817-821},
      doi = {10.1103/PhysRev.47.817},
   adsurl = {http://adsabs.harvard.edu/abs/1935PhRv...47..817C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1968ApSS2431G,
   author = {{Gleeson}, L.~J. and {Axford}, W.~I.},
    title = "{The Compton-Getting Effect}",
  journal = {\apss},
     year = 1968,
    month = dec,
   volume = 2,
    pages = {431-437},
      doi = {10.1007/BF02175919},
   adsurl = {http://adsabs.harvard.edu/abs/1968Ap%26SS...2..431G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{buriganaetal08,
   author = {{Burigana}, C. and {Popa}, L.~A. and {Salvaterra}, R. and {Schneider}, R. and 
	{Choudhury}, T.~R. and {Ferrara}, A.},
    title = "{Cosmic microwave background polarization constraints on radiative feedback}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0712.1913},
 keywords = {galaxies: formation , intergalactic medium , cosmic microwave background},
     year = 2008,
    month = mar,
   volume = 385,
    pages = {404-410},
      doi = {10.1111/j.1365-2966.2008.12845.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385..404B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sunyaevkhatri2013,
   author = {{Sunyaev}, R.~A. and {Khatri}, R.},
    title = "{Unavoidable CMB Spectral Features and Blackbody Photosphere of Our Universe}",
  journal = {International Journal of Modern Physics D},
archivePrefix = "arXiv",
   eprint = {1302.6553},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, origin and formation of the Universe, background radiations, observational cosmology, intergalactic matter, Cosmology, Origin and formation of the Universe, Background radiations, Observational cosmology, Intergalactic matter, quasar absorption and emission-line systems, Lyman forest},
     year = 2013,
    month = jun,
   volume = 22,
      eid = {1330014},
    pages = {1330014},
      doi = {10.1142/S0218271813300140},
   adsurl = {http://adsabs.harvard.edu/abs/2013IJMPD..2230014S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chlubaal12,
   author = {{Chluba}, J. and {Erickcek}, A.~L. and {Ben-Dayan}, I.},
    title = "{Probing the Inflaton: Small-scale Power Spectrum Constraints from Measurements of the Cosmic Microwave Background Energy Spectrum}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.2681},
 keywords = {cosmic background radiation, cosmological parameters, cosmology: observations, cosmology: theory, early universe, inflation},
     year = 2012,
    month = oct,
   volume = 758,
      eid = {76},
    pages = {76},
      doi = {10.1088/0004-637X/758/2/76},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...758...76C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{daneseburigana94,
   author = {{Danese}, L. and {Burigana}, C.},
    title = "{Theoretical Aspects of the CMB Spectrum}",
booktitle = {Present and Future of the Cosmic Microwave Background},
     year = 1994,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 429,
   editor = {{Sanz}, J.~L. and {Martinez-Gonzalez}, E. and {Cayon}, L.},
    pages = {28},
      doi = {10.1007/3-540-57755-6_29},
   adsurl = {http://adsabs.harvard.edu/abs/1994LNP...429...28D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ostrikerthompson87,
   author = {{Ostriker}, J.~P. and {Thompson}, C.},
    title = "{Distortion of the cosmic background radiation by superconducting strings}",
  journal = {\apjl},
 keywords = {Background Radiation, Cosmic Rays, Cosmology, String Theory, Superconductivity, Compton Effect, Computational Astrophysics, Energy Sources, Heating, Red Shift, Thomson Scattering},
     year = 1987,
    month = dec,
   volume = 323,
    pages = {L97-L101},
      doi = {10.1086/185065},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...323L..97O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{carretal2010,
   author = {{Carr}, B.~J. and {Kohri}, K. and {Sendouda}, Y. and {Yokoyama}, J.
	},
    title = "{New cosmological constraints on primordial black holes}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0912.5297},
 primaryClass = "astro-ph.CO",
 keywords = {Quantum aspects of black holes evaporation thermodynamics, Dark matter, Black holes, Particle-theory and field-theory models of the early Universe},
     year = 2010,
    month = may,
   volume = 81,
   number = 10,
      eid = {104019},
    pages = {104019},
      doi = {10.1103/PhysRevD.81.104019},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..81j4019C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paniloeb2013,
   author = {{Pani}, P. and {Loeb}, A.},
    title = "{Constraining primordial black-hole bombs through spectral distortions of the cosmic microwave background}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1307.5176},
 primaryClass = "astro-ph.CO",
 keywords = {Relativity and gravitation, Dark matter, Black holes, Classical black holes},
     year = 2013,
    month = aug,
   volume = 88,
   number = 4,
      eid = {041301},
    pages = {041301},
      doi = {10.1103/PhysRevD.88.041301},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..88d1301P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jedamziketal2000,
   author = {{Jedamzik}, K. and {Katalini{\'c}}, V. and {Olinto}, A.~V.},
    title = "{Limit on Primordial Small-Scale Magnetic Fields from Cosmic Microwave Background Distortions}",
  journal = {Physical Review Letters},
   eprint = {astro-ph/9911100},
     year = 2000,
    month = jul,
   volume = 85,
    pages = {700-703},
      doi = {10.1103/PhysRevLett.85.700},
   adsurl = {http://adsabs.harvard.edu/abs/2000PhRvL..85..700J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BartlettSilk1990,
   author = {{Bartlett}, J.~G. and {Silk}, J.},
    title = "{A Comptonization model for the submillimeter background}",
  journal = {\apj},
 keywords = {Astronomical Models, Black Body Radiation, Compton Effect, Relic Radiation, Intergalactic Media, Spectrum Analysis, Submillimeter Waves},
     year = 1990,
    month = apr,
   volume = 353,
    pages = {399-405},
      doi = {10.1086/168625},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...353..399B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ejllidolgov2014,
   author = {{Ejlli}, D. and {Dolgov}, A.~D.},
    title = "{CMB constraints on mass and coupling constant of light pseudoscalar particles}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1312.3558},
 primaryClass = "hep-ph",
 keywords = {Dark matter, Other particles, Cosmology, Background radiations},
     year = 2014,
    month = sep,
   volume = 90,
   number = 6,
      eid = {063514},
    pages = {063514},
      doi = {10.1103/PhysRevD.90.063514},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90f3514E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.437.2507T,
   author = {{Trombetti}, T. and {Burigana}, C.},
    title = "{Semi-analytical description of clumping factor and cosmic microwave background free-free distortions from reionization}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.6177},
 keywords = {radiation mechanisms: general, intergalactic medium, cosmic background radiation, dark ages, reionization, first stars, dark matter},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {2507-2520},
      doi = {10.1093/mnras/stt2063},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437.2507T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...730..138S,
   author = {{Singal}, J. and {Fixsen}, D.~J. and {Kogut}, A. and {Levin}, S. and 
	{Limon}, M. and {Lubin}, P. and {Mirel}, P. and {Seiffert}, M. and 
	{Villela}, T. and {Wollack}, E. and {Wuensche}, C.~A.},
    title = "{The ARCADE 2 Instrument}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.0546},
 primaryClass = "astro-ph.IM",
 keywords = {cosmic background radiation, instrumentation: detectors, radio continuum: galaxies},
     year = 2011,
    month = apr,
   volume = 730,
      eid = {138},
    pages = {138},
      doi = {10.1088/0004-637X/730/2/138},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...730..138S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016arXiv161207151P,
   author = {{Planck Collaboration} and {Akrami}, Y. and {Ashdown}, M. and 
	{Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and 
	{Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and 
	{Basak}, S. and others},
    title = "{Planck intermediate results. LII. Planet flux densities}",
      journal = {accepted by \aap},
   archivePrefix = "arXiv",
   eprint = {1612.07151},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161207151P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016A&A...594A...1P,
   author = {{Planck Collaboration} and {Adam}, R. and {Ade}, P.~A.~R. and 
	{Aghanim}, N. and {Akrami}, Y. and {Alves}, M.~I.~R. and {Arg{\"u}eso}, F. and 
	{Arnaud}, M. and {Arroja}, F. and {Ashdown}, M. and others},
    title = "{Planck 2015 results. I. Overview of products and scientific results}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1502.01582},
 keywords = {cosmology: observations, cosmic background radiation, surveys, space vehicles: instruments, instrumentation: detectors},
     year = 2016,
    month = sep,
   volume = 594,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201527101},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A...1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...594A...5P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and 
	{Barreiro}, R.~B. and {Bartolo}, N. and {Battaglia}, P. and others},
    title = "{Planck 2015 results. V. LFI calibration}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1505.08022},
 primaryClass = "astro-ph.IM",
 keywords = {cosmic background radiation, instrumentation: polarimeters, methods: data analysis},
     year = 2016,
    month = aug,
   volume = 594,
      eid = {A5},
    pages = {A5},
      doi = {10.1051/0004-6361/201526632},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A...5P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...594A...8P,
   author = {{Planck Collaboration} and {Adam}, R. and {Ade}, P.~A.~R. and 
	{Aghanim}, N. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and 
	{Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and others},
    title = "{Planck 2015 results. VIII. High Frequency Instrument data processing: Calibration and maps}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1502.01587},
 keywords = {cosmology: observations, cosmic background radiation, surveys, methods: data analysis},
     year = 2016,
    month = aug,
   volume = 594,
      eid = {A8},
    pages = {A8},
      doi = {10.1051/0004-6361/201525820},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A...8P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...622..759G,
   author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and 
	{Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and 
	{Bartelmann}, M.},
    title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
  journal = {\apj},
   eprint = {astro-ph/0409513},
 keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical},
     year = 2005,
    month = apr,
   volume = 622,
    pages = {759-771},
      doi = {10.1086/427976},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..759G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{delabrouille_etal_ECO,
   author = {{J. Delabrouille, P. de Bernardis, F.~R. Bouchet, A. Ach{\'u}carro, P.~A.~R. Ade, et al., for the CORE collaboration}},
       title = "{Exploring Cosmic Origins with CORE: Survey requirements and mission design}",
           journal = {{\rm Companion Paper}, ArXiv e-prints},
           archivePrefix = "arXiv",
      eprint = {1706.04516},
 keywords = {},
     year = 2017,
         month = jun
}    

@ARTICLE{debernardis_etal_ECO,
   author = {{P. de Bernardis, P.~A.~R. Ade, J. Baselmans, E.~S. Battistelli, A. Benoit, et al., for the CORE Collaboration}},
    title = "{Exploring Cosmic Origins with CORE: The Instrument}",
             journal = {{\rm Companion Paper}, ArXiv e-prints},
             archivePrefix = "arXiv",
   eprint = {1705.02170},
 keywords = {},
     year = 2017,
     month = may
}

@ARTICLE{2016arXiv160907263D,
   author = {{G. De Zotti, J. Gonzalez-Nuevo, M. Lopez-Caniego, M. Negrello, J. Greenslade, et al., for the CORE Collaboration}},
    title = "{Exploring Cosmic Origins with CORE: Extragalactic sources in Cosmic Microwave Background maps}",
  journal = {{\rm Companion Paper}, ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.07263},
 keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160907263D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baccigalupi_etal_ECO,
   author = {{M. Remazeilles, A.J. Banday, C. Baccigalupi, S. Basak, A. Bonaldi, A., et al., for the CORE Collaboration}},
   title = "{Exploring Cosmic Origins with CORE: B-mode Component Separation}",
     journal = {{\rm Companion Paper}, ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1704.04501},
 keywords = {},
     year = 2017,
     month = apr
}

@ARTICLE{ashdown_etal_ECO,
   author = {{P. Natoli, M. Ashdown, R. Banerji, J. Borrill, A. Buzzelli, et al., for the CORE Collaboration}},
   title = "{Exploring Cosmic Origins with CORE: mitigation of systematic effects}",
     journal = {{\rm Companion Paper}, ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1707.04224},
 keywords = {},
     year = 2017,
     month = jul
}

@ARTICLE{2002PhRvD..66j3511L,
    author = {{Lewis}, A. and {Bridle}, S.},
     title = "{Cosmological parameters from CMB and other data: A Monte
Carlo approach}",
   journal = {\prd},
    eprint = {astro-ph/0205436},
  keywords = {Observational cosmology, Applications of Monte Carlo
methods, Neutrino mass and mixing},
      year = 2002,
     month = nov,
    volume = 66,
    number = 10,
       eid = {103511},
     pages = {103511},
       doi = {10.1103/PhysRevD.66.103511},
    adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..66j3511L},
   adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Metropolis53,
   author = "Nicholas Metropolis and Arianna W. Rosenbluth and Marshall
N. Rosenbluth and Augusta H. Teller and Edward Teller",
   title = "Equation of State Calculations by Fast Computing Machines",
   journal = "Journal of Chemical Physics",
   volume = "21",
   pages = "1087-1092",
   year = "1953"
}

@article{Hastings70,
  author = "W.K. Hastings",
  title = "Monte Carlo samping methods using Markov chains and their
applications",
  journal = "Biometrika",
  volume = "57",
  pages = "97-109",
  year = "1970",
  doi ="10.1093/biomet/57.1.97"
}

@ARTICLE{2011JCAP...07..025K,
   author = {{Kogut}, A. and {Fixsen}, D.~J. and {Chuss}, D.~T. and {Dotson}, J. and 
	{Dwek}, E. and {Halpern}, M. and {Hinshaw}, G.~F. and {Meyer}, S.~M. and 
	{Moseley}, S.~H. and {Seiffert}, M.~D. and {Spergel}, D.~N. and 
	{Wollack}, E.~J.},
    title = "{The Primordial Inflation Explorer (PIXIE): a nulling polarimeter for cosmic microwave background observations}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1105.2044},
     year = 2011,
    month = jul,
   volume = 7,
      eid = {025},
    pages = {025},
      doi = {10.1088/1475-7516/2011/07/025},
   adsurl = {http://adsabs.harvard.edu/abs/2011JCAP...07..025K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2016SPIE.9904E..0WK,
   author = {{Kogut}, A. and {Chluba}, J. and {Fixsen}, D.~J. and {Meyer}, S. and 
	{Spergel}, D.},
    title = "{The Primordial Inflation Explorer (PIXIE)}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2016,
   series = {\procspie},
   volume = 9904,
    month = jul,
      eid = {99040W},
    pages = {99040W},
      doi = {10.1117/12.2231090},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9904E..0WK},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...707..916F,
   author = {{Fixsen}, D.~J.},
    title = "{The Temperature of the Cosmic Microwave Background}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0911.1955},
 keywords = {cosmic microwave background, cosmology: observations},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {916-920},
      doi = {10.1088/0004-637X/707/2/916},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707..916F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...512..511M,
   author = {{Mather}, J.~C. and {Fixsen}, D.~J. and {Shafer}, R.~A. and 
	{Mosier}, C. and {Wilkinson}, D.~T.},
    title = "{Calibrator Design for the COBE Far-Infrared Absolute Spectrophotometer (FIRAS)}",
  journal = {\apj},
   eprint = {astro-ph/9810373},
 keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: OBSERVATIONS, INSTRUMENTATION: SPECTROGRAPHS, Cosmology: Cosmic Microwave Background, Cosmology: Observations, Instrumentation: Spectrographs},
     year = 1999,
    month = feb,
   volume = 512,
    pages = {511-520},
      doi = {10.1086/306805},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...512..511M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009JInst...4T2006V,
   author = {{Valenziano}, L. and {Cuttaia}, F. and {De Rosa}, A. and {Terenzi}, L. and 
	{Brighenti}, A. and {Cazzola}, G.~P. and {Garbesi}, A. and {Mariotti}, S. and 
	{Orsi}, G. and others},
    title = "{Planck-LFI: design and performance of the 4 Kelvin Reference Load Unit}",
  journal = {Journal of Instrumentation},
archivePrefix = "arXiv",
   eprint = {1001.4778},
 primaryClass = "astro-ph.IM",
     year = 2009,
    month = dec,
   volume = 4,
    pages = {T12006},
      doi = {10.1088/1748-0221/4/12/T12006},
   adsurl = {http://adsabs.harvard.edu/abs/2009JInst...4T2006V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PLArefESA,
   author = {{Planck Collaboration}},
    title = "{Planck 2015 Release Explanatory Supplement}",
  journal = {ESA},
   eprint = {https://www.cosmos.esa.int/web/planck/publications},
 keywords = {},
     year = 2015,
}

@INPROCEEDINGS{2016SPIE.9904E..0XI,
   author = {{Ishino}, H. and {Akiba}, Y. and {Arnold}, K. and {Barron}, D. and 
	{Borrill}, J. and {Chendra}, R. and {Chinone}, Y. and {Cho}, S. and 
	{Cukierman}, A. and others},
    title = "{LiteBIRD: lite satellite for the study of B-mode polarization and inflation from cosmic microwave background radiation detection}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2016,
   series = {\procspie},
   volume = 9904,
    month = jul,
      eid = {99040X},
    pages = {99040X},
      doi = {10.1117/12.2231995},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9904E..0XI},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...555A.117R,
   author = {{Rubart}, M. and {Schwarz}, D.~J.},
    title = "{Cosmic radio dipole from NVSS and WENSS}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.5559},
 primaryClass = "astro-ph.CO",
 keywords = {radio continuum: galaxies, large-scale structure of Universe},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A117},
    pages = {A117},
      doi = {10.1051/0004-6361/201321215},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A.117R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...810..143A,
   author = {{Atrio-Barandela}, F. and {Kashlinsky}, A. and {Ebeling}, H. and 
	{Fixsen}, D.~J. and {Kocevski}, D.},
    title = "{Probing the Dark Flow Signal in WMAP 9 -Year and Planck Cosmic Microwave Background Maps}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1411.4180},
 keywords = {cosmic background radiation, cosmology: observations, galaxies: clusters: general, large-scale structure of the universe},
     year = 2015,
    month = sep,
   volume = 810,
      eid = {143},
    pages = {143},
      doi = {10.1088/0004-637X/810/2/143},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...810..143A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...734...61F,
   author = {{Fixsen}, D.~J. and {Kashlinsky}, A.},
    title = "{Probing the Universe's Tilt with the Cosmic Infrared Background Dipole}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.0901},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmology: observations, infrared: diffuse background},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/734/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734...61F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1970Ap&SS...7...20S,
   author = {{Sunyaev}, R.~A. and {Zeldovich}, Y.~B.},
    title = "{The interaction of matter and radiation in the hot model of the Universe, II}",
  journal = {\apss},
     year = 1970,
    month = apr,
   volume = 7,
    pages = {20-30},
      doi = {10.1007/BF00653472},
   adsurl = {http://adsabs.harvard.edu/abs/1970Ap%26SS...7...20S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1972JETP...35..643Z,
   author = {{Zel'dovich}, Y.~B. and {Illarionov}, A.~F. and {Sunyaev}, R.~A.
	},
    title = "{The Effect of Energy Release on the Emission Spectrum in a Hot Universe}",
  journal = {Soviet Journal of Experimental and Theoretical Physics},
     year = 1972,
   volume = 35,
    pages = {643},
   adsurl = {http://adsabs.harvard.edu/abs/1972JETP...35..643Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...434..811C,
   author = {{Chluba}, J. and {H{\"u}tsi}, G. and {Sunyaev}, R.~A.},
    title = "{Clusters of galaxies in the microwave band: Influence of the motion of the Solar System}",
  journal = {\aap},
   eprint = {astro-ph/0409058},
 keywords = {galaxies: clusters: general, cosmology: cosmic microwave background, cosmology: observations},
     year = 2005,
    month = may,
   volume = 434,
    pages = {811-817},
      doi = {10.1051/0004-6361:20041942},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...434..811C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.460..227C,
   author = {{Chluba}, J.},
    title = "{Which spectral distortions does {$\Lambda$}CDM actually predict?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1603.02496},
 keywords = {cosmology: observations, cosmology: theory},
     year = 2016,
    month = jul,
   volume = 460,
    pages = {227-239},
      doi = {10.1093/mnras/stw945},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460..227C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969Ap&SS...4..301Z,
   author = {{Zeldovich}, Y.~B. and {Sunyaev}, R.~A.},
    title = "{The Interaction of Matter and Radiation in a Hot-Model Universe}",
  journal = {\apss},
     year = 1969,
    month = jul,
   volume = 4,
    pages = {301-316},
      doi = {10.1007/BF00661821},
   adsurl = {http://adsabs.harvard.edu/abs/1969Ap%26SS...4..301Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1986rpa..book.....R,
   author = {{Rybicki}, G.~B. and {Lightman}, A.~P.},
    title = "{Radiative Processes in Astrophysics}",
booktitle = {Radiative Processes in Astrophysics, by George B.~Rybicki, Alan P.~Lightman, pp.~400.~ISBN 0-471-82759-2.~Wiley-VCH , June 1986.},
publisher = "{Wiley}",
     year = 1986,
    month = jun,
    pages = {400},
   adsurl = {http://adsabs.harvard.edu/abs/1986rpa..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003PhRvD..67f3001K,
   author = {{Kamionkowski}, M. and {Knox}, L.},
    title = "{Aspects of the cosmic microwave background dipole}",
  journal = {\prd},
   eprint = {astro-ph/0210165},
 keywords = {Background radiations},
     year = 2003,
    month = mar,
   volume = 67,
   number = 6,
      eid = {063001},
    pages = {063001},
      doi = {10.1103/PhysRevD.67.063001},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvD..67f3001K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...424..389C,
   author = {{Chluba}, J. and {Sunyaev}, R.~A.},
    title = "{Superposition of blackbodies and the dipole anisotropy: A possibility to calibrate CMB experiments}",
  journal = {\aap},
   eprint = {astro-ph/0404067},
 keywords = {cosmology: cosmic microwave background, cosmology: observations},
     year = 2004,
    month = sep,
   volume = 424,
    pages = {389-408},
      doi = {10.1051/0004-6361:20041016},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...424..389C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..89l3504D,
   author = {{Dai}, L. and {Chluba}, J.},
    title = "{New operator approach to the CMB aberration kernels in harmonic space}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1403.6117},
 keywords = {Cosmology, Special relativity, Symmetry and conservation laws, Background radiations},
     year = 2014,
    month = jun,
   volume = 89,
   number = 12,
      eid = {123504},
    pages = {123504},
      doi = {10.1103/PhysRevD.89.123504},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..89l3504D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000PhRvD..61l3001R,
   author = {{Refregier}, A. and {Komatsu}, E. and {Spergel}, D.~N. and {Pen}, U.-L.},
    title = "{Power spectrum of the Sunyaev-Zel'dovich effect}",
  journal = {\prd},
   eprint = {astro-ph/9912180},
 keywords = {Background radiations, Superclusters, large-scale structure of the Universe, Observational cosmology},
     year = 2000,
    month = jun,
   volume = 61,
   number = 12,
      eid = {123001},
    pages = {123001},
      doi = {10.1103/PhysRevD.61.123001},
   adsurl = {http://adsabs.harvard.edu/abs/2000PhRvD..61l3001R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008PhRvD..78h3012E,
   author = {{Erickcek}, A.~L. and {Carroll}, S.~M. and {Kamionkowski}, M.
	},
    title = "{Superhorizon perturbations and the cosmic microwave background}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0808.1570},
 keywords = {Background radiations, Particle-theory and field-theory models of the early Universe, Mathematical and relativistic aspects of cosmology},
     year = 2008,
    month = oct,
   volume = 78,
   number = 8,
      eid = {083012},
    pages = {083012},
      doi = {10.1103/PhysRevD.78.083012},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhRvD..78h3012E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008PhRvD..78l3529Z,
   author = {{Zibin}, J.~P. and {Scott}, D.},
    title = "{Gauging the cosmic microwave background}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0808.2047},
 keywords = {Background radiations, Mathematical and relativistic aspects of cosmology},
     year = 2008,
    month = dec,
   volume = 78,
   number = 12,
      eid = {123529},
    pages = {123529},
      doi = {10.1103/PhysRevD.78.123529},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhRvD..78l3529Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980MNRAS.190..413S,
   author = {{Sunyaev}, R.~A. and {Zeldovich}, I.~B.},
    title = "{The velocity of clusters of galaxies relative to the microwave background - The possibility of its measurement}",
  journal = {\mnras},
 keywords = {Background Radiation, Galactic Clusters, Microwave Emission, Polarized Radiation, Velocity Measurement, Background Noise, Cosmic Gases, Cosmology},
     year = 1980,
    month = feb,
   volume = 190,
    pages = {413-420},
      doi = {10.1093/mnras/190.3.413},
   adsurl = {http://adsabs.harvard.edu/abs/1980MNRAS.190..413S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1981Ap&SS..77..529F,
   author = {{Fabbri}, R.},
    title = "{Spectrum of the Sunyaev-Zel'dovich effect for high electron temperatures}",
  journal = {\apss},
 keywords = {Background Radiation, Cosmic Rays, Hot Electrons, Relativistic Effects, Spectrum Analysis, Anisotropy, Electron Energy, Electron Gas, Infrared Radiation},
     year = 1981,
    month = jul,
   volume = 77,
    pages = {529-537},
      doi = {10.1007/BF00649478},
   adsurl = {http://adsabs.harvard.edu/abs/1981Ap%26SS..77..529F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979ApJ...232..348W,
   author = {{Wright}, E.~L.},
    title = "{Distortion of the microwave background by a hot intergalactic medium}",
  journal = {\apj},
 keywords = {Background Radiation, Intergalactic Media, Microwaves, X Ray Astronomy, Cosmic X Rays, Electrons, Frequency Shift, Velocity Distribution},
     year = 1979,
    month = sep,
   volume = 232,
    pages = {348-351},
      doi = {10.1086/157294},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...232..348W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1987MNRAS.228P...5H,
   author = {{Harmon}, R.~T. and {Lahav}, O. and {Meurs}, E.~J.~A.},
    title = "{The dipole anisotropy of a new, colour-selected, IRAS galaxy sample}",
  journal = {\mnras},
 keywords = {Anisotropic Media, Galactic Clusters, Infrared Spectra, Interstellar Magnetic Fields, Magnetic Dipoles, Astronomical Catalogs, Background Radiation, Dipole Moments, Infrared Astronomy Satellite, Void Ratio},
     year = 1987,
    month = sep,
   volume = 228,
    pages = {5P-10P},
      doi = {10.1093/mnras/228.1.5P},
   adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.228P...5H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1992ApJ...397..395S,
   author = {{Strauss}, M.~A. and {Yahil}, A. and {Davis}, M. and {Huchra}, J.~P. and 
	{Fisher}, K.},
    title = "{A redshift survey of IRAS galaxies. V - The acceleration on the Local Group}",
  journal = {\apj},
 keywords = {Infrared Sources (Astronomy), Local Group (Astronomy), Red Shift, Sky Surveys (Astronomy), Astronomical Models, Computational Astrophysics, Infrared Astronomy Satellite, Power Spectra, Relic Radiation},
     year = 1992,
    month = oct,
   volume = 397,
    pages = {395-419},
      doi = {10.1086/171796},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...397..395S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...598L...1M,
   author = {{Maller}, A.~H. and {McIntosh}, D.~H. and {Katz}, N. and {Weinberg}, M.~D.
	},
    title = "{The Clustering Dipole of the Local Universe from the Two Micron All Sky Survey}",
  journal = {\apjl},
   eprint = {astro-ph/0303592},
 keywords = {Cosmology: Cosmic Microwave Background, Galaxies: Clusters: General, Infrared: Galaxies, Cosmology: Large-Scale Structure of Universe},
     year = 2003,
    month = nov,
   volume = 598,
    pages = {L1-L5},
      doi = {10.1086/380388},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598L...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.368.1515E,
   author = {{Erdo{\v g}du}, P. and {Huchra}, J.~P. and {Lahav}, O. and {Colless}, M. and 
	{Cutri}, R.~M. and {Falco}, E. and {George}, T. and {Jarrett}, T. and 
	{Jones}, D.~H. and {Kochanek}, C.~S. and {Macri}, L. and {Mader}, J. and 
	{Martimbeau}, N. and {Pahre}, M. and {Parker}, Q. and {Rassat}, A. and 
	{Saunders}, W.},
    title = "{The dipole anisotropy of the 2 Micron All-Sky Redshift Survey}",
  journal = {\mnras},
   eprint = {astro-ph/0507166},
 keywords = {methods: data analysis , Local Group , cosmology: observations , large-scale structure of Universe , infrared: galaxies},
     year = 2006,
    month = jun,
   volume = 368,
    pages = {1515-1526},
      doi = {10.1111/j.1365-2966.2006.10243.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368.1515E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1996ApJ...460..569B,
   author = {{Branchini}, E. and {Plionis}, M.},
    title = "{Reconstructing Positions and Peculiar Velocities of Galaxy Clusters within 25,000 Kilometers per Second: The Cluster Real Space Dipole}",
  journal = {\apj},
   eprint = {astro-ph/9501028},
 keywords = {COSMOLOGY: OBSERVATIONS, GALAXIES: CLUSTERS: GENERAL, GALAXIES: DISTANCES AND REDSHIFTS, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE},
     year = 1996,
    month = apr,
   volume = 460,
    pages = {569},
      doi = {10.1086/176993},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...460..569B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...500....1P,
   author = {{Plionis}, M. and {Kolokotronis}, V.},
    title = "{The X-Ray Cluster Dipole}",
  journal = {\apj},
   eprint = {astro-ph/9707147},
 keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, GALAXIES: CLUSTERS: GENERAL, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE, X-RAYS: GALAXIES, Cosmology: Cosmic Microwave Background, Galaxies: Clusters: General, Cosmology: Large-Scale Structure of Universe, X-Rays: Galaxies},
     year = 1998,
    month = jun,
   volume = 500,
    pages = {1-7},
      doi = {10.1086/305709},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500....1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2000MNRAS.314..375R,
   author = {{Rowan-Robinson}, M. and {Sharpe}, J. and {Oliver}, S.~J. and 
	{Keeble}, O. and {Canavezes}, A. and {Saunders}, W. and {Taylor}, A.~N. and 
	{Valentine}, H. and {Frenk}, C.~S. and {Efstathiou}, G.~P. and 
	{McMahon}, R.~G. and {White}, S.~D.~M. and {Sutherland}, W. and 
	{Tadros}, H. and {Maddox}, S.},
    title = "{The IRAS PSCz dipole}",
  journal = {\mnras},
   eprint = {astro-ph/9912223},
 keywords = {GALAXIES: CLUSTERS: GENERAL, COSMIC MICROWAVE BACKGROUND, LARGE-SCALE STRUCTURE OF UNIVERSE, INFRARED: GALAXIES},
     year = 2000,
    month = may,
   volume = 314,
    pages = {375-397},
      doi = {10.1046/j.1365-8711.2000.03313.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.314..375R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2006MNRAS.373.1112B,
   author = {{Basilakos}, S. and {Plionis}, M.},
    title = "{The PSCz dipole revisited}",
  journal = {\mnras},
   eprint = {astro-ph/0609476},
 keywords = {galaxies: clusters: general, large-scale structure of Universe, infrared: galaxies},
     year = 2006,
    month = dec,
   volume = 373,
    pages = {1112-1116},
      doi = {10.1111/j.1365-2966.2006.11075.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.373.1112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011ApJ...741...31B,
   author = {{Bilicki}, M. and {Chodorowski}, M. and {Jarrett}, T. and {Mamon}, G.~A.
	},
    title = "{Is the Two Micron All Sky Survey Clustering Dipole Convergent?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1102.4356},
 keywords = {cosmology: observations, cosmology: theory, large-scale structure of Universe, methods: data analysis, methods: statistical, surveys},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {31},
    pages = {31},
      doi = {10.1088/0004-637X/741/1/31},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2013PhRvD..88h3529W,
   author = {{Wiltshire}, D.~L. and {Smale}, P.~R. and {Mattsson}, T. and 
	{Watkins}, R.},
    title = "{Hubble flow variance and the cosmic rest frame}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1201.5371},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, Classical general relativity, Observational cosmology},
     year = 2013,
    month = oct,
   volume = 88,
   number = 8,
      eid = {083529},
    pages = {083529},
      doi = {10.1103/PhysRevD.88.083529},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..88h3529W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JCAP...06..035B,
   author = {{Bolejko}, K. and {Nazer}, M.~A. and {Wiltshire}, D.~L.},
    title = "{Differential cosmic expansion and the Hubble flow anisotropy}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1512.07364},
     year = 2016,
    month = jun,
   volume = 6,
      eid = {035},
    pages = {035},
      doi = {10.1088/1475-7516/2016/06/035},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...06..035B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JCAP...12..022G,
   author = {{Garc{\'{\i}}a-Garc{\'{\i}}a}, C. and {Maroto}, A.~L. and {Mart{\'{\i}}n-Moruno}, P.
	},
    title = "{Cosmology with moving bimetric fluids}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1608.06493},
 primaryClass = "gr-qc",
     year = 2016,
    month = dec,
   volume = 12,
      eid = {022},
    pages = {022},
      doi = {10.1088/1475-7516/2016/12/022},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...12..022G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012MNRAS.427.1994G,
   author = {{Gibelyou}, C. and {Huterer}, D.},
    title = "{Dipoles in the sky}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1205.6476},
 primaryClass = "astro-ph.CO",
 keywords = {large-scale structure of Universe},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {1994-2021},
      doi = {10.1111/j.1365-2966.2012.22032.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.1994G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984MNRAS.206..377E,
   author = {{Ellis}, G.~F.~R. and {Baldwin}, J.~E.},
    title = "{On the expected anisotropy of radio source counts}",
  journal = {\mnras},
 keywords = {Anisotropy, Background Radiation, Radio Sources (Astronomy), Relic Radiation, Extragalactic Radio Sources, Microwave Emission, Velocity Distribution},
     year = 1984,
    month = jan,
   volume = 206,
    pages = {377-381},
      doi = {10.1093/mnras/206.2.377},
   adsurl = {http://adsabs.harvard.edu/abs/1984MNRAS.206..377E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015APh....61....1T,
   author = {{Tiwari}, P. and {Kothari}, R. and {Naskar}, A. and {Nadkarni-Ghosh}, S. and 
	{Jain}, P.},
    title = "{Dipole anisotropy in sky brightness and source count distribution in radio NVSS data}",
  journal = {Astroparticle Physics},
archivePrefix = "arXiv",
   eprint = {1307.1947},
 keywords = {Radio galaxies: high-redshift, Galaxies: active, CMBR dipole},
     year = 2015,
    month = feb,
   volume = 61,
    pages = {1-11},
      doi = {10.1016/j.astropartphys.2014.06.004},
   adsurl = {http://adsabs.harvard.edu/abs/2015APh....61....1T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.447.2658T,
   author = {{Tiwari}, P. and {Jain}, P.},
    title = "{Dipole anisotropy in integrated linearly polarized flux density in NVSS data}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.3970},
 keywords = {polarization, galaxies: active, galaxies: high-redshift, cosmology: miscellaneous},
     year = 2015,
    month = mar,
   volume = 447,
    pages = {2658-2670},
      doi = {10.1093/mnras/stu2535},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.2658T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...397..420B,
   author = {{Boggess}, N.~W. and {Mather}, J.~C. and {Weiss}, R. and {Bennett}, C.~L. and 
	{Cheng}, E.~S. and {Dwek}, E. and {Gulkis}, S. and {Hauser}, M.~G. and 
	{Janssen}, M.~A. and {Kelsall}, T. and {Meyer}, S.~S. and {Moseley}, S.~H. and 
	{Murdock}, T.~L. and {Shafer}, R.~A. and {Silverberg}, R.~F. and 
	{Smoot}, G.~F. and {Wilkinson}, D.~T. and {Wright}, E.~L.},
    title = "{The COBE mission - Its design and performance two years after launch}",
  journal = {\apj},
 keywords = {Cosmic Background Explorer Satellite, Infrared Radiation, Microwaves, Relic Radiation, Spaceborne Astronomy, Astronomical Satellites, Radiation Measurement, Satellite Instruments},
     year = 1992,
    month = oct,
   volume = 397,
    pages = {420-429},
      doi = {10.1086/171797},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...397..420B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.466..425W,
   author = {{Wallis}, C.~G.~R. and {Brown}, M.~L. and {Battye}, R.~A. and 
	{Delabrouille}, J.},
    title = "{Optimal scan strategies for future CMB satellite experiments}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1604.02290},
 keywords = {methods: observational, cosmic background radiation, cosmology: observations, inflation},
     year = 2017,
    month = apr,
   volume = 466,
    pages = {425-442},
      doi = {10.1093/mnras/stw2577},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466..425W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999AJ....118..337C,
   author = {{Courteau}, S. and {van den Bergh}, S.},
    title = "{The Solar Motion Relative to the Local Group}",
  journal = {\aj},
   eprint = {astro-ph/9903298},
 keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, GALAXIES: LOCAL GROUP},
     year = 1999,
    month = jul,
   volume = 118,
    pages = {337-345},
      doi = {10.1086/300942},
   adsurl = {http://adsabs.harvard.edu/abs/1999AJ....118..337C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.427..274S,
   author = {{Sch{\"o}nrich}, R.},
    title = "{Galactic rotation and solar motion from stellar kinematics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.3079},
 keywords = {stars: kinematics and dynamics, Galaxy: disc, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, solar neighbourhood},
     year = 2012,
    month = nov,
   volume = 427,
    pages = {274-287},
      doi = {10.1111/j.1365-2966.2012.21631.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427..274S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015aska.confE..32S,
   author = {{Schwarz}, D.~J. and {Bacon}, D. and {Chen}, S. and {Clarkson}, C. and 
	{Huterer}, D. and {Kunz}, M. and {Maartens}, R. and {Raccanelli}, A. and 
	{Rubart}, M. and {Starck}, J.~L.},
    title = "{Testing foundations of modern cosmology with SKA all-sky surveys}",
  journal = {Advancing Astrophysics with the Square Kilometre Array (AASKA14)},
archivePrefix = "arXiv",
   eprint = {1501.03820},
     year = 2015,
    month = apr,
      eid = {32},
    pages = {32},
   adsurl = {http://adsabs.harvard.edu/abs/2015aska.confE..32S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016PhRvD..94d3006N,
   author = {{Notari}, A. and {Quartin}, M.},
    title = "{CMB all-scale blackbody distortions induced by linearizing temperature}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1510.08793},
     year = 2016,
    month = aug,
   volume = 94,
   number = 4,
      eid = {043006},
    pages = {043006},
      doi = {10.1103/PhysRevD.94.043006},
   adsurl = {http://adsabs.harvard.edu/abs/2016PhRvD..94d3006N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Planck_inprep,
   author = {{Planck Collaboration}},
    title = "{Dipole-modulated Compton-$y$ signature}",
  journal = {{\rm in prep.}},
   eprint = {},
 keywords = {},
     year = 2017
}

